Global Structure-from-Motion Revisited

Recovering 3D structure and camera motion from images has been a long-standing focus of computer vision research and is known as Structure-from-Motion (SfM). Solutions to this problem are categorized into incremental and global approaches. Until now, the most popular systems follow the incremental paradigm due to its superior accuracy and robustness, while global approaches are drastically more scalable and efficient. With this work, we revisit the problem of global SfM and propose GLOMAP as a new general-purpose system that outperforms the state of the art in global SfM. In terms of accuracy and robustness, we achieve results on-par or superior to COLMAP, the most widely used incremental SfM, while being orders of magnitude faster. We share our system as an open-source implementation at {https://github.com/colmap/glomap}.

==> tex/fig/ablations.tex <==

% \begin{figure}[t]
%     \centering
%      \includegraphics[width=0.85\textwidth]{figure/long_legend.png}\\
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/loss_function.png}
%          \caption{log(loss) vs iterations}
%          \label{fig:loss_function}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figure/ablation_pt.png}
%          \caption{AUC@$3^\circ$ vs noise level}
%          \label{fig:ablation_pt}
%      \end{subfigure}
%      % \begin{subfigure}[b]{0.25\textwidth}
%      %     \centering
%      %     \includegraphics[width=\textwidth]{figure/legend.png}
%      %     % \caption{AUC@$3^\circ$ vs noise level}
%      %     \label{fig:result_euroc}
%      % \end{subfigure}
%     \caption{ \todo{should it be kept?}
%     }
%     \label{fig:ablation}\vspace{-4mm}
%     % \vspace{-10px}
% \end{figure}

==> tex/tbl/eth3d_dslr_hsfm.tex <==
\begin{table}[t]
    \centering
    \caption{Results on ETH3D MVS (DSLR)~\cite{schoeps2017cvpr}. On this dataset, the proposed method outperforms other global SfM baselines and is comparable to COLMAP~\cite{schoenberger2016sfm}.}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{AUC @ $1^\circ$} && \multicolumn{5}{c}{AUC @ $3^\circ$} && \multicolumn{5}{c}{AUC @ $5^\circ$} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
% courtyard && 54.6 & \textbf{89.3} & 45.7 & 86.2 & 86.9 && 73.1 & \textbf{96.4} & 78.4 & 95.4 & 95.6 && 79.8 & \textbf{97.9} & 86.8 & 97.2 & 97.4 && 11.2 & \textbf{9.2} & 18.4 & 21.5 & 39.2 \\
% delivery\_area && 91.2 & 89.2 & 60.0 & 92.1 & \textbf{92.2} && 97.1 & 96.4 & 85.0 & \textbf{97.4} & \textbf{97.4} && 98.2 & 97.8 & 90.9 & \textbf{98.4} & \textbf{98.5} && 235.7 & \textbf{3.4} & 9.7 & 9.0 & 26.4 \\
% electro && 72.3 & 63.6 & 40.6 & \textbf{80.7} & 69.6 && 81.6 & 72.9 & 62.9 & \textbf{90.6} & 75.5 && 83.7 & 76.1 & 68.6 & \textbf{93.7} & 76.8 && 99.9 & \textbf{3.7} & 4.8 & 6.0 & 23.9 \\
% facade && 89.2 & 89.8 & 65.8 & \textbf{90.4} & 90.1 && 96.3 & 96.6 & 84.4 & \textbf{96.8} & 96.7 && 97.8 & 98.0 & 89.1 & \textbf{98.1} & 98.0 && \textbf{35.1} & 37.1 & 65.5 & 79.4 & 113.5 \\
% kicker && 81.3 & 78.4 & 51.3 & 85.5 & \textbf{86.2} && 89.3 & 85.5 & 73.2 & \textbf{95.1} & 91.1 && 91.0 & 88.2 & 78.6 & \textbf{97.0} & 92.1 && \textbf{1.6} & 2.3 & 4.1 & 4.8 & 16.2 \\
% meadow && 8.4 & 20.7 & 0.0 & \textbf{74.8} & 58.4 && 12.0 & 32.4 & 0.7 & \textbf{90.5} & 76.4 && 12.9 & 36.5 & 0.8 & \textbf{94.3} & 80.5 && \textbf{0.2} & 0.7 & 0.5 & 1.1 & 5.1 \\
% office && 17.9 & 37.3 & 3.5 & \textbf{57.1} & 43.6 && 22.9 & 51.5 & 4.2 & \textbf{80.6} & 55.5 && 24.5 & 57.4 & 4.4 & \textbf{87.8} & 59.1 && 0.4 & 0.5 & \textbf{0.3} & 1.0 & 19.1 \\
% pipes && 26.4 & 74.8 & 22.9 & \textbf{88.5} & 85.9 && 34.6 & 91.1 & 56.1 & \textbf{96.2} & 95.3 && 39.6 & 94.7 & 70.6 & \textbf{97.7} & 97.2 && \textbf{0.3} & \textbf{0.4} & 0.6 & 0.6 & 3.4 \\
% playground && 48.6 & 75.3 & 53.0 & \textbf{90.9} & 90.6 && 54.9 & 81.7 & 72.6 & \textbf{96.9} & 96.8 && 56.2 & 83.1 & 77.3 & \textbf{98.2} & 98.1 && 121.5 & 6.2 & \textbf{4.7} & 7.5 & 29.8 \\
% relief && 89.3 & \textbf{92.8} & 68.3 & \textbf{92.8} & 92.7 && 96.4 & \textbf{97.6} & 87.9 & \textbf{97.6} & \textbf{97.6} && 97.9 & \textbf{98.6} & 92.7 & \textbf{98.6} & 98.5 && \textbf{3.7} & 5.6 & 9.7 & 11.8 & 34.1 \\
% relief\_2 && 11.1 & 93.7 & 51.5 & 93.7 & \textbf{94.4} && 11.6 & 97.9 & 79.5 & 97.9 & \textbf{98.1} && 11.7 & 98.7 & 87.5 & 98.7 & \textbf{98.9} && \textbf{0.7} & 2.3 & 5.3 & 5.7 & 24.1 \\
% terrace && 91.8 & 91.1 & 74.5 & 92.0 & \textbf{92.2} && 97.3 & 97.0 & 91.3 & 97.3 & \textbf{97.4} && \textbf{98.4} & 98.2 & 94.8 & \textbf{98.4} & \textbf{98.5} && \textbf{1.1} & 1.4 & 2.4 & 3.9 & 10.9 \\
% terrains && 69.7 & 49.2 & 45.5 & \textbf{84.5} & 81.7 && 88.9 & 77.5 & 73.0 & \textbf{94.6} & 93.5 && 93.2 & 85.8 & 81.5 & \textbf{96.7} & 96.0 && 62.6 & \textbf{2.6} & 7.9 & 4.5 & 21.7 \\
% botanical\_garden && 25.0 & \textbf{82.9} & 3.1 & 82.8 & 4.5 && 29.2 & \textbf{94.1} & 4.2 & 94.0 & 4.7 && 30.0 & 96.3 & 4.5 & \textbf{96.4} & 4.8 && 1.0 & 1.7 & \textbf{0.6} & 3.6 & 9.1 \\
% boulders && 89.3 & 86.9 & 68.4 & 90.4 & \textbf{90.6} && 96.4 & 95.6 & 87.6 & 96.8 & \textbf{96.9} && 97.8 & 97.4 & 92.1 & \textbf{98.1} & \textbf{98.1} && 4.1 & \textbf{2.9} & 5.7 & 11.4 & 18.5 \\
% bridge && 44.4 & 86.7 & 83.4 & 45.0 & \textbf{91.4} && 47.4 & 94.4 & 94.0 & 47.6 & \textbf{97.1} && 48.0 & 96.3 & 96.4 & 48.1 & \textbf{98.3} && 35.1 & \textbf{29.6} & 61.2 & 98.3 & 91.9 \\
% door && 93.6 & 93.6 & 0.0 & 95.8 & \textbf{96.5} && 97.8 & 97.9 & 0.0 & 98.6 & \textbf{98.8} && 98.7 & 98.7 & 0.0 & 99.2 & \textbf{99.3} && 1.2 & 0.6 & \textbf{0.5} & 3.5 & 4.2 \\
% exhibition\_hall && 10.2 & 31.4 & - & 18.7 & \textbf{85.4} && 14.3 & 37.7 & - & 21.8 & \textbf{94.3} && 15.5 & 39.3 & - & 22.6 & \textbf{96.5} && \textbf{20.6} & 71.8 & - & 174.1 & 72.0 \\
% lecture\_room && 79.9 & 76.4 & 52.1 & \textbf{84.0} & 82.7 && 92.6 & 91.3 & 78.9 & \textbf{94.4} & 94.0 && 95.6 & 94.8 & 86.0 & \textbf{96.6} & 96.4 && 3.3 & \textbf{2.0} & 2.6 & 12.5 & 10.9 \\
% living\_room && 87.7 & 84.5 & 64.2 & 87.4 & \textbf{88.0} && 95.7 & 94.5 & 85.8 & 95.6 & \textbf{95.8} && \textbf{97.4} & 96.7 & 90.8 & 97.3 & \textbf{97.4} && \textbf{9.4} & 13.3 & 28.9 & 32.3 & 49.1 \\
% lounge && \textbf{31.6} & 26.8 & 10.6 & 30.5 & 31.3 && \textbf{32.7} & 31.1 & 12.4 & 32.4 & \textbf{32.7} && \textbf{33.0} & 32.0 & 12.8 & 32.8 & 32.9 && \textbf{0.4} & \textbf{0.4} & \textbf{0.4} & 0.8 & 1.8 \\
% observatory && 56.0 & 61.5 & \textbf{65.7} & 63.1 & 62.8 && 82.8 & 85.6 & \textbf{87.3} & 86.1 & 85.9 && 89.5 & 91.3 & \textbf{92.4} & 91.6 & 91.5 && 5.8 & \textbf{3.4} & 6.0 & 27.2 & 24.4 \\
% old\_computer && 22.0 & 48.2 & 14.2 & 49.7 & \textbf{78.0} && 40.4 & 58.9 & 37.6 & 57.7 & \textbf{90.0} && 47.5 & 61.2 & 46.5 & 59.4 & \textbf{92.5} && 5.9 & \textbf{2.4} & 4.7 & 12.7 & 19.6 \\
% statue && 96.1 & 98.7 & 94.7 & \textbf{98.8} & 98.6 && 98.7 & \textbf{99.6} & 98.2 & \textbf{99.6} & 99.5 && 99.2 & 99.7 & 98.9 & \textbf{99.8} & 99.7 && \textbf{0.9} & 1.4 & 1.5 & 11.6 & 7.4 \\
% terrace\_2 && 87.1 & 88.8 & 84.1 & \textbf{90.5} & 90.2 && 95.5 & 96.2 & 94.7 & \textbf{96.8} & 96.7 && 97.3 & 97.7 & 96.8 & \textbf{98.1} & 98.0 && \textbf{0.9} & \textbf{1.0} & 1.2 & 4.2 & 10.2 \\
% \midrule
% \textit{Average} && 59.0 & 72.5 & 46.8 & 77.8 & \textbf{78.6} && 67.2 & 82.1 & 63.8 & 85.9 & \textbf{86.1} && 69.4 & 84.5 & 68.4 & \textbf{87.8} & \textbf{87.8} && 26.5 & \textbf{8.2} & 10.3 & 22.0 & 27.5 \\

courtyard && 54.6 & \textbf{89.3} & 88.8 & 86.2 & 86.9 && 73.1 & \textbf{96.4} & 96.3 & 95.4 & 95.6 && 79.8 & \textbf{97.9} & 97.8 & 97.2 & 97.4 && 11.2 & \textbf{9.2} & 17.9 & 21.5 & 39.2 \\
delivery\_area && 91.2 & 89.2 & 88.8 & 92.1 & \textbf{92.2} && 97.1 & 96.4 & 96.3 & \textbf{97.4} & \textbf{97.4} && 98.2 & 97.8 & 97.8 & \textbf{98.4} & \textbf{98.5} && 235.7 & \textbf{3.4} & 8.3 & 9.0 & 26.4 \\
electro && 72.3 & 63.6 & 67.8 & \textbf{80.7} & 69.6 && 81.6 & 72.9 & 74.8 & \textbf{90.6} & 75.5 && 83.7 & 76.1 & 76.3 & \textbf{93.7} & 76.8 && 99.9 & \textbf{3.7} & 4.3 & 6.0 & 23.9 \\
facade && 89.2 & 89.8 & 87.6 & \textbf{90.4} & 90.1 && 96.3 & 96.6 & 94.1 & \textbf{96.8} & 96.7 && 97.8 & 98.0 & 95.4 & \textbf{98.1} & 98.0 && \textbf{35.1} & 37.1 & 65.9 & 79.4 & 113.5 \\
kicker && 81.3 & 78.4 & 78.2 & 85.5 & \textbf{86.2} && 89.3 & 85.5 & 84.2 & \textbf{95.1} & 91.1 && 91.0 & 88.2 & 85.5 & \textbf{97.0} & 92.1 && \textbf{1.6} & 2.3 & 3.9 & 4.8 & 16.2 \\
meadow && 8.4 & 20.7 & 0.8 & \textbf{74.8} & 58.4 && 12.0 & 32.4 & 0.9 & \textbf{90.5} & 76.4 && 12.9 & 36.5 & 0.9 & \textbf{94.3} & 80.5 && \textbf{0.2} & 0.7 & 0.5 & 1.1 & 5.1 \\
office && 17.9 & 37.3 & 2.4 & \textbf{57.1} & 43.6 && 22.9 & 51.5 & 3.9 & \textbf{80.6} & 55.5 && 24.5 & 57.4 & 4.2 & \textbf{87.8} & 59.1 && 0.4 & 0.5 & \textbf{0.3} & 1.0 & 19.1 \\
pipes && 26.4 & 74.8 & 61.4 & \textbf{88.5} & 85.9 && 34.6 & 91.1 & 68.8 & \textbf{96.2} & 95.3 && 39.6 & 94.7 & 70.3 & \textbf{97.7} & 97.2 && \textbf{0.3} & \textbf{0.4} & 0.5 & 0.6 & 3.4 \\
playground && 48.6 & 75.3 & 75.3 & \textbf{90.9} & 90.6 && 54.9 & 81.7 & 81.4 & \textbf{96.9} & 96.8 && 56.2 & 83.1 & 82.7 & \textbf{98.2} & 98.1 && 121.5 & 6.2 & \textbf{5.1} & 7.5 & 29.8 \\
relief && 89.3 & 92.8 & \textbf{93.1} & 92.8 & 92.7 && 96.4 & 97.6 & \textbf{97.7} & 97.6 & 97.6 && 97.9 & \textbf{98.6} & \textbf{98.6} & \textbf{98.6} & 98.5 && \textbf{3.7} & 5.6 & 10.0 & 11.8 & 34.1 \\
relief\_2 && 11.1 & 93.7 & 92.9 & 93.7 & \textbf{94.4} && 11.6 & 97.9 & 97.6 & 97.9 & \textbf{98.1} && 11.7 & 98.7 & 98.6 & 98.7 & \textbf{98.9} && \textbf{0.7} & 2.3 & 5.0 & 5.7 & 24.1 \\
terrace && 91.8 & 91.1 & 91.4 & 92.0 & \textbf{92.2} && 97.3 & 97.0 & 97.1 & 97.3 & \textbf{97.4} && \textbf{98.4} & 98.2 & 98.3 & \textbf{98.4} & \textbf{98.5} && \textbf{1.1} & 1.4 & 2.3 & 3.9 & 10.9 \\
terrains && 69.7 & 49.2 & \textbf{85.6} & 84.5 & 81.7 && 88.9 & 77.5 & \textbf{95.0} & 94.6 & 93.5 && 93.2 & 85.8 & \textbf{97.0} & 96.7 & 96.0 && 62.6 & \textbf{2.6} & 5.8 & 4.5 & 21.7 \\
botanical\_garden && 25.0 & \textbf{82.9} & 4.3 & 82.8 & 4.5 && 29.2 & \textbf{94.1} & 4.7 & 94.0 & 4.7 && 30.0 & 96.3 & 4.7 & \textbf{96.4} & 4.8 && 1.0 & 1.7 & \textbf{0.6} & 3.6 & 9.1 \\
boulders && 89.3 & 86.9 & 87.5 & 90.4 & \textbf{90.6} && 96.4 & 95.6 & 95.8 & 96.8 & \textbf{96.9} && 97.8 & 97.4 & 97.5 & \textbf{98.1} & \textbf{98.1} && 4.1 & \textbf{2.9} & 5.4 & 11.4 & 18.5 \\
bridge && 44.4 & 86.7 & 91.0 & 45.0 & \textbf{91.4} && 47.4 & 94.4 & 96.9 & 47.6 & \textbf{97.1} && 48.0 & 96.3 & 98.2 & 48.1 & \textbf{98.3} && 35.1 & \textbf{29.6} & 57.9 & 98.3 & 91.9 \\
door && 93.6 & 93.6 & 0.0 & 95.8 & \textbf{96.5} && 97.8 & 97.9 & 0.0 & 98.6 & \textbf{98.8} && 98.7 & 98.7 & 0.0 & 99.2 & \textbf{99.3} && 1.2 & 0.6 & \textbf{0.5} & 3.5 & 4.2 \\
exhibition\_hall && 10.2 & 31.4 & - & 18.7 & \textbf{85.4} && 14.3 & 37.7 & - & 21.8 & \textbf{94.3} && 15.5 & 39.3 & - & 22.6 & \textbf{96.5} && \textbf{20.6} & 71.8 & - & 174.1 & 72.0 \\
lecture\_room && 79.9 & 76.4 & 79.4 & \textbf{84.0} & 82.7 && 92.6 & 91.3 & 92.5 & \textbf{94.4} & 94.0 && 95.6 & 94.8 & 95.5 & \textbf{96.6} & 96.4 && 3.3 & \textbf{2.0} & 2.5 & 12.5 & 10.9 \\
living\_room && 87.7 & 84.5 & 87.7 & 87.4 & \textbf{88.0} && 95.7 & 94.5 & 95.7 & 95.6 & \textbf{95.8} && \textbf{97.4} & 96.7 & \textbf{97.4} & 97.3 & \textbf{97.4} && \textbf{9.4} & 13.3 & 29.3 & 32.3 & 49.1 \\
lounge && \textbf{31.6} & 26.8 & 11.7 & 30.5 & 31.3 && \textbf{32.7} & 31.1 & 12.8 & 32.4 & \textbf{32.7} && \textbf{33.0} & 32.0 & 13.0 & 32.8 & 32.9 && \textbf{0.4} & \textbf{0.4} & \textbf{0.4} & 0.8 & 1.8 \\
observatory && 56.0 & 61.5 & 62.6 & \textbf{63.1} & 62.8 && 82.8 & 85.6 & 86.0 & \textbf{86.1} & 85.9 && 89.5 & 91.3 & \textbf{91.5} & \textbf{91.6} & 91.5 && 5.8 & \textbf{3.4} & 5.7 & 27.2 & 24.4 \\
old\_computer && 22.0 & 48.2 & 43.8 & 49.7 & \textbf{78.0} && 40.4 & 58.9 & 56.1 & 57.7 & \textbf{90.0} && 47.5 & 61.2 & 58.7 & 59.4 & \textbf{92.5} && 5.9 & \textbf{2.4} & 4.7 & 12.7 & 19.6 \\
statue && 96.1 & 98.7 & 98.7 & \textbf{98.8} & 98.6 && 98.7 & \textbf{99.6} & \textbf{99.6} & \textbf{99.6} & 99.5 && 99.2 & 99.7 & \textbf{99.8} & \textbf{99.8} & 99.7 && \textbf{0.9} & 1.4 & 1.5 & 11.6 & 7.4 \\
terrace\_2 && 87.1 & 88.8 & 88.8 & \textbf{90.5} & 90.2 && 95.5 & 96.2 & 96.2 & \textbf{96.8} & 96.7 && 97.3 & 97.7 & 97.7 & \textbf{98.1} & 98.0 && \textbf{0.9} & \textbf{1.0} & 1.2 & 4.2 & 10.2 \\
\midrule
\textit{Average} && 59.0 & 72.5 & 65.4 & 77.8 & \textbf{78.6} && 67.2 & 82.1 & 71.8 & 85.9 & \textbf{86.1} && 69.4 & 84.5 & 73.2 & \textbf{87.8} & \textbf{87.8} && 26.5 & \textbf{8.2} & 10.0 & 22.0 & 27.5 \\

      \bottomrule
    \end{tabular}
    }
    \label{tbl:eth3d_drls}
    \vspace{-15px}
\end{table}


==> tex/tbl/eth3d_rig_hsfm.tex <==
\begin{table}[t]
    \centering
    \caption{Results on ETH3D MVS (rig)~\cite{schoeps2017cvpr}. Proposed GLOMAP largely outperforms other SfM systems by a large margin while maintaining the efficiency of global SfM.}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{Recall @ 0.1m} && \multicolumn{5}{c}{AUC @ 0.1m} && \multicolumn{5}{c}{AUC @ 0.5m}
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
delivery\_area && 8.2 & 99.8 & - & \textbf{100.0} & \textbf{100.0} && 5.0 & 75.1 & - & 82.6 & \textbf{83.4} && 8.4 & 94.9 & - & 96.5 & \textbf{96.7} && \textbf{235.7} & 250.0 & - & 415.4 & 1745.9 \\
electro && 18.9 & 86.0 & 89.4 & \textbf{98.8} & 89.1 && 9.2 & 35.9 & 32.4 & \textbf{50.5} & 26.4 && 19.9 & 85.0 & 78.1 & \textbf{89.8} & 84.1 && \textbf{99.9} & 181.2 & 240.6 & 366.8 & 3283.1 \\
forest && 10.9 & \textbf{99.6} & \textbf{99.6} & \textbf{99.6} & \textbf{99.6} && 6.5 & 94.2 & \textbf{94.5} & 93.3 & 94.3 && 13.6 & 98.5 & \textbf{98.6} & 98.3 & 98.5 && \textbf{306.6} & 532.1 & 1262.4 & 1254.8 & 7571.6 \\
playground && 8.8 & 90.1 & 92.2 & \textbf{99.0} & 1.8 && 3.4 & 35.3 & 80.9 & \textbf{92.5} & 1.0 && 11.3 & 85.6 & 89.9 & \textbf{97.7} & 1.6 && \textbf{121.5} & 386.0 & 491.7 & 680.8 & 350.2 \\
terrains && 20.6 & 98.6 & \textbf{99.4} & \textbf{99.4} & \textbf{99.4} && 13.0 & 69.4 & \textbf{93.5} & 93.2 & \textbf{93.5} && 19.4 & 93.0 & \textbf{98.2} & 98.1 & \textbf{98.2} && \textbf{62.6} & 194.7 & 256.4 & 261.7 & 1333.9 \\
\midrule
\textit{Average} && 13.5 & 94.8 & 95.2 & \textbf{99.4} & 78.0 && 7.4 & 62.0 & 75.3 & \textbf{82.4} & 59.7 && 14.5 & 91.4 & 91.2 & \textbf{96.1} & 75.8 && \textbf{165.3} & 308.8 & 562.8 & 595.9 & 2856.9 \\
      \bottomrule
    \end{tabular}
    }
    % \caption{Results on ETH3D MVS~\cite{schoeps2017cvpr}, rig sequences. The proposed GLOMAP largely outperforms other SfM systems by a large margin.}
    \label{tbl:eth3d_rig}
    \vspace{-10px}
\end{table}



==> tex/tbl/eth3d_slam_hsfm.tex <==
\begin{table}[t]
    \centering
    \caption{Result on ETH3D SLAM~\cite{Schops_2019_CVPR} dataset. Each row represents the average results on scenes with the same prefix. The proposed system largely outperforms global SfM baselines by a large margin, and also achieves better results than COLMAP~\cite{schoenberger2016sfm}.}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{Recall @ 0.1m} && \multicolumn{5}{c}{AUC @ 0.1m} && \multicolumn{5}{c}{AUC @ 0.5m}
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule

cables && 76.8 & \textbf{88.0} & 68.0 & \textbf{88.0} & 67.7 && 56.0 & 53.1 & 48.6 & \textbf{77.0} & 56.4 && 76.7 & 81.0 & 64.1 & \textbf{85.8} & 69.7 && 103.1 & 170.9 & \textbf{87.6} & \textbf{87.6} & 2553.4 \\
camera && 2.2 & 33.0 & 0.0 & \textbf{47.3} & 34.7 && 2.0 & 14.4 & 0.0 & \textbf{27.6} & 25.7 && 2.2 & 35.0 & 0.0 & \textbf{43.9} & 33.2 && \textbf{1.5} & 24.6 & 13.2 & 13.2 & 196.2 \\
ceiling && 6.1 & 28.2 & 3.5 & \textbf{33.5} & 28.6 && 3.5 & 12.9 & 3.0 & 16.5 & \textbf{17.9} && 8.0 & 29.3 & 3.4 & \textbf{31.2} & 26.8 && \textbf{78.3} & 132.5 & 84.0 & 84.0 & 1057.7 \\
desk && 27.9 & 33.7 & 6.5 & \textbf{34.1} & 24.4 && 16.9 & 17.0 & 5.8 & \textbf{27.1} & 20.8 && 28.6 & 32.8 & 6.4 & \textbf{35.3} & 23.7 && 376.2 & 200.9 & \textbf{145.3} & \textbf{145.3} & 1115.1 \\
einstein && 32.7 & 41.1 & 22.9 & \textbf{43.3} & 33.7 && 23.3 & 30.0 & 17.7 & \textbf{33.6} & 25.6 && 34.3 & 42.3 & 24.3 & \textbf{42.9} & 36.9 && 150.3 & \textbf{61.2} & 85.2 & 81.7 & 1230.8 \\
kidnap && 73.1 & \textbf{73.3} & 31.2 & \textbf{73.3} & \textbf{73.3} && 63.4 & 59.8 & 28.5 & \textbf{69.5} & 68.5 && 71.2 & 70.6 & 30.6 & \textbf{72.5} & 72.3 && 114.4 & 668.8 & \textbf{78.7} & \textbf{78.7} & 731.2 \\
large && 35.6 & \textbf{47.3} & 0.0 & 37.3 & 44.5 && 17.4 & 20.2 & 0.0 & \textbf{31.7} & 21.2 && 34.0 & 43.4 & 0.0 & 36.8 & \textbf{43.5} && 91.9 & 113.0 & \textbf{62.4} & \textbf{62.4} & 983.8 \\
mannequin && 49.0 & 58.5 & 1.0 & \textbf{67.9} & 59.3 && 36.9 & 38.8 & 0.7 & 50.0 & \textbf{52.8} && 49.1 & 58.4 & 1.0 & \textbf{67.4} & 58.4 && 33.5 & 66.5 & \textbf{32.3} & 32.9 & 301.2 \\
motion && 18.4 & 14.1 & 0.0 & \textbf{23.9} & 18.2 && \textbf{11.8} & 7.1 & 0.0 & 8.2 & \textbf{11.8} && 23.4 & 13.7 & 0.0 & \textbf{28.2} & 19.4 && 859.7 & \textbf{84.8} & - & 345.2 & 9995.1 \\
planar && 30.4 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} && 13.3 & 94.4 & 94.4 & 97.6 & \textbf{98.3} && 44.8 & 98.9 & 98.9 & 99.5 & \textbf{99.7} && 313.8 & \textbf{154.8} & 291.8 & 291.8 & 2349.7 \\
plant && 76.9 & 86.9 & 65.0 & 90.3 & \textbf{93.1} && 62.5 & 71.3 & 61.0 & 72.5 & \textbf{81.7} && 76.8 & 89.3 & 64.2 & 91.6 & \textbf{92.4} && \textbf{21.7} & 48.8 & 24.0 & 24.0 & 202.7 \\
reflective && 13.5 & 14.2 & 0.1 & 18.4 & \textbf{25.8} && 4.3 & 7.6 & 0.1 & 7.6 & \textbf{9.5} && 20.2 & 21.6 & 0.1 & 24.7 & \textbf{33.5} && 721.3 & \textbf{104.7} & 215.1 & 215.1 & 6573.9 \\
repetitive && 26.3 & 28.7 & 10.1 & \textbf{33.3} & 28.5 && 23.9 & 17.0 & 8.7 & \textbf{27.3} & 27.2 && 25.8 & 27.4 & 9.8 & \textbf{32.1} & 28.3 && \textbf{63.2} & 106.4 & 81.9 & 81.9 & 561.1 \\
sfm && 83.4 & \textbf{90.3} & 50.4 & 90.1 & 55.9 && 57.2 & 48.0 & 35.9 & \textbf{62.7} & 37.3 && 79.8 & 86.7 & 49.6 & \textbf{89.5} & 56.3 && \textbf{91.7} & 158.7 & 230.7 & 230.7 & 469.6 \\
sofa && 11.2 & 18.6 & 0.0 & 24.2 & \textbf{32.2} && 5.5 & 11.4 & 0.0 & 14.0 & \textbf{28.6} && 10.3 & 18.4 & 0.0 & 23.0 & \textbf{31.6} && \textbf{9.1} & 9.9 & 12.1 & 12.1 & 157.3 \\
table && 79.1 & 83.8 & 39.7 & \textbf{99.9} & \textbf{99.9} && 68.2 & 58.4 & 24.9 & 74.8 & \textbf{95.6} && 76.9 & 82.0 & 37.8 & 94.9 & \textbf{99.1} && 182.0 & \textbf{61.2} & 118.3 & 118.3 & 2777.7 \\
vicon && 63.0 & 73.3 & 6.2 & \textbf{94.8} & 81.2 && 23.6 & 51.9 & 5.6 & \textbf{56.5} & 34.4 && 72.3 & 84.4 & 6.1 & \textbf{91.0} & 74.2 && 50.9 & 149.8 & \textbf{39.6} & \textbf{39.6} & 474.8 \\
\midrule
\textit{Average} && 48.1 & 60.0 & 28.0 & \textbf{65.5} & 58.0 && 34.9 & 41.0 & 23.2 & \textbf{49.3} & 47.7 && 48.8 & 60.1 & 27.6 & \textbf{64.7} & 57.9 && 120.8 & 97.7 & \textbf{84.2} & 87.7 & 1115.4 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:eth3d_drls}
    \vspace{-15px}
\end{table}


==> tex/tbl/imc_hsfm.tex <==
\begin{table}[t]
    \centering
    \caption{Results on IMC 2023~\cite{IMC2023}. Our GLOMAP method comes close to COLMAP generated ground truth while outperforming global SfM by a large margin.}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{AUC @ $1^\circ$} && \multicolumn{5}{c}{AUC @ $3^\circ$} && \multicolumn{5}{c}{AUC @ $5^\circ$} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
bike && - & 32.8 & 0.0 & 63.2 & \textbf{76.7} && - & 43.9 & 0.0 & 72.6 & \textbf{86.0} && - & 65.9 & 0.0 & 79.6 & \textbf{93.0} && - & 2.0 & \textbf{0.8} & 1.6 & 1.1 \\
chairs && - & 11.0 & 0.0 & \textbf{17.8} & 0.0 && - & 15.2 & 0.0 & \textbf{23.2} & 0.0 && - & 21.3 & 0.0 & \textbf{30.6} & 0.0 && - & 2.8 & 1.6 & 3.2 & \textbf{0.6} \\
fountain && 20.9 & 90.2 & 0.0 & 88.9 & \textbf{91.0} && 23.0 & 94.1 & 0.0 & 93.4 & \textbf{94.6} && 24.5 & 97.0 & 1.1 & 96.7 & \textbf{97.3} && \textbf{0.8} & 2.2 & 2.0 & 2.8 & 5.9 \\
cyprus && 1.2 & 69.5 & 2.8 & \textbf{73.2} & 44.8 && 1.3 & 74.2 & 3.6 & \textbf{78.7} & 48.1 && 1.3 & 77.8 & 4.2 & \textbf{84.3} & 50.6 && \textbf{0.3} & 3.1 & 0.9 & 1.6 & 11.1 \\
dioscuri && 0.0 & 0.3 & 0.0 & 36.3 & \textbf{58.6} && 0.0 & 0.7 & 0.0 & 38.9 & \textbf{61.3} && 0.1 & 2.2 & 0.0 & 42.7 & \textbf{63.8} && 41.9 & 23.2 & \textbf{8.9} & 53.8 & 156.2 \\
wall && 56.1 & \textbf{91.5} & 19.1 & 20.5 & 88.4 && 73.3 & \textbf{94.9} & 31.2 & 33.5 & 93.0 && 86.7 & \textbf{97.4} & 54.9 & 58.1 & 96.5 && \textbf{23.8} & 35.4 & 39.1 & 198.2 & 63.5 \\
kyiv-puppet-theater && 0.0 & \textbf{1.4} & 0.0 & \textbf{1.4} & 0.0 && 0.0 & 2.2 & 0.2 & \textbf{2.6} & 0.0 && 0.3 & \textbf{4.2} & 0.4 & 4.1 & 0.0 && 0.3 & 2.0 & 0.4 & 1.1 & \textbf{0.3} \\
brandenburg\_gate && 21.0 & 1.6 & 0.8 & 51.5 & \textbf{70.0} && 34.6 & 4.3 & 2.6 & 61.9 & \textbf{77.2} && 53.4 & 12.3 & 9.0 & 73.3 & \textbf{83.8} && 1171.8 & \textbf{131.3} & 151.2 & 256.2 & 1472.1 \\
british\_museum && 18.0 & 17.5 & 2.0 & 43.5 & \textbf{61.5} && 31.5 & 29.1 & 5.5 & 56.9 & \textbf{72.7} && 50.8 & 46.4 & 15.2 & 73.1 & \textbf{83.9} && 78.1 & \textbf{44.5} & 83.9 & 71.5 & 318.0 \\
buckingham\_palace && 3.8 & 1.3 & 1.5 & 67.8 & \textbf{80.5} && 12.1 & 3.8 & 4.6 & 74.8 & \textbf{86.2} && 33.8 & 11.7 & 13.8 & 82.3 & \textbf{91.0} && 429.7 & \textbf{156.1} & 205.7 & 295.9 & 4948.2 \\
colosseum\_exterior && 37.2 & 2.8 & 0.3 & 41.7 & \textbf{80.7} && 52.7 & 6.1 & 1.0 & 61.5 & \textbf{86.0} && 69.1 & 13.4 & 4.6 & 77.9 & \textbf{90.8} && 542.8 & \textbf{331.3} & 554.5 & 527.5 & 3561.7 \\
grand\_place\_brussels && 18.1 & 8.6 & 0.5 & 62.5 & \textbf{68.6} && 32.3 & 14.8 & 1.8 & 72.1 & \textbf{76.4} && 50.4 & 33.2 & 9.5 & 81.2 & \textbf{84.1} && 124.2 & \textbf{71.6} & 164.8 & 123.4 & 520.3 \\
lincoln..\_statue && 0.5 & 7.1 & 0.1 & 63.1 & \textbf{67.1} && 3.9 & 16.4 & 0.6 & 68.3 & \textbf{71.4} && 23.5 & 32.7 & 3.4 & 73.3 & \textbf{75.2} && 99.9 & \textbf{44.3} & 58.4 & 71.0 & 362.3 \\
notre\_dame..\_facade && 32.4 & 1.0 & 0.7 & 59.7 & \textbf{69.1} && 42.9 & 4.3 & 3.3 & 65.2 & \textbf{72.5} && 55.1 & 14.6 & 12.5 & 70.6 & \textbf{75.5} && 2592.1 & \textbf{801.0} & 1614.0 & 1978.6 & 52135.4 \\
pantheon\_exterior && 49.3 & 51.3 & 0.6 & 66.2 & \textbf{79.4} && 62.1 & 63.0 & 2.4 & 74.2 & \textbf{83.5} && 74.4 & 74.6 & 9.9 & 81.8 & \textbf{87.2} && 285.7 & \textbf{208.7} & 300.5 & 237.1 & 1454.6 \\
piazza\_san\_marco && 1.4 & 4.9 & 0.4 & \textbf{68.2} & 57.0 && 5.2 & 14.8 & 1.6 & \textbf{78.6} & 70.3 && 23.0 & 39.7 & 8.6 & \textbf{88.0} & 83.4 && 16.7 & \textbf{12.5} & 34.1 & 27.1 & 74.2 \\
sacre\_coeur && 37.0 & 14.9 & 2.9 & 73.6 & \textbf{78.4} && 50.7 & 23.7 & 7.1 & 77.6 & \textbf{80.8} && 64.7 & 39.9 & 17.6 & 81.0 & \textbf{82.8} && 196.1 & \textbf{105.1} & 181.7 & 193.8 & 682.2 \\
sagrada\_familia && 29.7 & 46.7 & 0.1 & 52.6 & \textbf{53.8} && 38.6 & 52.1 & 0.9 & 57.0 & \textbf{58.4} && 48.3 & 57.2 & 5.5 & 61.3 & \textbf{62.5} && 42.6 & \textbf{37.5} & 88.2 & 65.4 & 237.0 \\
st\_pauls\_cathedral && 1.2 & 9.7 & 0.1 & 64.7 & \textbf{72.6} && 5.8 & 24.3 & 0.7 & 73.4 & \textbf{78.8} && 25.5 & 44.6 & 7.0 & 81.7 & \textbf{84.9} && 61.9 & \textbf{35.9} & 70.9 & 72.1 & 241.4 \\
st\_peters\_square && 30.9 & 6.1 & 1.4 & 66.5 & \textbf{83.6} && 45.8 & 12.3 & 4.1 & 74.7 & \textbf{87.8} && 64.0 & 24.6 & 11.9 & 83.0 & \textbf{91.7} && 961.0 & 374.9 & \textbf{363.9} & 610.2 & 6051.9 \\
taj\_mahal && 38.4 & 4.6 & 1.1 & \textbf{68.8} & \textbf{68.8} && 50.9 & 11.1 & 3.4 & 74.2 & \textbf{75.4} && 64.9 & 23.2 & 12.3 & 79.9 & \textbf{81.6} && 380.1 & \textbf{176.4} & 271.3 & 386.0 & 4528.9 \\
trevi\_fountain && 43.3 & 22.5 & 0.3 & 74.6 & \textbf{80.5} && 56.2 & 40.4 & 1.9 & 79.7 & \textbf{84.4} && 69.2 & 59.1 & 10.9 & 84.6 & \textbf{87.8} && 1202.9 & \textbf{689.5} & 886.4 & 715.2 & 12294.4 \\
\midrule
\textit{Average} && 22.0 & 22.6 & 1.6 & 55.7 & \textbf{65.0} && 31.2 & 29.4 & 3.5 & 63.3 & \textbf{70.2} && 44.1 & 40.6 & 9.6 & 71.3 & \textbf{74.9} && 412.6 & \textbf{149.6} & 231.1 & 267.9 & 4051.0 \\
\bottomrule 
    \end{tabular}
    }
    \label{tbl:imc}
    \vspace{-10px}
\end{table}



==> tex/tbl/lamar_map_hsfm.tex <==
\begin{table}[t]
    \centering
    \caption{Result on ETH3D SLAM~\cite{Schops_2019_CVPR} dataset. Each row represents the average results on scenes with the same prefix. The proposed system largely outperforms global SfM baselines by a large margin, and also achieves better results than COLMAP~\cite{schoenberger2016sfm}.}
    \vspace{-5px}

    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{Recall @ 0.1m} && \multicolumn{5}{c}{AUC @ 0.1m} && \multicolumn{5}{c}{AUC @ 0.5m}
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
        
CAB && - & 3.2 & - & 6.3 & \textbf{12.9} && - & 1.3 & - & 2.7 & \textbf{8.5} && - & 9.2 & - & 11.5 & \textbf{15.6} && - & 1953.5 & - & 4833.0 & \textbf{0.0} \\
HGE && - & 3.4 & 0.9 & 13.4 & \textbf{38.9} && - & 1.3 & 0.5 & 8.1 & \textbf{18.0} && - & 9.6 & 0.8 & 14.5 & \textbf{46.9} && - & 1829.7 & \textbf{1749.4} & 4618.2 & 249771.1 \\
LIN && - & 8.6 & 0.0 & 24.5 & \textbf{45.1} && - & 3.3 & 0.0 & 9.8 & \textbf{20.9} && - & 24.1 & 0.0 & 31.6 & \textbf{52.3} && - & 2783.3 & \textbf{2369.6} & 9747.2 & 620176.4 \\
\midrule
\textit{Average} && - & 5.1 & 0.5 & 14.7 & \textbf{32.3} && - & 2.0 & 0.2 & 6.9 & \textbf{15.8} && - & 14.3 & 0.4 & 19.2 & \textbf{38.3} && - & 2188.8 & \textbf{2059.5} & 6399.5 & 289982.5 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:eth3d_drls}
    \vspace{-15px}
\end{table}

==> tex/tbl/lamar_map_postsubmission.tex <==

\begin{table}[t]
    \centering
    \caption{LaMAR}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c a l c c c a l c c c a l c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        % && \multicolumn{3}{c}{Thres 5m} && \multicolumn{3}{c}{AUC @ 5} && \multicolumn{3}{c}{AUC @ 10} 
        && \multicolumn{4}{c}{Recall @ 1m} && \multicolumn{4}{c}{AUC @ 1m} && \multicolumn{4}{c}{AUC @ 5m} 
        && \multicolumn{4}{c}{Time (s)}
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} &&  \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
% LIN && 57.8 & 77.1 & \textbf{83.7} && 21.1 & 35.9 & \textbf{44.0} && 46.6 & 60.9 & \textbf{66.4} && \textbf{532.4} & 5245.3 & 620176.4 \\
submission\\
CAB && - & 3.2 & 6.3 & \textbf{12.9} && - & 1.3 & 2.7 & \textbf{8.5} && - & 9.2 & 11.5 & \textbf{15.6} && - & \textbf{1453.5} & 3114.9 & 194033.6 \\
HGE && - & 3.4 & 13.4 & \textbf{38.9} && - & 1.3 & 8.1 & \textbf{18.0} && - & 1.3 & 14.5 & \textbf{46.9} && - & \textbf{1829.7} & 2996.4 & 249771.1 \\
LIN && - & 8.6 & 24.5 & \textbf{45.1} && - & 3.3 & 9.8 & \textbf{20.9} && - & 24.1 & 31.6 & \textbf{52.3} && - & \textbf{2783.3} & 7496.2 & 620176.4 \\
\midrule
new pipeline\\
CAB && - & 3.2 & 6.6 & \textbf{13.0} && - & 1.3 & 2.9 & \textbf{5.8} && - & 9.2 & 11.2 & \textbf{19.2} && - & \textbf{1453.5} & \textbf{0.0} & \textbf{0.0} \\
HGE && - & 3.4 & 16.1 & \textbf{38.9} && - & 1.3 & 10.5 & \textbf{18.0} && - & 1.3 & 17.3 & \textbf{46.9} && - & \textbf{1829.7} & 2996.4 & 249771.1 \\
LIN && - & 8.6 & \textbf{74.1} & 44.2 && - & 3.3 & \textbf{39.8} & 17.7 &&  - & 24.1 & \textbf{81.3} & 52.3 &&  - & \textbf{2783.3} & \textbf{0.0} & 620176.4 \\
      \bottomrule
    \end{tabular}
    }
\end{table}

==> tex/tbl/mip360_hsfm.tex <==
\begin{table}[t]
    \centering
    \caption{Results on MIP360~\cite{barron2022mip} datasets. The proposed method largely outperforms other baselines while obtaining similar results as COLMAP~\cite{schoenberger2016sfm}.}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{AUC @ $3^\circ$} && \multicolumn{5}{c}{AUC @ $5^\circ$} && \multicolumn{5}{c}{AUC @ $10^\circ$} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~HSfM~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule

bicycle && 89.3 & 70.1 & 0.1 & 95.3 & \textbf{95.8} && 92.7 & 80.7 & 1.0 & 97.2 & \textbf{97.5} && 95.3 & 89.2 & 7.6 & 98.6 & \textbf{98.8} && 176.9 & \textbf{34.5} & 51.2 & 69.9 & 120.6 \\
bonsai && 9.5 & 48.2 & 1.7 & 87.8 & \textbf{92.3} && 28.2 & 50.3 & 5.2 & 92.6 & \textbf{95.3} && 61.3 & 69.5 & 13.3 & 96.3 & \textbf{97.7} && \textbf{176.0} & 218.0 & 304.4 & 291.2 & 662.5 \\
counter && 96.9 & 99.0 & 2.1 & 97.9 & \textbf{99.2} && 98.1 & 99.4 & 7.0 & 98.7 & \textbf{99.5} && 99.1 & 99.7 & 21.2 & 99.4 & \textbf{99.8} && \textbf{46.6} & 79.5 & 211.2 & 141.7 & 270.5 \\
garden && 95.0 & 0.0 & 0.0 & 97.1 & \textbf{97.4} && 97.0 & 0.2 & 0.0 & 98.3 & \textbf{98.4} && 98.5 & 1.8 & 0.4 & 99.1 & \textbf{99.2} && 40.2 & \textbf{36.2} & 65.3 & 109.7 & 291.8 \\
kitchen && 88.5 & 92.1 & 1.4 & 92.3 & \textbf{95.0} && 93.1 & 95.2 & 5.6 & 95.4 & \textbf{97.0} && 96.5 & 97.6 & 19.8 & 97.7 & \textbf{98.5} && \textbf{127.0} & 146.8 & 361.4 & 325.2 & 619.1 \\
room && 39.4 & 32.4 & 0.4 & 88.0 & \textbf{96.2} && 42.0 & 33.7 & 1.5 & 92.2 & \textbf{97.7} && 44.8 & 35.6 & 5.1 & 95.8 & \textbf{98.8} && 96.3 & 80.2 & \textbf{66.7} & 182.3 & 371.6 \\
stump && 95.2 & 2.8 & 0.0 & 97.0 & \textbf{99.2} && 97.0 & 5.0 & 0.0 & 98.2 & \textbf{99.5} && 98.5 & 16.2 & 0.1 & 99.1 & \textbf{99.8} && 38.7 & 15.5 & \textbf{7.4} & 31.9 & 83.9 \\
\midrule
\textit{Average} && 73.4 & 49.2 & 0.8 & 93.6 & \textbf{96.4} && 78.3 & 52.1 & 2.9 & 96.1 & \textbf{97.8} && 84.9 & 58.5 & 9.7 & 98.0 & \textbf{98.9} && 100.2 & \textbf{87.2} & 152.5 & 164.5 & 345.7 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:eth3d_drls}
    \vspace{-15px}
\end{table}

==> tex/tbl/postsubmission.tex <==



\begin{table}[t]
    \centering
    \caption{New results -- Mip360}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{AUC @ $3^\circ$} && \multicolumn{5}{c}{AUC @ $5^\circ$} && \multicolumn{5}{c}{AUC @ $10^\circ$} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} \\  \midrule
bicycle && 89.2 & 70.7 & 95.3 & 95.2 & \textbf{95.8} && 92.7 & 81.0 & 97.2 & 97.1 & \textbf{97.5} && 95.3 & 89.4 & 98.6 & 98.6 & \textbf{98.7} && 176.9 & \textbf{34.5} & 55.3 & 58.6 & 120.6 \\
bonsai && 9.4 & 48.4 & 87.7 
& 87.6 & \textbf{92.7} && 27.9 & 50.3 & 92.5 & 92.5 & \textbf{95.6} && 61.2 & 66.9 & 96.2 & 96.2 & \textbf{97.8} && \textbf{176.0} & 218.0 & 265.2 & 278.6 & 662.5 \\
counter && 96.9 & 99.0 & 97.9 & 98.0 & \textbf{99.2} && 98.1 & 99.4 & 98.8 & 98.8 & \textbf{99.5} && 99.1 & 99.7 & 99.4 & 99.4 & \textbf{99.8} && \textbf{46.6} & 79.5 & 130.8 & 145.3 & 270.5 \\
garden && 95.0 & 0.6 & 97.0 & 96.8 & \textbf{97.3} && 97.0 & 0.7 & 98.2 & 98.1 & \textbf{98.4} && 98.5 & 2.2 & 99.1 & 99.0 & \textbf{99.2} && 40.2 & \textbf{36.2} & 98.7 & 107.7 & 291.8 \\
kitchen && 88.5 & 92.0 & 92.3 & 92.4 & \textbf{94.9} && 93.1 & 95.2 & 95.4 & 95.4 & \textbf{97.0} && 96.5 & 97.6 & 97.7 & 97.7 & \textbf{98.5} && \textbf{127.0} & 146.8 & 303.5 & 312.9 & 619.1 \\
room && 39.6 & 32.6 & 88.1 & 96.1 & \textbf{96.2} && 42.2 & 33.8 & 92.3 & \textbf{97.7} & \textbf{97.7} && 45.0 & 35.7 & 95.8 & 98.8 & \textbf{98.9} && 96.3 & \textbf{80.2} & 168.5 & 179.4 & 371.6 \\
stump && 95.3 & 3.5 & 97.0 & 96.4 & \textbf{99.2} && 97.1 & 5.7 & 98.2 & 97.8 & \textbf{99.5} && 98.5 & 16.8 & 99.1 & 98.9 & \textbf{99.7} && 38.7 & \textbf{15.5} & 26.4 & 43.8 & 83.9 \\
\midrule
\textit{Average} && 73.4 & 49.5 & 93.6 & 94.6 & \textbf{96.5} && 78.3 & 52.3 & 96.1 & 96.8 & \textbf{97.9} && 84.9 & 58.3 & 98.0 & 98.4 & \textbf{98.9} && 100.2 & \textbf{87.2} & 149.8 & 160.9 & 345.7 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


\begin{table}[t]
    \centering
    \caption{New results -- ETH3D rig}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{AUC @ $1^\circ$} && \multicolumn{5}{c}{AUC @ $3^\circ$} && \multicolumn{5}{c}{AUC @ $5^\circ$} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} \\  \midrule
delivery\_area && 0.0 & 30.0 & 67.0 & \textbf{70.1} & 66.6 && 0.1 & 71.0 & 87.6 & \textbf{88.7} & 87.5 && 0.3 & 81.6 & 92.3 & \textbf{92.9} & 92.2 && 235.7 & 250.0 & 264.8 & \textbf{232.2} & 1745.9 \\
electro && 0.2 & 13.4 & 40.6 & \textbf{41.5} & 38.4 && 1.8 & 48.2 & 70.5 & \textbf{71.9} & 65.2 && 2.9 & 63.4 & 80.5 & \textbf{81.6} & 75.2 && \textbf{99.9} & 181.2 & 283.0 & 218.3 & 3283.2 \\
forest && 0.0 & 68.3 & 73.4 & 74.0 & \textbf{74.7} && 0.1 & 87.7 & 89.6 & 89.8 & \textbf{90.3} && 0.1 & 92.1 & 93.3 & 93.4 & \textbf{93.8} && \textbf{306.6} & 532.1 & 992.0 & 889.2 & 7571.6 \\
playground && 0.0 & 18.0 & 45.4 & \textbf{46.1} & 0.0 && 0.1 & 40.9 & \textbf{76.6} & 75.3 & 0.0 && 0.2 & 52.0 & \textbf{84.5} & 82.4 & 0.0 && \textbf{121.5} & 386.0 & 511.2 & 486.8 & 350.2 \\
terrains && 0.7 & 19.1 & 42.4 & 42.0 & \textbf{48.0} && 2.6 & 59.1 & 74.5 & 74.6 & \textbf{76.8} && 3.1 & 71.7 & 82.8 & 83.0 & \textbf{84.3} && \textbf{62.6} & 194.7 & 176.1 & 180.8 & 1333.9 \\
\midrule
\textit{Average} && 0.2 & 29.8 & 53.8 & \textbf{54.7} & 45.5 && 0.9 & 61.4 & 79.8 & \textbf{80.0} & 64.0 && 1.3 & 72.1 & \textbf{86.7} & \textbf{86.7} & 69.1 && \textbf{165.3} & 308.8 & 445.4 & 401.5 & 2857.0 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


\begin{table}[t]
    \centering
    \caption{New results -- ETH3D DSLR}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{AUC @ $1^\circ$} && \multicolumn{5}{c}{AUC @ $3^\circ$} && \multicolumn{5}{c}{AUC @ $5^\circ$} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} \\  \midrule
courtyard && 56.3 & \textbf{89.6} & 86.7 & 86.7 & 87.3 && 75.4 & \textbf{96.5} & 95.6 & 95.6 & 95.8 && 81.5 & \textbf{97.9} & 97.3 & 97.3 & 97.5 && 11.2 & \textbf{9.2} & 16.2 & 20.2 & 39.2 \\
delivery\_area && 91.4 & 89.5 & 92.2 & 92.2 & \textbf{92.3} && 97.1 & 96.5 & \textbf{97.4} & \textbf{97.4} & \textbf{97.4} && 98.3 & 97.9 & 98.4 & 98.5 & \textbf{98.5} && 235.7 & \textbf{3.4} & 8.0 & 9.3 & 26.4 \\
electro && 72.6 & 64.7 & 81.3 & \textbf{81.4} & 70.0 && 81.8 & 73.5 & \textbf{90.9} & \textbf{90.9} & 75.7 && 83.9 & 76.6 & \textbf{94.0} & 93.9 & 77.0 && 99.9 & \textbf{3.7} & 5.2 & 6.4 & 23.9 \\
facade && 89.4 & 90.0 & \textbf{90.6} & \textbf{90.6} & 90.3 && 96.4 & 96.6 & \textbf{96.8} & \textbf{96.8} & 96.7 && 97.8 & 98.0 & \textbf{98.1} & \textbf{98.1} & 98.0 && \textbf{35.1} & 37.1 & 57.7 & 68.3 & 113.5 \\
kicker && 82.0 & 79.2 & 86.0 & 86.0 & \textbf{86.6} && 89.6 & 86.0 & \textbf{95.2} & \textbf{95.2} & 91.2 && 91.2 & 88.5 & \textbf{97.1} & \textbf{97.1} & 92.2 && \textbf{1.6} & 2.3 & 3.7 & 4.3 & 16.2 \\
meadow && 10.5 & 26.1 & 76.4 & \textbf{78.5} & 61.6 && 13.8 & 36.7 & 90.7 & \textbf{91.7} & 77.8 && 14.7 & 40.6 & 94.4 & \textbf{95.0} & 81.5 && \textbf{0.2} & 0.7 & 0.7 & 0.8 & 5.1 \\
office && 19.3 & 40.3 & \textbf{59.3} & 58.6 & 45.2 && 24.1 & 53.5 & \textbf{81.5} & 81.0 & 56.5 && 25.6 & 59.1 & \textbf{88.3} & 87.9 & 59.9 && \textbf{0.4} & 0.5 & 0.8 & 0.8 & 19.1 \\
pipes && 29.4 & 76.6 & 88.9 & \textbf{89.1} & 86.3 && 36.3 & 91.6 & 96.3 & \textbf{96.4} & 95.4 && 41.1 & 95.0 & \textbf{97.8} & \textbf{97.8} & 97.3 && \textbf{0.3} & \textbf{0.4} & \textbf{0.4} & \textbf{0.5} & 3.4 \\
playground && 49.4 & 75.6 & \textbf{90.9} & \textbf{90.9} & 90.6 && 55.6 & 82.0 & \textbf{96.9} & \textbf{96.9} & 96.8 && 56.9 & 83.5 & \textbf{98.2} & \textbf{98.2} & 98.1 && 121.5 & \textbf{6.2} & 6.3 & 6.4 & 29.8 \\
relief && 89.8 & \textbf{93.4} & \textbf{93.3} & \textbf{93.4} & 93.3 && 96.6 & \textbf{97.8} & \textbf{97.8} & \textbf{97.8} & \textbf{97.8} && 98.0 & \textbf{98.7} & \textbf{98.7} & \textbf{98.7} & \textbf{98.7} && \textbf{3.7} & 5.6 & 10.9 & 12.8 & 34.1 \\
relief\_2 && 11.9 & 94.3 & 94.2 & 94.2 & \textbf{94.9} && 12.4 & 98.1 & 98.1 & 98.1 & \textbf{98.2} && 12.5 & \textbf{98.9} & 98.8 & 98.8 & \textbf{98.9} && \textbf{0.7} & 2.3 & 5.0 & 5.9 & 24.1 \\
terrace && 91.9 & 91.4 & 92.1 & 92.1 & \textbf{92.3} && 97.3 & 97.1 & \textbf{97.4} & \textbf{97.4} & \textbf{97.4} && 98.4 & 98.3 & 98.4 & 98.4 & \textbf{98.5} && \textbf{1.1} & 1.4 & 3.3 & 3.1 & 10.9 \\
terrains && 70.9 & 49.0 & \textbf{84.6} & 84.0 & 81.9 && 89.3 & 77.5 & \textbf{94.6} & 94.4 & 93.6 && 93.4 & 85.8 & \textbf{96.7} & 96.6 & 96.1 && 62.6 & \textbf{2.6} & 4.0 & 4.7 & 21.7 \\
botanical\_garden && 26.0 & 83.2 & \textbf{83.6} & 83.0 & 5.0 && 30.1 & 94.1 & \textbf{94.3} & 94.1 & 5.3 && 30.9 & 96.4 & \textbf{96.6} & 96.5 & 5.4 && \textbf{1.0} & 1.7 & 3.3 & 3.7 & 9.1 \\
boulders && 89.6 & 87.3 & 90.4 & 90.4 & \textbf{90.6} && 96.4 & 95.7 & 96.8 & 96.7 & \textbf{96.9} && 97.9 & 97.4 & 98.0 & 98.0 & \textbf{98.1} && 4.1 & \textbf{2.9} & 10.9 & 43.3 & 18.5 \\
bridge && 44.9 & 86.9 & 45.6 & 45.6 & \textbf{91.6} && 47.9 & 94.5 & 48.1 & 48.1 & \textbf{97.2} && 48.5 & 96.4 & 48.6 & 48.6 & \textbf{98.3} && 35.1 & \textbf{29.6} & 85.2 & 68.5 & 91.9 \\
door && 93.8 & 93.8 & 96.5 & 95.9 & \textbf{96.9} && 97.9 & 97.9 & 98.8 & 98.6 & \textbf{99.0} && 98.8 & 98.8 & 99.3 & 99.2 & \textbf{99.4} && 1.2 & \textbf{0.6} & 3.3 & 1.2 & 4.2 \\
exhibition\_hall && 11.0 & 32.4 & 19.8 & 19.8 & \textbf{85.4} && 15.2 & 38.6 & 22.9 & 22.9 & \textbf{94.3} && 16.4 & 40.2 & 23.8 & 23.8 & \textbf{96.5} && \textbf{20.6} & 71.8 & 107.8 & 89.7 & 72.0 \\
lecture\_room && 80.2 & 77.1 & \textbf{84.2} & 83.9 & 82.9 && 92.7 & 91.5 & \textbf{94.4} & 94.3 & 94.0 && 95.6 & 94.9 & \textbf{96.6} & \textbf{96.6} & 96.4 && 3.3 & \textbf{2.0} & 11.9 & 5.2 & 10.9 \\
living\_room && 88.0 & 85.1 & 87.7 & 87.8 & \textbf{88.3} && \textbf{95.8} & 94.6 & 95.7 & 95.7 & \textbf{95.8} && 97.4 & 96.8 & 97.4 & 97.4 & \textbf{97.5} && \textbf{9.4} & 13.3 & 30.3 & 22.1 & 49.1 \\
lounge && \textbf{34.1} & 30.2 & 33.1 & 33.1 & 33.9 && \textbf{35.4} & 34.1 & 35.0 & 35.0 & 35.3 && \textbf{35.6} & 34.8 & 35.4 & 35.4 & \textbf{35.6} && \textbf{0.4} & \textbf{0.4} & 0.6 & 0.6 & 1.8 \\
observatory && 58.4 & 63.8 & 64.7 & \textbf{64.9} & 64.4 && 83.7 & 86.3 & 86.7 & \textbf{86.8} & 86.5 && 89.9 & 91.7 & 91.9 & \textbf{92.0} & 91.8 && 5.8 & \textbf{3.4} & 25.8 & 12.2 & 24.4 \\
old\_computer && 23.3 & 49.0 & 50.7 & 50.7 & \textbf{78.7} && 41.5 & 59.6 & 58.4 & 58.4 & \textbf{90.2} && 48.4 & 61.9 & 60.1 & 60.1 & \textbf{92.7} && 5.9 & \textbf{2.4} & 11.4 & 5.8 & 19.6 \\
statue && 96.4 & \textbf{98.9} & \textbf{98.9} & \textbf{98.9} & 98.7 && 98.8 & \textbf{99.6} & \textbf{99.6} & \textbf{99.6} & \textbf{99.6} && 99.3 & \textbf{99.8} & \textbf{99.8} & \textbf{99.8} & 99.7 && \textbf{0.9} & 1.3 & 11.4 & 3.2 & 7.4 \\
terrace\_2 && 87.9 & 89.4 & \textbf{91.0} & \textbf{91.0} & 90.7 && 95.7 & 96.3 & \textbf{96.9} & \textbf{96.9} & 96.8 && 97.4 & 97.8 & \textbf{98.2} & \textbf{98.2} & 98.1 && \textbf{0.9} & \textbf{1.0} & 3.9 & 3.7 & 10.2 \\
\midrule
\textit{Average} && 59.9 & 73.5 & 78.5 & 78.5 & \textbf{79.2} && 67.9 & 82.7 & 86.3 & 86.3 & \textbf{86.5} && 70.0 & 85.0 & \textbf{88.1} & \textbf{88.1} & \textbf{88.1} && 26.5 & \textbf{8.2} & 17.1 & 16.1 & 27.5 \\

      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}

\begin{table}[t]
    \centering
    \caption{New results -- IMC}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{AUC @ $3^\circ$} && \multicolumn{5}{c}{AUC @ $5^\circ$} && \multicolumn{5}{c}{AUC @ $10^\circ$} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} \\  \midrule
bike && - & 37.9 & 65.8 & 54.3 & \textbf{77.9} && - & 47.5 & 74.3 & 67.5 & \textbf{86.7} && - & 67.7 & 80.7 & 77.3 & \textbf{93.4} && - & 2.0 & \textbf{0.9} & 1.0 & 1.1 \\
chairs && - & 16.4 & \textbf{22.0} & 10.3 & 0.8 && - & 20.3 & \textbf{27.4} & 12.9 & 0.8 && - & 26.1 & \textbf{34.4} & 16.5 & 0.8 && - & 2.8 & 1.6 & 1.6 & \textbf{0.6} \\
fountain && 22.1 & 90.6 & 89.3 & 87.2 & \textbf{91.3} && 24.2 & 94.3 & 93.6 & 92.3 & \textbf{94.8} && 25.7 & 97.2 & 96.8 & 96.1 & \textbf{97.4} && \textbf{0.8} & 2.2 & 1.8 & 1.6 & 5.9 \\
cyprus && 1.6 & 70.3 & \textbf{73.8} & 69.2 & 45.7 && 1.7 & 74.9 & \textbf{79.2} & 76.4 & 48.9 && 1.7 & 78.3 & \textbf{84.8} & 83.2 & 51.4 && \textbf{0.3} & 3.1 & 1.2 & 2.0 & 11.1 \\
dioscuri && 0.4 & 0.8 & 36.6 & 41.5 & \textbf{58.7} && 0.4 & 1.2 & 39.2 & 46.3 & \textbf{61.4} && 0.5 & 2.7 & 42.9 & 50.9 & \textbf{63.9} && 41.9 & \textbf{23.2} & 49.4 & 50.2 & 156.3 \\
wall && 57.1 & 91.6 & 22.3 & \textbf{96.2} & 88.6 && 73.9 & 95.0 & 35.0 & \textbf{97.7} & 93.2 && 87.0 & 97.5 & 59.1 & \textbf{98.8} & 96.6 && \textbf{23.8} & 35.4 & 196.5 & 52.3 & 63.5 \\
kyiv-puppet-theater && 0.7 & 4.0 & 4.1 & \textbf{5.1} & 0.3 && 0.7 & 4.7 & 5.2 & \textbf{6.5} & 0.3 && 0.9 & 6.4 & 6.6 & \textbf{9.5} & 0.3 && \textbf{0.3} & 2.0 & 0.8 & 0.7 & \textbf{0.3} \\
brandenburg\_gate && 21.4 & 1.8 & 51.6 & 53.0 & \textbf{70.1} && 35.0 & 4.6 & 62.0 & 63.2 & \textbf{77.2} && 53.6 & 12.5 & 73.4 & 74.1 & \textbf{83.9} && 1171.8 & \textbf{131.3} & 182.4 & 152.5 & 1472.1 \\
british\_museum && 18.5 & 18.1 & 43.9 & 44.9 & \textbf{61.6} && 32.0 & 29.6 & 57.2 & 58.6 & \textbf{72.7} && 51.3 & 46.9 & 73.3 & 74.5 & \textbf{83.9} && 78.1 & \textbf{44.5} & 49.6 & 54.8 & 318.0 \\
buckingham\_palace && 4.1 & 1.5 & 67.7 & 64.8 & \textbf{80.5} && 12.5 & 4.0 & 74.8 & 73.3 & \textbf{86.2} && 34.0 & 11.9 & 82.3 & 81.9 & \textbf{91.1} && 429.7 & \textbf{156.1} & 240.3 & 287.4 & 4948.2 \\
colosseum\_exterior && 37.3 & 3.0 & 41.7 & 72.9 & \textbf{80.7} && 52.8 & 6.3 & 61.5 & 80.3 & \textbf{86.1} && 69.2 & 13.5 & 77.9 & 87.3 & \textbf{90.8} && 542.8 & \textbf{331.3} & 429.9 & 419.5 & 3561.7 \\
grand\_place\_brussels && 18.3 & 8.9 & 62.7 & 62.0 & \textbf{68.7} && 32.4 & 15.1 & 72.2 & 71.7 & \textbf{76.6} && 50.5 & 33.5 & 81.3 & 81.1 & \textbf{84.2} && 124.2 & \textbf{71.6} & 94.7 & 116.9 & 520.3 \\
lincoln..\_statue && 1.0 & 7.7 & 63.2 & 63.5 & \textbf{67.2} && 4.4 & 17.0 & 68.4 & 68.7 & \textbf{71.5} && 23.8 & 33.1 & 73.4 & 73.5 & \textbf{75.3} && 99.9 & \textbf{44.3} & 50.9 & 56.3 & 362.3 \\
notre\_dame..\_facade && 32.5 & 1.2 & 59.7 & 59.9 & \textbf{69.1} && 43.0 & 4.5 & 65.2 & 65.6 & \textbf{72.5} && 55.2 & 14.6 & 70.6 & 70.9 & \textbf{75.5} && 2592.1 & \textbf{801.0} & 1723.6 & 2853.3 & 52135.4 \\
pantheon\_exterior && 49.6 & 51.4 & 66.2 & 60.5 & \textbf{79.4} && 62.3 & 63.1 & 74.2 & 69.9 & \textbf{83.5} && 74.4 & 74.6 & 81.9 & 78.8 & \textbf{87.2} && 285.7 & 208.7 & \textbf{174.7} & 274.5 & 1454.6 \\
piazza\_san\_marco && 2.6 & 6.2 & \textbf{68.7} & 67.9 & 58.0 && 6.4 & 16.0 & \textbf{78.9} & 77.9 & 71.0 && 23.7 & 40.7 & \textbf{88.2} & 86.6 & 83.7 && 16.7 & \textbf{12.5} & 22.7 & 34.8 & 74.2 \\
sacre\_coeur && 37.1 & 15.5 & 73.7 & 74.5 & \textbf{78.5} && 50.8 & 24.4 & 77.7 & 78.1 & \textbf{80.9} && 64.8 & 40.6 & 81.1 & 81.3 & \textbf{82.8} && 196.1 & \textbf{105.1} & 138.8 & 180.8 & 682.2 \\
sagrada\_familia && 30.3 & 47.4 & 53.1 & 51.1 & \textbf{54.3} && 39.2 & 52.7 & 57.4 & 56.1 & \textbf{58.9} && 48.9 & 57.7 & 61.7 & 60.9 & \textbf{62.9} && 42.6 & \textbf{37.5} & 53.5 & 82.8 & 237.0 \\
st\_pauls\_cathedral && 1.9 & 10.3 & 64.7 & 64.1 & \textbf{72.7} && 6.5 & 24.6 & 73.5 & 72.4 & \textbf{78.9} && 25.8 & 44.8 & 81.8 & 80.5 & \textbf{85.0} && 61.9 & \textbf{35.9} & 52.0 & 64.7 & 241.4 \\
st\_peters\_square && 31.1 & 6.2 & 66.4 & 65.8 & \textbf{83.6} && 46.0 & 12.4 & 74.7 & 74.3 & \textbf{87.8} && 64.0 & 24.8 & 83.0 & 82.8 & \textbf{91.6} && 961.0 & \textbf{374.9} & 505.6 & 407.8 & 6051.9 \\
taj\_mahal && 38.6 & 4.9 & 68.8 & 64.0 & \textbf{68.9} && 51.0 & 11.4 & 74.2 & 71.0 & \textbf{75.5} && 64.9 & 23.6 & 80.0 & 78.0 & \textbf{81.7} && 380.1 & \textbf{176.4} & 326.5 & 372.0 & 4528.9 \\
trevi\_fountain && 43.4 & 22.6 & 74.6 & 74.2 & \textbf{80.5} && 56.2 & 40.5 & 79.7 & 79.4 & \textbf{84.4} && 69.3 & 59.2 & 84.6 & 84.3 & \textbf{87.8} && 1202.9 & 689.5 & \textbf{569.5} & 684.9 & 12294.4 \\
\midrule
\textit{Average} && 22.5 & 23.6 & 56.4 & 59.4 & \textbf{65.3} && 31.6 & 30.2 & 63.9 & 66.4 & \textbf{70.4} && 44.5 & 41.3 & 71.8 & 73.1 & \textbf{75.1} && 412.6 & \textbf{149.6} & 221.2 & 279.7 & 4051.0 \\

      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}

\begin{table}[t]
    \centering
    \caption{New results -- SLAM}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{Recall @ 0.1m} && \multicolumn{5}{c}{AUC @ 0.1m} && \multicolumn{5}{c}{AUC @ 0.5m} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} \\  \midrule
cables && 76.8 & \textbf{88.0} & \textbf{88.0} & \textbf{88.0} & 68.0 && 59.1 & 53.6 & 77.0 & \textbf{77.7} & 56.5 && 77.4 & 81.1 & 85.8 & \textbf{85.9} & 70.4 && 103.1 & 170.9 & \textbf{68.5} & 75.0 & 2553.4 \\
camera && 2.2 & 33.0 & \textbf{47.1} & 46.1 & 34.8 && 2.0 & 15.7 & 32.5 & \textbf{33.4} & 24.7 && 2.2 & 35.4 & \textbf{44.9} & 44.2 & 33.2 && \textbf{1.5} & 24.6 & 11.5 & 10.8 & 196.2 \\
ceiling && 6.4 & 28.2 & \textbf{33.8} & 33.5 & 28.6 && 2.9 & 11.8 & 15.3 & \textbf{16.9} & 15.3 && 8.2 & 29.0 & 30.8 & \textbf{30.9} & 26.3 && 78.3 & 132.5 & \textbf{62.3} & 66.5 & 1057.7 \\
desk && 28.0 & 33.8 & 34.2 & \textbf{34.8} & 24.4 && 16.0 & 17.2 & \textbf{27.1} & 27.0 & 21.1 && 28.6 & 32.9 & \textbf{35.2} & 35.0 & 23.7 && 376.2 & 200.9 & \textbf{92.3} & 93.3 & 1115.1 \\
einstein && 32.9 & 41.3 & \textbf{43.2} & 43.0 & 33.6 && 22.7 & 29.2 & 33.6 & \textbf{35.7} & 25.4 && 34.2 & 42.4 & 42.8 & \textbf{43.6} & 36.7 && 150.3 & \textbf{61.2} & 61.5 & 65.0 & 1230.8 \\
kidnap && 73.1 & \textbf{73.3} & \textbf{73.3} & \textbf{73.3} & \textbf{73.3} && 63.4 & 59.8 & \textbf{69.5} & 67.8 & 68.5 && 71.2 & 70.6 & \textbf{72.5} & 72.2 & 72.3 && 114.4 & 668.8 & \textbf{64.0} & 69.3 & 731.2 \\
large && 35.4 & \textbf{47.6} & 37.3 & 37.3 & 44.8 && 18.1 & 20.2 & 31.7 & \textbf{33.6} & 20.8 && 33.7 & \textbf{43.4} & 36.8 & 36.7 & \textbf{43.4} && 91.9 & 113.0 & \textbf{42.1} & 47.3 & 983.8 \\
mannequin && 49.1 & 58.5 & 67.9 & \textbf{68.6} & 59.3 && 36.7 & 39.0 & 50.8 & 51.9 & \textbf{52.8} && 49.1 & 58.5 & \textbf{67.4} & 67.1 & 58.4 && 33.5 & 66.5 & \textbf{26.1} & 26.4 & 301.2 \\
motion && 18.8 & 14.1 & 23.1 & \textbf{31.7} & 17.7 && 11.0 & 7.7 & 10.3 & \textbf{15.9} & 12.9 && 23.3 & 13.7 & 28.2 & \textbf{46.7} & 19.7 && 859.7 & \textbf{84.8} & 291.4 & 343.4 & 9995.1 \\
planar && 30.6 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} && 12.5 & 94.4 & 97.6 & 97.7 & \textbf{98.3} && 38.0 & 98.9 & 99.5 & 99.5 & \textbf{99.7} && 313.8 & \textbf{154.8} & 228.5 & 269.5 & 2349.7 \\
plant && 77.0 & 87.0 & 90.4 & 89.4 & \textbf{92.8} && 62.9 & 71.4 & 75.1 & 76.3 & \textbf{82.3} && 77.1 & 89.4 & 92.0 & 91.0 & \textbf{92.5} && 21.7 & 48.8 & \textbf{19.9} & 21.6 & 202.7 \\
reflective && 12.6 & 16.2 & 18.8 & 21.5 & \textbf{26.2} && 6.7 & 4.8 & 7.0 & 7.7 & \textbf{9.2} && 16.5 & 20.0 & 24.9 & 29.6 & \textbf{33.5} && 721.3 & \textbf{104.7} & 171.6 & 182.8 & 6573.9 \\
repetitive && 26.3 & 28.7 & \textbf{33.3} & 32.9 & 28.5 && 23.9 & 14.1 & \textbf{27.3} & 25.1 & 27.2 && 25.8 & 26.8 & \textbf{32.1} & 31.4 & 28.3 && 63.2 & 106.4 & 53.0 & \textbf{47.8} & 561.1 \\
sfm && 83.2 & \textbf{90.4} & 90.1 & 89.8 & 55.8 && 57.9 & 46.0 & \textbf{62.7} & 60.0 & 36.4 && 80.0 & 86.3 & \textbf{89.5} & 88.8 & 55.9 && \textbf{91.7} & 158.7 & 207.7 & 202.2 & 469.6 \\
sofa && 11.2 & 18.6 & 24.2 & 24.5 & \textbf{32.2} && 5.5 & 10.7 & 14.0 & 16.1 & \textbf{28.6} && 10.3 & 18.3 & 23.0 & 23.4 & \textbf{31.6} && 9.1 & 9.9 & \textbf{8.2} & 8.8 & 157.3 \\
table && 79.1 & 83.9 & \textbf{99.9} & \textbf{99.9} & \textbf{99.9} && 68.2 & 57.8 & 74.8 & 78.1 & \textbf{95.6} && 76.9 & 81.9 & 94.9 & 95.5 & \textbf{99.1} && 182.0 & \textbf{61.2} & 89.9 & 86.6 & 2777.7 \\
vicon && 64.6 & 74.4 & 94.8 & \textbf{98.2} & 81.1 && 20.4 & 49.6 & 56.5 & \textbf{61.0} & 38.9 && 71.7 & 84.0 & 91.0 & \textbf{92.2} & 75.0 && 50.9 & 149.8 & \textbf{33.2} & 36.8 & 474.8 \\
\midrule
\textit{Average} && 48.2 & 60.1 & 65.5 & \textbf{65.7} & 57.9 && 34.9 & 40.6 & 50.1 & \textbf{51.2} & 47.7 && 48.6 & 60.0 & 64.8 & \textbf{65.2} & 57.9 && 120.8 & 97.7 & \textbf{70.2} & 73.7 & 1115.4 \\

      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}

\begin{table}[t]
    \centering
    \caption{New results -- LaMAR}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{Recall @ 1m} && \multicolumn{5}{c}{AUC @ 1m} && \multicolumn{5}{c}{AUC @ 5m} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} \\  \midrule
% submission\\
% CAB && - & 3.2 & 6.3 & \textbf{12.9} && - & 1.3 & 2.7 & \textbf{8.5} && - & 9.2 & 11.5 & \textbf{15.6} && - & \textbf{1453.5} & 3114.9 & 194033.6 \\
% HGE && - & 3.4 & 13.4 & \textbf{38.9} && - & 1.3 & 8.1 & \textbf{18.0} && - & 1.3 & 14.5 & \textbf{46.9} && - & \textbf{1829.7} & 2996.4 & 249771.1 \\
% LIN && - & 8.6 & 24.5 & \textbf{45.1} && - & 3.3 & 9.8 & \textbf{20.9} && - & 24.1 & 31.6 & \textbf{52.3} && - & \textbf{2783.3} & 7496.2 & 620176.4 \\
% \midrule
% new pipeline\\
CAB && - & 3.2 & 6.3 & 11.5 & \textbf{13.0} && - & 1.3 & 2.7 & \textbf{5.9} & 5.8 && - & 9.2 & 11.5 & 16.5 & \textbf{19.2} && - & \textbf{1453.5} & 3114.9 & 3696.4 & 194033.6 \\
HGE && - & 3.4 & 13.4 & 33.9 & \textbf{38.9} && - & 1.3 & 8.1 & \textbf{18.6} & 18.0 && - & 1.3 & 14.5 & 37.0 & \textbf{46.9} && - & \textbf{1829.7} & 2996.4 & 3974.0 & 249771.1 \\
LIN && - & 8.6 & 24.5 & \textbf{83.4} & 44.2 && - & 3.3 & 9.8 & \textbf{38.7} & 17.7 &&  - & 24.1 & 31.6 & \textbf{83.5} & 52.3 &&  - & \textbf{2783.3} & 7496.2 &  6994.4 & 620176.4 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


\begin{table}[t]
    \centering
    \caption{New results -- LaMAR}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c a l c c a l c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{3}{c}{PSNR \uparrow} && \multicolumn{3}{c}{SSIM \uparrow} && \multicolumn{3}{c}{LPIPS\downarrow} 
        \\
        \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13} 
        && \tiny{GLOMAP} & \tiny{GLOMAP (re)} & \tiny{COLMAP} && \tiny{GLOMAP} & \tiny{GLOMAP (re)} & \tiny{COLMAP}  && \tiny{GLOMAP} & \tiny{GLOMAP (re)} & \tiny{COLMAP} \\  \midrule
co3d\_bench && 32.91 & \textbf{33.62} & 19.16 && 0.924 & \textbf{0.934} & 0.618 && 0.056 & \textbf{0.047} & 0.357 \\
co3d\_hydrant && 29.71 & \textbf{30.76} & 30.65 && 0.884 & \textbf{0.905} & 0.903 && 0.087 & \textbf{0.064} & 0.066 \\
llff\_fern && 20.89 & \textbf{23.74} & 23.61 && 0.743 & \textbf{0.808} & 0.804 && 0.203 & \textbf{0.143} & 0.144 \\
llff\_flower && 21.68 & \textbf{28.69} & 28.40 && 0.728 & \textbf{0.868} & 0.864 && 0.210 & \textbf{0.103} & 0.105 \\
llff\_fortress && 27.83 & \textbf{29.27} & 29.13 && 0.853 & \textbf{0.866} & \textbf{0.866} && 0.108 & 0.085 & \textbf{0.084} \\
llff\_horns && 24.81 & 26.55 & \textbf{26.72} && 0.834 & \textbf{0.868} & \textbf{0.868} && 0.149 & 0.108 & \textbf{0.107} \\
llff\_orchids && 16.32 & 18.81 & \textbf{18.86} && 0.528 & 0.627 & \textbf{0.629} && 0.247 & 0.155 & \textbf{0.152} \\
llff\_room && 28.07 & 28.99 & \textbf{29.21} && 0.929 & \textbf{0.938} & 0.936 && 0.110 & 0.089 & \textbf{0.085} \\
llff\_trex && 24.86 & 26.50 & \textbf{26.62} && 0.883 & 0.905 & \textbf{0.907} && 0.097 & 0.072 & \textbf{0.070} \\
tandt\_barn && 24.84 & 25.15 & \textbf{26.53} && 0.822 & 0.825 & \textbf{0.866} && 0.175 & 0.173 & \textbf{0.109} \\
tandt\_caterpillar && 27.50 & 27.70 & \textbf{27.81} && 0.807 & 0.818 & \textbf{0.820} && 0.151 & 0.134 & \textbf{0.133} \\
tandt\_church && 28.13 & 27.92 & \textbf{28.26} && 0.865 & 0.859 & \textbf{0.869} && 0.102 & 0.118 & \textbf{0.098} \\
tandt\_courthouse && \textbf{27.84} & 27.55 & 27.36 && 0.914 & \textbf{0.916} & 0.915 && 0.063 & \textbf{0.060} & \textbf{0.060} \\
tandt\_family && 26.07 & \textbf{26.40} & \textbf{26.40} && 0.853 & \textbf{0.868} & \textbf{0.868} && 0.124 & 0.100 & \textbf{0.098} \\
tandt\_francis && 28.98 & 30.22 & \textbf{30.83} && 0.869 & 0.884 & \textbf{0.885} && 0.157 & 0.128 & \textbf{0.127} \\
tandt\_horse && 25.92 & 26.82 & \textbf{26.89} && 0.885 & \textbf{0.899} & \textbf{0.899} && 0.120 & 0.100 & \textbf{0.099} \\
tandt\_ignatius && 23.29 & 24.10 & \textbf{24.47} && 0.720 & 0.746 & \textbf{0.762} && 0.206 & 0.168 & \textbf{0.158} \\
tandt\_m60 && 24.40 & \textbf{25.02} & 21.48 && 0.828 & \textbf{0.847} & 0.807 && 0.181 & \textbf{0.156} & 0.218 \\
tandt\_museum && 24.18 & 24.29 & \textbf{27.58} && 0.765 & 0.776 & \textbf{0.845} && 0.204 & 0.179 & \textbf{0.101} \\
tandt\_panther && 26.14 & 26.76 & \textbf{26.90} && 0.856 & 0.870 & \textbf{0.871} && 0.147 & \textbf{0.127} & \textbf{0.127} \\
tandt\_playground && 24.03 & \textbf{24.23} & 23.08 && 0.721 & \textbf{0.736} & 0.725 && 0.239 & \textbf{0.204} & 0.234 \\
tandt\_train && 25.35 & 25.72 & \textbf{25.94} && 0.852 & \textbf{0.866} & 0.863 && 0.104 & \textbf{0.088} & 0.090 \\
tandt\_truck && 23.49 & 24.40 & \textbf{24.85} && 0.794 & 0.819 & \textbf{0.828} && 0.148 & 0.115 & \textbf{0.111} \\
mipnerf360\_bonsai && 31.22 & \textbf{31.74} & 31.45 && 0.936 & \textbf{0.942} & 0.937 && 0.065 & \textbf{0.061} & 0.063 \\
mipnerf360\_counter && 28.61 & \textbf{29.08} & 28.83 && 0.899 & \textbf{0.909} & 0.908 && 0.115 & \textbf{0.101} & \textbf{0.101} \\
mipnerf360\_kitchen && 28.42 & 30.20 & \textbf{30.82} && 0.928 & 0.943 & \textbf{0.944} && 0.058 & 0.044 & \textbf{0.043} \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


\begin{table}[t]
    \centering
    \caption{New results -- LaMAR}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c a l c c a l c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{3}{c}{PSNR \uparrow} && \multicolumn{3}{c}{SSIM \uparrow} && \multicolumn{3}{c}{LPIPS \downarrow} 
        \\
        \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13} 
        && \tiny{GLOMAP} & \tiny{GLOMAP (re)} & \tiny{COLMAP} && \tiny{GLOMAP} & \tiny{GLOMAP (re)} & \tiny{COLMAP}  && \tiny{GLOMAP} & \tiny{GLOMAP (re)} & \tiny{COLMAP} \\  \midrule
co3d && 31.31 & \textbf{32.19} & 24.91 && 0.904 & \textbf{0.920} & 0.760 && 0.072 & \textbf{0.055} & 0.211 \\
llff && 23.49 & \textbf{26.08} & \textbf{26.08} && 0.786 & \textbf{0.840} & 0.839 && 0.161 & 0.108 & \textbf{0.107} \\
tandt && 25.73 & 26.16 & \textbf{26.31} && 0.825 & 0.838 & \textbf{0.845} && 0.152 & 0.132 & \textbf{0.126} \\
mipnerf360 && 29.42 & 30.34 & \textbf{30.37} && 0.921 & \textbf{0.931} & 0.930 && 0.079 & \textbf{0.069} & \textbf{0.069} \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


\begin{table}[t]
    \centering
    \caption{New results -- LaMAR}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c l c c c c l c c c c
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{4}{c}{PSNR \uparrow} && \multicolumn{4}{c}{SSIM \uparrow} && \multicolumn{4}{c}{LPIPS \downarrow} 
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} 
        && \tiny{GLOMAP} & \tiny{COLMAP} & \tiny{COLMAP$^*$} & \tiny{FlowMap$^*$} && \tiny{GLOMAP} & \tiny{COLMAP} & \tiny{COLMAP$^*$} & \tiny{FlowMap$^*$ }&& \tiny{GLOMAP} & \tiny{COLMAP} & \tiny{COLMAP$^*$} & \tiny{FlowMap$^*$} \\  \midrule
co3d && \textbf{32.19} & 24.91 & 25.17 & 31.11 && \textbf{0.920} & 0.760 & 0.750 & 0.896 && \textbf{0.055} & 0.211 & 0.190 & 0.064 \\
llff && 26.08 & 26.08 & 25.73 & \textbf{27.23} && 0.840 & 0.839 & \textbf{0.851} & 0.849 && 0.108 & 0.107 & 0.098 & \textbf{0.079} \\
tandt && 26.16 & 26.31 & 26.74 & \textbf{27.00} && 0.838 & 0.845 & 0.848 & \textbf{0.854} && 0.132 & 0.126 & 0.130 & \textbf{0.101} \\
mipnerf360 && 30.34 & \textbf{30.37} & 29.95 & 29.84 && \textbf{0.931} & 0.930 & 0.928 & 0.916 && \textbf{0.069} & \textbf{0.069} & 0.074 & 0.073 \\

      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}

==> tex/tbl/postsubmission_draft.tex <==

\begin{table}[t]
    \centering
    \caption{Results on IMC 2023~\cite{IMC2023}. Our GLOMAP method comes close to COLMAP generated ground truth while outperforming global SfM by a large margin.}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c a l c c c a l c c c a l c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{4}{c}{AUC @ $3^\circ$} && \multicolumn{4}{c}{AUC @ $5^\circ$} && \multicolumn{4}{c}{AUC @ $10^\circ$} 
        && \multicolumn{4}{c}{Time (s)}
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
\textit{Fix rotation} \\
dioscuri && 0.0 & 0.3 & 40.3 & \textbf{58.6} && 0.0 & 0.7 & 44.1 & \textbf{61.3} && 0.1 & 2.2 & 47.8 & \textbf{63.8} && 41.9 & \textbf{23.2} & 100.0 & 156.2 \\
wall && 56.1 & 91.5 & \textbf{96.4} & 88.4 && 73.3 & 94.9 & \textbf{97.9} & 93.0 && 86.7 & 97.4 & \textbf{98.9} & 96.5 && \textbf{23.8} & 35.4 & 424.3 & 63.5 \\
meadow && 8.4 & 20.7 & \textbf{75.8} & 58.4 && 12.0 & 32.4 & \textbf{91.3} & 76.4 && 12.9 & 36.5 & \textbf{94.8} & 80.5 && \textbf{0.2} & 0.7 & 1.4 & 5.1 \\
\midrule
\textit{Full bundle} \\
dioscuri && 0.0 & 0.3 & 36.3 & \textbf{58.6} && 0.0 & 0.7 & 38.9 & \textbf{61.3} && 0.1 & 2.2 & 42.7 & \textbf{63.8} && 41.9 & \textbf{23.2} & 53.8 & 156.2 \\
wall && 56.1 & \textbf{91.5} & 20.5 & 88.4 && 73.3 & \textbf{94.9} & 33.5 & 93.0 && 86.7 & \textbf{97.4} & 58.1 & 96.5 && \textbf{23.8} & 35.4 & 198.2 & 63.5 \\
meadow && 8.4 & 20.7 & \textbf{74.8} & 58.4 && 12.0 & 32.4 & \textbf{90.5} & 76.4 && 12.9 & 36.5 & \textbf{94.3} & 80.5 && \textbf{0.2} & 0.7 & 1.1 & 5.1 \\
\midrule
\midrule
\textit{Fix rotation} \\
courtyard && 54.6 & \textbf{89.3} & 86.2 & 86.9 && 73.1 & \textbf{96.4} & 95.4 & 95.6 && 79.8 & \textbf{97.9} & 97.2 & 97.4 && 11.2 & \textbf{9.2} & 21.9 & 39.2 \\
delivery\_area && 91.2 & 89.2 & 92.1 & \textbf{92.2} && 97.1 & 96.4 & \textbf{97.4} & \textbf{97.4} && 98.2 & 97.8 & \textbf{98.4} & \textbf{98.5} && 235.7 & \textbf{3.4} & 16.4 & 26.4 \\
electro && 72.3 & 63.6 & \textbf{80.7} & 69.6 && 81.6 & 72.9 & \textbf{90.6} & 75.5 && 83.7 & 76.1 & \textbf{93.7} & 76.8 && 99.9 & \textbf{3.7} & 10.7 & 23.9 \\
facade && 89.2 & 89.8 & \textbf{90.4} & 90.1 && 96.3 & 96.6 & \textbf{96.8} & 96.7 && 97.8 & 98.0 & \textbf{98.1} & 98.0 && \textbf{35.1} & 37.1 & 102.5 & 113.5 \\
kicker && 81.3 & 78.4 & 85.5 & \textbf{86.2} && 89.3 & 85.5 & \textbf{95.1} & 91.1 && 91.0 & 88.2 & \textbf{97.0} & 92.1 && \textbf{1.6} & 2.3 & 5.1 & 16.2 \\
meadow && 8.4 & 20.7 & \textbf{75.8} & 58.4 && 12.0 & 32.4 & \textbf{91.3} & 76.4 && 12.9 & 36.5 & \textbf{94.8} & 80.5 && \textbf{0.2} & 0.7 & 1.4 & 5.1 \\
office && 17.9 & 37.3 & \textbf{56.7} & 43.6 && 22.9 & 51.5 & \textbf{80.4} & 55.5 && 24.5 & 57.4 & \textbf{87.7} & 59.1 && \textbf{0.4} & 0.5 & 1.1 & 19.1 \\
pipes && 26.4 & 74.8 & \textbf{88.5} & 85.9 && 34.6 & 91.1 & \textbf{96.2} & 95.3 && 39.6 & 94.7 & \textbf{97.7} & 97.2 && \textbf{0.3} & \textbf{0.4} & 0.6 & 3.4 \\
playground && 48.6 & 75.3 & \textbf{91.0} & 90.6 && 54.9 & 81.7 & \textbf{97.0} & 96.8 && 56.2 & 83.1 & \textbf{98.2} & 98.1 && 121.5 & \textbf{6.2} & 8.7 & 29.8 \\
relief && 89.3 & \textbf{92.8} & \textbf{92.8} & 92.7 && 96.4 & \textbf{97.6} & \textbf{97.6} & \textbf{97.6} && 97.9 & \textbf{98.6} & \textbf{98.6} & 98.5 && \textbf{3.7} & 5.6 & 13.8 & 34.1 \\
relief\_2 && 11.1 & 93.7 & 93.7 & \textbf{94.4} && 11.6 & 97.9 & 97.9 & \textbf{98.1} && 11.7 & 98.7 & 98.7 & \textbf{98.9} && \textbf{0.7} & 2.3 & 6.4 & 24.1 \\
terrace && 91.8 & 91.1 & 92.0 & \textbf{92.2} && 97.3 & 97.0 & 97.3 & \textbf{97.4} && \textbf{98.4} & 98.2 & \textbf{98.4} & \textbf{98.5} && \textbf{1.1} & 1.4 & 4.7 & 10.9 \\
terrains && 69.7 & 49.2 & \textbf{84.5} & 81.7 && 88.9 & 77.5 & \textbf{94.6} & 93.5 && 93.2 & 85.8 & \textbf{96.7} & 96.0 && 62.6 & \textbf{2.6} & 5.3 & 21.7 \\
botanical\_garden && 25.0 & 82.9 & \textbf{83.1} & 4.5 && 29.2 & 94.1 & \textbf{94.2} & 4.7 && 30.0 & 96.3 & \textbf{96.5} & 4.8 && \textbf{1.0} & 1.7 & 4.5 & 9.1 \\
boulders && 89.3 & 86.9 & 90.4 & \textbf{90.6} && 96.4 & 95.6 & 96.8 & \textbf{96.9} && 97.8 & 97.4 & \textbf{98.1} & \textbf{98.1} && 4.1 & \textbf{2.9} & 12.8 & 18.5 \\
bridge && 44.4 & 86.7 & 45.0 & \textbf{91.4} && 47.4 & 94.4 & 47.6 & \textbf{97.1} && 48.0 & 96.3 & 48.1 & \textbf{98.3} && 35.1 & \textbf{29.6} & 64.0 & 91.9 \\
door && 93.6 & 93.6 & 95.8 & \textbf{96.5} && 97.8 & 97.9 & 98.6 & \textbf{98.8} && 98.7 & 98.7 & 99.2 & \textbf{99.3} && 1.2 & \textbf{0.6} & 2.1 & 4.2 \\
exhibition\_hall && 10.2 & 31.4 & 18.7 & \textbf{85.4} && 14.3 & 37.7 & 21.8 & \textbf{94.3} && 15.5 & 39.3 & 22.6 & \textbf{96.5} && \textbf{20.6} & 71.8 & 157.7 & 72.0 \\
lecture\_room && 79.9 & 76.4 & \textbf{84.1} & 82.7 && 92.6 & 91.3 & \textbf{94.4} & 94.0 && 95.6 & 94.8 & \textbf{96.7} & 96.4 && 3.3 & \textbf{2.0} & 6.5 & 10.9 \\
living\_room && 87.7 & 84.5 & 87.4 & \textbf{88.0} && 95.7 & 94.5 & 95.6 & \textbf{95.8} && \textbf{97.4} & 96.7 & 97.3 & \textbf{97.4} && \textbf{9.4} & 13.3 & 19.4 & 49.1 \\
lounge && \textbf{31.6} & 26.8 & 30.6 & 31.3 && \textbf{32.7} & 31.1 & 32.4 & \textbf{32.7} && \textbf{33.0} & 32.0 & 32.8 & 32.9 && \textbf{0.4} & \textbf{0.4} & 1.0 & 1.8 \\
observatory && 56.0 & 61.5 & \textbf{63.1} & 62.8 && 82.8 & 85.6 & \textbf{86.1} & 85.9 && 89.5 & 91.3 & \textbf{91.6} & 91.5 && 5.8 & \textbf{3.4} & 14.2 & 24.4 \\
old\_computer && 22.0 & 48.2 & 49.7 & \textbf{78.0} && 40.4 & 58.9 & 57.7 & \textbf{90.0} && 47.5 & 61.2 & 59.4 & \textbf{92.5} && 5.9 & \textbf{2.4} & 7.8 & 19.6 \\
statue && 96.1 & 98.7 & \textbf{98.8} & 98.6 && 98.7 & \textbf{99.6} & \textbf{99.6} & 99.5 && 99.2 & 99.7 & \textbf{99.8} & 99.7 && \textbf{0.9} & 1.4 & 3.8 & 7.4 \\
terrace\_2 && 87.1 & 88.8 & \textbf{90.5} & 90.2 && 95.5 & 96.2 & \textbf{96.8} & 96.7 && 97.3 & 97.7 & \textbf{98.1} & 98.0 && \textbf{0.9} & \textbf{1.0} & 4.2 & 10.2 \\
\midrule
\textit{Average} && 59.0 & 72.5 & 77.9 & \textbf{78.6} && 67.2 & 82.1 & 86.0 & \textbf{86.1} && 69.4 & 84.5 & \textbf{87.8} & \textbf{87.8} && 26.5 & \textbf{8.2} & 19.9 & 27.5 \\
\midrule
cables && 76.8 & \textbf{88.0} & \textbf{88.0} & 67.7 && 56.0 & 53.9 & \textbf{77.2} & 56.4 && 76.7 & 81.2 & \textbf{85.8} & 69.7 && 103.1 & 170.9 & 38.1 & \textbf{0.0} \\
camera && 2.2 & 33.1 & \textbf{47.1} & 34.7 && 2.0 & 15.1 & \textbf{33.9} & 25.7 && 2.2 & 35.2 & \textbf{45.1} & 33.2 && 1.5 & 24.6 & 33.1 & \textbf{0.0} \\
ceiling && 6.1 & 28.5 & \textbf{33.4} & 28.6 && 3.5 & 12.4 & 14.5 & \textbf{17.9} && 8.0 & 29.2 & \textbf{31.9} & 26.8 && 78.3 & 132.5 & 126.3 & \textbf{0.0} \\
desk && 27.9 & \textbf{33.8} & 33.0 & 24.4 && 16.9 & 16.8 & \textbf{27.7} & 20.8 && 28.6 & 32.8 & \textbf{34.7} & 23.7 && 376.2 & 200.9 & 149.9 & \textbf{0.0} \\
einstein && 32.7 & 41.3 & \textbf{42.3} & 33.7 && 23.3 & 29.1 & \textbf{35.1} & 25.6 && 34.3 & 42.3 & \textbf{43.3} & 36.9 && 150.3 & 61.2 & 58.1 & \textbf{0.0} \\
kidnap && 73.1 & \textbf{73.3} & \textbf{73.3} & \textbf{73.3} && 63.4 & 59.8 & 68.1 & \textbf{68.5} && 71.2 & 70.6 & 72.2 & \textbf{72.3} && 114.4 & 668.8 & 45.0 & \textbf{0.0} \\
large && 35.6 & 47.3 & \textbf{49.3} & 44.5 && 17.4 & 20.2 & \textbf{32.2} & 21.2 && 34.0 & 43.4 & \textbf{45.9} & 43.5 && 91.9 & 113.0 & 54.1 & \textbf{0.0} \\
mannequin && 49.0 & 58.5 & \textbf{70.6} & 59.3 && 36.9 & 38.8 & 52.6 & \textbf{52.8} && 49.1 & 58.4 & \textbf{68.0} & 58.4 && 33.5 & 66.5 & 24.4 & \textbf{0.0} \\
motion && 18.4 & 14.1 & \textbf{20.6} & 18.2 && \textbf{11.8} & 7.1 & 10.6 & \textbf{11.8} && 23.4 & 13.7 & \textbf{30.2} & 19.4 && 859.7 & 84.8 & 655.1 & \textbf{0.0} \\
planar && 30.4 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} && 13.3 & 94.4 & 97.6 & \textbf{98.3} && 44.8 & 98.9 & 99.5 & \textbf{99.7} && 313.8 & 154.8 & 119.9 & \textbf{0.0} \\
plant && 76.9 & 86.9 & 86.9 & \textbf{93.1} && 62.5 & 71.3 & 73.6 & \textbf{81.7} && 76.8 & 89.3 & 90.2 & \textbf{92.4} && 21.7 & 48.8 & 23.1 & \textbf{0.0} \\
reflective && 13.5 & 14.2 & 15.5 & \textbf{25.8} && 4.3 & 7.6 & 5.3 & \textbf{9.5} && 20.2 & 21.6 & 24.3 & \textbf{33.5} && 721.3 & 104.7 & 221.7 & \textbf{0.0} \\
repetitive && 26.3 & 28.7 & \textbf{33.3} & 28.5 && 23.9 & 17.0 & 27.1 & \textbf{27.2} && 25.8 & 27.4 & \textbf{32.1} & 28.3 && 63.2 & 106.4 & 29.3 & \textbf{0.0} \\
sfm && 83.4 & \textbf{90.3} & 89.8 & 55.9 && 57.2 & 48.0 & \textbf{64.5} & 37.3 && 79.8 & 86.7 & \textbf{90.0} & 56.3 && 91.7 & 158.7 & 19.9 & \textbf{0.0} \\
sofa && 11.2 & 18.6 & 24.3 & \textbf{32.2} && 5.5 & 11.4 & 14.4 & \textbf{28.6} && 10.3 & 18.4 & 23.1 & \textbf{31.6} && 9.1 & 9.9 & 11.4 & \textbf{0.0} \\
table && 79.1 & 83.8 & 99.0 & \textbf{99.9} && 68.2 & 58.4 & 70.2 & \textbf{95.6} && 76.9 & 82.0 & 93.9 & \textbf{99.1} && 182.0 & 61.2 & 108.5 & \textbf{0.0} \\
vicon && 63.0 & 73.3 & \textbf{91.1} & 81.2 && 23.6 & 51.9 & \textbf{65.0} & 34.4 && 72.3 & 84.4 & \textbf{92.0} & 74.2 && 50.9 & 149.8 & 40.5 & \textbf{0.0} \\
\midrule
\textit{Average} && 48.1 & 60.0 & \textbf{65.1} & 58.0 && 34.9 & 41.0 & \textbf{50.6} & 47.7 && 48.8 & 60.1 & \textbf{65.0} & 57.9 && 120.8 & 97.7 & 61.3 & \textbf{0.0} \\
\midrule
\textit{consistency check}\\
cables && 76.8 & \textbf{88.0} & 87.8 & 68.0 && 59.1 & 53.6 & \textbf{76.7} & 56.6 && 77.4 & 81.1 & \textbf{85.7} & 69.9 && 103.1 & 170.9 & 38.1 & \textbf{0.0} \\
camera && 2.2 & 33.0 & \textbf{46.2} & 34.8 && 2.0 & 15.7 & \textbf{25.5} & 24.6 && 2.2 & 35.4 & \textbf{43.1} & 33.0 && 1.5 & 24.6 & 33.1 & \textbf{0.0} \\
ceiling && 6.4 & 28.2 & \textbf{33.6} & 28.6 && 2.9 & 11.8 & \textbf{17.5} & 17.4 && 8.2 & 29.0 & \textbf{31.2} & 26.7 && 78.3 & 132.5 & 126.3 & \textbf{0.0} \\
desk && 28.0 & 33.8 & \textbf{33.9} & 24.4 && 16.0 & 17.2 & \textbf{23.4} & 21.0 && 28.6 & 32.9 & \textbf{34.8} & 23.7 && 376.2 & 200.9 & 149.9 & \textbf{0.0} \\
einstein && 32.9 & 41.3 & \textbf{48.6} & 33.7 && 22.7 & 29.2 & \textbf{34.0} & 25.4 && 34.2 & 42.4 & \textbf{46.8} & 36.9 && 150.3 & 61.2 & 58.1 & \textbf{0.0} \\
kidnap && 73.1 & \textbf{73.3} & \textbf{73.3} & \textbf{73.3} && 63.4 & 59.8 & 64.9 & \textbf{68.5} && 71.2 & 70.6 & 71.6 & \textbf{72.3} && 114.4 & 668.8 & 45.0 & \textbf{0.0} \\
large && 35.4 & \textbf{47.6} & 37.1 & 45.1 && 18.1 & 20.2 & \textbf{28.4} & 18.9 && 33.7 & \textbf{43.4} & 35.4 & 43.0 && 91.9 & 113.0 & 54.1 & \textbf{0.0} \\
mannequin && 49.1 & 58.5 & \textbf{65.9} & 59.3 && 36.7 & 39.0 & 40.5 & \textbf{52.4} && 49.1 & 58.5 & \textbf{64.6} & 58.3 && 33.5 & 66.5 & 24.4 & \textbf{0.0} \\
motion && 18.8 & 14.1 & \textbf{33.4} & 18.1 && 11.0 & 7.7 & \textbf{15.4} & 12.5 && 23.3 & 13.7 & \textbf{44.6} & 19.6 && 859.7 & 84.8 & 655.1 & \textbf{0.0} \\
planar && 30.6 & \textbf{100.0} & \textbf{100.0} & \textbf{100.0} && 12.5 & 94.4 & 97.8 & \textbf{98.3} && 38.0 & 98.9 & 99.6 & \textbf{99.7} && 313.8 & 154.8 & 119.9 & \textbf{0.0} \\
plant && 77.0 & 87.0 & 85.2 & \textbf{92.8} && 62.9 & 71.4 & 72.3 & \textbf{81.9} && 77.1 & 89.4 & 85.8 & \textbf{92.5} && 21.7 & 48.8 & 23.1 & \textbf{0.0} \\
reflective && 12.6 & 16.2 & 20.4 & \textbf{25.7} && 6.7 & 4.8 & 6.9 & \textbf{8.9} && 16.5 & 20.0 & 25.7 & \textbf{33.6} && 721.3 & 104.7 & 221.7 & \textbf{0.0} \\
repetitive && 26.3 & 28.7 & \textbf{31.0} & 28.5 && 23.9 & 14.1 & 19.7 & \textbf{27.2} && 25.8 & 26.8 & \textbf{30.3} & 28.3 && 63.2 & 106.4 & 29.3 & \textbf{0.0} \\
sfm && 83.2 & \textbf{90.4} & 90.2 & 56.0 && 57.9 & 46.0 & \textbf{64.4} & 35.3 && 80.0 & 86.3 & \textbf{90.2} & 56.0 && 91.7 & 158.7 & 19.9 & \textbf{0.0} \\
sofa && 11.2 & 18.6 & 20.4 & \textbf{32.2} && 5.5 & 10.7 & 9.3 & \textbf{28.6} && 10.3 & 18.3 & 21.3 & \textbf{31.6} && 9.1 & 9.9 & 11.4 & \textbf{0.0} \\
table && 79.1 & 83.9 & 94.9 & \textbf{99.9} && 68.2 & 57.8 & 70.3 & \textbf{95.6} && 76.9 & 81.9 & 92.7 & \textbf{99.1} && 182.0 & 61.2 & 108.5 & \textbf{0.0} \\
vicon && 64.6 & 74.4 & \textbf{91.6} & 79.9 && 20.4 & 49.6 & \textbf{60.9} & 48.3 && 71.7 & 84.0 & \textbf{91.3} & 77.1 && 50.9 & 149.8 & 40.5 & \textbf{0.0} \\
\midrule
\textit{Average} && 48.2 & 60.1 & \textbf{64.5} & 57.9 && 34.9 & 40.6 & 47.1 & \textbf{47.9} && 48.6 & 60.0 & \textbf{63.9} & 57.9 && 120.8 & 97.7 & 61.3 & \textbf{0.0} \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


==> tex/tbl/rebuttal_table.tex <==

% \begin{table}[h]
%     \centering
%     \vspace{-5px}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l l c c l c c l c c l c c
%     } \toprule 
%         && \multicolumn{2}{c}{Metric 1} && \multicolumn{2}{c}{Metric 2} && \multicolumn{2}{c}{Metric 3} 
%         && \multicolumn{2}{c}{Time (s)}
%         \\
%         \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
%         && LiGT & GLOMAP && LiGT & GLOMAP && LiGT & GLOMAP && LiGT & GLOMAP\\  \midrule
%         MIP360 && 43.8 & \textbf{93.6} && 49.3 & \textbf{96.1} && 57.1 & \textbf{98.0} && \textbf{107.1} & 149.8 \\
%         IMC2023 && 11.0 & \textbf{55.7} && 17.7 & \textbf{63.3} && 29.3 & \textbf{71.3} && 438.7 & \textbf{221.2} \\
%         ETH3D (DSLR) && 49.5 & \textbf{77.9} && 55.8 & \textbf{85.9} && 57.4 & \textbf{87.8} && 18.8 & \textbf{17.1} \\
%         ETH3D (SLAM) && 39.8 & \textbf{65.5} && 32.5 & \textbf{49.6} && 39.1 & \textbf{64.8} && 77.8 & \textbf{70.2} \\
%         ETH3D (Rig) && 2.7 & \textbf{99.4} && 1.5 & \textbf{81.3} && 3.0 & \textbf{95.9} && \textbf{127.1} & 445.4 \\
%         LaMAR && - & \textbf{14.7} && - & \textbf{6.9} && - & \textbf{19.2} && - & \textbf{4535.8} \\
%       \bottomrule
%     \end{tabular}
%     }
%     \vspace{-5px}
%     \caption{Average esults for datasets used in the paper.
%     % Here, meterics are kept the same as in the paper, and average results are reported.
%     }
%     \label{tbl:rebuttal_full}
% \end{table}

\begin{table}[h]
    \centering
    \vspace{-5px}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l l c c l c c l c c l c c
    } \toprule 
        && LiGT & GLOMAP && LiGT & GLOMAP && LiGT & GLOMAP && LiGT & GLOMAP\\
        \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
        && \multicolumn{2}{c}{AUC@$3^\circ$} && \multicolumn{2}{c}{AUC@$5^\circ$} && \multicolumn{2}{c}{AUC@$10^\circ$} 
        && \multicolumn{2}{c}{Time (s)}
        \\
         \midrule
        MIP360 && 43.8 & \textbf{93.6} && 49.3 & \textbf{96.1} && 57.1 & \textbf{98.0} && \textbf{107.1} & 149.8 \\
        IMC2023 && 11.0 & \textbf{55.7} && 17.7 & \textbf{63.3} && 29.3 & \textbf{71.3} && 438.7 & \textbf{221.2} \\  \midrule
        && \multicolumn{2}{c}{AUC@$1^\circ$} && \multicolumn{2}{c}{AUC@$3^\circ$} && \multicolumn{2}{c}{AUC@$5^\circ$} 
        && \multicolumn{2}{c}{Time (s)}
        \\
        \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
        ETH3D (DSLR) && 49.5 & \textbf{77.9} && 55.8 & \textbf{85.9} && 57.4 & \textbf{87.8} && 18.8 & \textbf{17.1} \\  \midrule
        && \multicolumn{2}{c}{Recall@$0.1m$} && \multicolumn{2}{c}{AUC@$0.1m$} && \multicolumn{2}{c}{AUC@$0.5m$} 
        && \multicolumn{2}{c}{Time (s)}
        \\
        \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
        ETH3D (SLAM) && 39.8 & \textbf{65.5} && 32.5 & \textbf{49.6} && 39.1 & \textbf{64.8} && 77.8 & \textbf{70.2} \\
        ETH3D (Rig) && 2.7 & \textbf{99.4} && 1.5 & \textbf{81.3} && 3.0 & \textbf{95.9} && \textbf{127.1} & 445.4 \\ 
        % \midrule
        % && \multicolumn{2}{c}{Recall@$1m$} && \multicolumn{2}{c}{AUC@$1m$} && \multicolumn{2}{c}{AUC@$5m$} 
        % && \multicolumn{2}{c}{Time (s)}
        % \\
        % \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13}
        % LaMAR && - & \textbf{14.7} && - & \textbf{6.9} && - & \textbf{19.2} && - & \textbf{4535.8} \\
      \bottomrule
    \end{tabular}
    }
    \vspace{-10px}
    \caption{Average results for datasets used in the paper.
    % Here, meterics are kept the same as in the paper, and average results are reported.
    }
    \label{tbl:rebuttal_full}
\end{table}

\begin{table}[h]
    \centering
    \vspace{-20px}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l l c c c c c c
    } \toprule 
        && Herz-Jesus-P8 & Herz-Jesus-P25 & Fountain-P11 & Entry-P10 & Castle-P19 & Castle-P30 \\\midrule
        LiGT$^*$ && 5.01 & 6.86 & 3.17 & \textbf{5.50} & 41.88 & 49.84 \\
        LiGT && \textbf{3.54} & \textbf{5.29} & \textbf{2.81} & 9.08 & \textbf{24.72} & 36.36 \\
        GLOMAP && 3.86 & 5.40 & \textbf{2.81} & 6.34 & 28.69 & \textbf{22.52} \\
      \bottomrule
    \end{tabular}
    }
    \vspace{-10px}
    \caption{Average camera position errors for Strecha dataset. Rows with $^*$ are taken from the paper [AA].}
    \label{tbl:rebuttal_strecha}
\vspace{-10px}
\end{table}

==> tex/tbl/refactored.tex <==

\begin{table}[t]
    \centering
    \caption{LaMAR}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c a l c c c a l c c c a l c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        % && \multicolumn{3}{c}{Thres 5m} && \multicolumn{3}{c}{AUC @ 5} && \multicolumn{3}{c}{AUC @ 10} 
        && \multicolumn{4}{c}{Recall @ 1m} && \multicolumn{4}{c}{AUC @ 1m} && \multicolumn{4}{c}{AUC @ 5m} 
        && \multicolumn{4}{c}{Time (s)}
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21}
        && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} &&  \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
CAB && - & 3.2 & \cellcolor{tabsecond}11.6 & \cellcolor{tabfirst}13.0 && - & 1.3 & \cellcolor{tabsecond} 4.7 & \cellcolor{tabfirst} 5.8 && - & 9.2 & \cellcolor{tabsecond}16.9 & \cellcolor{tabfirst}19.2 && - & \cellcolor{tabfirst}1453.5 &\cellcolor{tabsecond} 6162.24 & 194033.6 \\
HGE && - & 3.4 & \cellcolor{tabfirst}48.4 & \cellcolor{tabsecond}38.9 && - & 1.3 & \cellcolor{tabfirst}22.2 & \cellcolor{tabsecond}18.0 && - & 1.3 & \cellcolor{tabfirst}50.3 & \cellcolor{tabsecond}46.9 && - & \cellcolor{tabfirst}1829.7 & \cellcolor{tabsecond}12587.2 & 249771.1 \\
LIN$^*$ && - & 8.6 & \cellcolor{tabfirst}87.3 & \cellcolor{tabsecond}44.2 && - & 3.3 & \cellcolor{tabfirst}46.7 & \cellcolor{tabsecond}17.7 &&  - & 24.1 & \cellcolor{tabfirst}85.6 & \cellcolor{tabsecond}52.3 &&  - & \cellcolor{tabfirst}2783.3 & \cellcolor{tabsecond}17182.9 & 620176.4 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}

\begin{table}[t]
    \centering
    \caption{Mip360}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c a l c c c a l c c c a l c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{4}{c}{AUC @ $3^\circ$} && \multicolumn{4}{c}{AUC @ $5^\circ$} && \multicolumn{4}{c}{AUC @ $10^\circ$} 
        && \multicolumn{4}{c}{Time (s)}
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21}
        && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} &&  \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
bicycle && \cellcolor{tabsecond}89.2 & 70.7 & \cellcolor{tabfirst}95.8 & \cellcolor{tabfirst}95.8 && \cellcolor{tabsecond}92.7 & 81.0 & \cellcolor{tabfirst}97.5 & \cellcolor{tabfirst}97.5 && \cellcolor{tabsecond}95.3 & 89.4 & \cellcolor{tabfirst}98.7 & \cellcolor{tabfirst}98.7 && 123.1 & \cellcolor{tabfirst}34.5 & \cellcolor{tabsecond}60.6 & 120.6 \\
bonsai && 9.4 & 48.4 & \cellcolor{tabfirst}98.5 & \cellcolor{tabsecond}92.6 && 27.9 & 50.3 & \cellcolor{tabfirst}99.1 & \cellcolor{tabsecond}95.6 && 61.2 & 66.9 & \cellcolor{tabfirst}99.6 & \cellcolor{tabsecond}97.8 && \cellcolor{tabfirst}176.0 & \cellcolor{tabsecond}218.0 & 463.5 & 662.5 \\
counter && 96.9 & 99.0 & \cellcolor{tabfirst}99.3 & \cellcolor{tabsecond}99.2 && 98.1 & 99.4 & \cellcolor{tabfirst}99.6 & \cellcolor{tabsecond}99.5 && 99.1 & \cellcolor{tabsecond}99.7 & \cellcolor{tabfirst}99.8 & \cellcolor{tabfirst}99.8 && \cellcolor{tabfirst}46.6 & \cellcolor{tabsecond}79.5 & 206.7 & 270.5 \\
garden && \cellcolor{tabsecond}95.0 & 0.5 & \cellcolor{tabfirst}97.3 & \cellcolor{tabfirst}97.3 && \cellcolor{tabsecond}97.0 & 0.7 & \cellcolor{tabfirst}98.4 & \cellcolor{tabfirst}98.4 && \cellcolor{tabsecond}98.5 & 2.2 & \cellcolor{tabfirst}99.2 & \cellcolor{tabfirst}99.2 && \cellcolor{tabsecond}40.2 & \cellcolor{tabfirst}36.2 & 135.6 & 291.8 \\
kitchen && 88.5 & 92.0 & \cellcolor{tabsecond}94.8 & \cellcolor{tabfirst}94.9 && 93.1 & 95.2 & \cellcolor{tabsecond}96.9 & \cellcolor{tabfirst}97.0 && 96.5 & 97.6 & \cellcolor{tabsecond}98.4 & \cellcolor{tabfirst}98.5 && \cellcolor{tabfirst}127.0 & \cellcolor{tabsecond}146.8 & 435.0 & 619.1 \\
room && 39.6 & 32.6 & \cellcolor{tabfirst}97.8 & \cellcolor{tabsecond}96.2 && 42.2 & 33.8 & \cellcolor{tabfirst}98.7 & \cellcolor{tabsecond}97.7 && 44.9 & 35.7 & \cellcolor{tabfirst}99.3 & \cellcolor{tabsecond}98.9 && \cellcolor{tabsecond}96.3 & \cellcolor{tabfirst}80.2 & 226.9 & 371.6 \\
stump && \cellcolor{tabsecond}95.3 & 3.5 & \cellcolor{tabfirst}99.1 & \cellcolor{tabfirst}99.1 && \cellcolor{tabsecond}97.1 & 5.7 & \cellcolor{tabfirst}99.5 & \cellcolor{tabfirst}99.5 && \cellcolor{tabsecond}98.5 & 16.8 & \cellcolor{tabfirst}99.7 & \cellcolor{tabfirst}99.7 && 38.7 & \cellcolor{tabfirst}15.5 & \cellcolor{tabsecond}26.7 & 83.9 \\
\midrule
\textit{Average} && 73.4 & 49.5 & \cellcolor{tabfirst}97.5 & \cellcolor{tabsecond}96.5 && 78.3 & 52.3 & \cellcolor{tabfirst}98.5 & \cellcolor{tabsecond}97.9 && 84.9 & 58.3 & \cellcolor{tabfirst}99.3 & \cellcolor{tabsecond}98.9 && \cellcolor{tabsecond}92.6 & \cellcolor{tabfirst}87.2 & 222.2 & 345.7 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


\begin{table}[t]
    \centering
    \caption{ETH3D DSLR}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c a l c c c a l c c c a l c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{4}{c}{AUC @ $1^\circ$} && \multicolumn{4}{c}{AUC @ $3^\circ$} && \multicolumn{4}{c}{AUC @ $5^\circ$} 
        && \multicolumn{4}{c}{Time (s)}
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21}
        && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} &&  \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
courtyard && 68.2 & \cellcolor{tabfirst}89.6 & \cellcolor{tabsecond}87.7 & 87.3 && 81.7 & \cellcolor{tabfirst}96.5 & \cellcolor{tabsecond}95.9 & 95.8 && 85.9 & \cellcolor{tabfirst}97.9 & \cellcolor{tabsecond}97.5 & \cellcolor{tabsecond}97.5 && \cellcolor{tabsecond}11.2 & \cellcolor{tabfirst}9.2 & 22.5 & 39.2 \\
delivery\_area && 91.4 & 89.5 & \cellcolor{tabfirst}92.8 & \cellcolor{tabsecond}92.3 && 97.1 & 96.5 & \cellcolor{tabfirst}97.6 & \cellcolor{tabsecond}97.4 && 98.3 & 97.9 & \cellcolor{tabfirst}98.6 & \cellcolor{tabsecond}98.5 && 235.7 & \cellcolor{tabfirst}3.3 & \cellcolor{tabsecond}12.3 & 26.4 \\
electro && \cellcolor{tabsecond}72.6 & 64.7 & \cellcolor{tabfirst}79.3 & 70.0 && \cellcolor{tabsecond}81.8 & 73.5 & \cellcolor{tabfirst}86.7 & 75.7 && \cellcolor{tabsecond}83.9 & 76.6 & \cellcolor{tabfirst}88.5 & 77.0 && 99.9 & \cellcolor{tabfirst}3.6 & \cellcolor{tabsecond}7.4 & 23.9 \\
facade && 89.4 & 90.0 & \cellcolor{tabfirst}91.1 & \cellcolor{tabsecond}90.3 && 96.4 & 96.6 & \cellcolor{tabfirst}97.0 & \cellcolor{tabsecond}96.7 && 97.8 & \cellcolor{tabsecond}98.0 & \cellcolor{tabfirst}98.2 & \cellcolor{tabsecond}98.0 && \cellcolor{tabsecond}35.1 & \cellcolor{tabfirst}33.0 & 80.2 & 113.5 \\
kicker && 82.0 & 79.2 & \cellcolor{tabsecond}86.3 & \cellcolor{tabfirst}86.6 && 89.6 & 86.0 & \cellcolor{tabfirst}94.3 & \cellcolor{tabsecond}91.3 && 91.2 & 88.5 & \cellcolor{tabfirst}96.5 & \cellcolor{tabsecond}92.2 && \cellcolor{tabfirst}1.7 & \cellcolor{tabsecond}2.2 & 6.7 & 16.2 \\
meadow && 10.5 & 26.1 & \cellcolor{tabfirst}74.7 & \cellcolor{tabsecond}61.6 && 13.8 & 36.7 & \cellcolor{tabfirst}90.4 & \cellcolor{tabsecond}77.8 && 14.7 & 40.6 & \cellcolor{tabfirst}94.2 & \cellcolor{tabsecond}81.5 && \cellcolor{tabfirst}0.3 & \cellcolor{tabsecond}1.0 & 2.1 & 5.1 \\
office && 19.3 & 40.3 & \cellcolor{tabfirst}59.9 & \cellcolor{tabsecond}45.2 && 24.1 & 53.5 & \cellcolor{tabfirst}82.2 & \cellcolor{tabsecond}56.5 && 25.6 & 59.1 & \cellcolor{tabfirst}88.9 & \cellcolor{tabsecond}59.9 && \cellcolor{tabfirst}0.4 & \cellcolor{tabsecond}0.6 & 1.1 & 19.1 \\
pipes && 29.4 & 76.6 & \cellcolor{tabfirst}89.8 & \cellcolor{tabsecond}86.3 && 36.3 & 91.6 & \cellcolor{tabfirst}96.6 & \cellcolor{tabsecond}95.4 && 41.1 & 95.0 & \cellcolor{tabfirst}98.0 & \cellcolor{tabsecond}97.3 && \cellcolor{tabfirst}0.3 & \cellcolor{tabsecond}0.4 & 0.8 & 3.4 \\
playground && 49.4 & 75.6 & \cellcolor{tabfirst}91.1 & \cellcolor{tabsecond}90.6 && 55.6 & 82.0 & \cellcolor{tabfirst}97.0 & \cellcolor{tabsecond}96.8 && 56.9 & 83.5 & \cellcolor{tabfirst}98.2 & \cellcolor{tabsecond}98.1 && 121.5 & \cellcolor{tabfirst}5.6 & \cellcolor{tabsecond}7.5 & 29.8 \\
relief && 89.8 & \cellcolor{tabsecond}93.4 & \cellcolor{tabfirst}93.7 & 93.3 && 96.6 & \cellcolor{tabsecond}97.8 & \cellcolor{tabfirst}97.9 & \cellcolor{tabsecond}97.8 && \cellcolor{tabsecond}97.9 & \cellcolor{tabfirst}98.7 & \cellcolor{tabfirst}98.7 & \cellcolor{tabfirst}98.7 && \cellcolor{tabfirst}3.7 & \cellcolor{tabsecond}5.7 & 15.3 & 34.1 \\
relief\_2 && 11.9 & 94.3 & \cellcolor{tabfirst}95.0 & \cellcolor{tabsecond}94.9 && 12.4 & 98.1 & \cellcolor{tabfirst}98.3 & \cellcolor{tabsecond}98.2 && 12.5 & \cellcolor{tabsecond}98.9 & \cellcolor{tabfirst}99.0 & \cellcolor{tabsecond}98.9 && \cellcolor{tabfirst}0.7 & \cellcolor{tabsecond}1.8 & 6.2 & 24.1 \\
terrace && 91.9 & 91.4 & \cellcolor{tabfirst}92.8 & \cellcolor{tabsecond}92.3 && 97.3 & 97.1 & \cellcolor{tabfirst}97.6 & \cellcolor{tabsecond}97.4 && 98.4 & 98.3 & \cellcolor{tabfirst}98.6 & \cellcolor{tabsecond}98.5 && \cellcolor{tabfirst}1.1 & \cellcolor{tabsecond}1.2 & 3.2 & 10.9 \\
terrains && 70.9 & 49.0 & \cellcolor{tabfirst}82.3 & \cellcolor{tabsecond}81.9 && 89.3 & 77.4 & \cellcolor{tabfirst}93.7 & \cellcolor{tabsecond}93.6 && 93.4 & 85.8 & \cellcolor{tabfirst}96.2 & \cellcolor{tabsecond}96.1 && 62.6 & \cellcolor{tabfirst}2.1 & \cellcolor{tabsecond}6.5 & 21.7 \\
botanical\_garden && 26.0 & \cellcolor{tabfirst}83.2 & \cellcolor{tabsecond}48.9 & 5.1 && 30.1 & \cellcolor{tabfirst}94.1 & \cellcolor{tabsecond}56.6 & 5.3 && 30.9 & \cellcolor{tabfirst}96.4 & \cellcolor{tabsecond}61.3 & 5.4 && \cellcolor{tabfirst}1.0 & \cellcolor{tabsecond}1.3 & 4.0 & 9.0 \\
boulders && 89.6 & 87.3 & \cellcolor{tabfirst}91.0 & \cellcolor{tabsecond}90.6 && 96.4 & 95.7 & \cellcolor{tabfirst}97.0 & \cellcolor{tabsecond}96.9 && 97.9 & 97.4 & \cellcolor{tabfirst}98.2 & \cellcolor{tabsecond}98.1 && \cellcolor{tabsecond}4.1 & \cellcolor{tabfirst}2.3 & 10.3 & 18.5 \\
bridge && 44.9 & 86.9 & \cellcolor{tabfirst}91.8 & \cellcolor{tabsecond}91.6 && 47.9 & \cellcolor{tabsecond}94.5 & \cellcolor{tabfirst}97.2 & \cellcolor{tabfirst}97.2 && 48.5 & \cellcolor{tabsecond}96.4 & \cellcolor{tabfirst}98.3 & \cellcolor{tabfirst}98.3 && \cellcolor{tabsecond}35.1 & \cellcolor{tabfirst}26.1 & 86.9 & 91.9 \\
door && 93.8 & 93.8 & \cellcolor{tabsecond}95.1 & \cellcolor{tabfirst}96.9 && 97.9 & 97.9 & \cellcolor{tabsecond}98.4 & \cellcolor{tabfirst}99.0 && 98.8 & 98.8 & \cellcolor{tabsecond}99.0 & \cellcolor{tabfirst}99.4 && \cellcolor{tabsecond}1.2 & \cellcolor{tabfirst}0.6 & 2.5 & 4.2 \\
exhibition\_hall && 11.0 & \cellcolor{tabsecond}32.4 & 25.5 & \cellcolor{tabfirst}85.4 && 15.2 & \cellcolor{tabsecond}38.6 & 29.7 & \cellcolor{tabfirst}94.3 && 16.3 & \cellcolor{tabsecond}40.2 & 30.7 & \cellcolor{tabfirst}96.5 && \cellcolor{tabfirst}20.6 & 72.3 & \cellcolor{tabsecond}69.5 & 72.0 \\
lecture\_room && 80.2 & 77.1 & \cellcolor{tabfirst}83.3 & \cellcolor{tabsecond}82.9 && \cellcolor{tabsecond}92.7 & 91.5 & \cellcolor{tabfirst}94.1 & \cellcolor{tabfirst}94.1 && 95.6 & 94.9 & \cellcolor{tabfirst}96.5 & \cellcolor{tabsecond}96.4 && \cellcolor{tabsecond}3.3 & \cellcolor{tabfirst}2.2 & 8.1 & 10.9 \\
living\_room && \cellcolor{tabsecond}88.0 & 85.1 & \cellcolor{tabsecond}88.0 & \cellcolor{tabfirst}88.3 && \cellcolor{tabfirst}95.8 & \cellcolor{tabsecond}94.6 & \cellcolor{tabfirst}95.8 & \cellcolor{tabfirst}95.8 && \cellcolor{tabsecond}97.4 & 96.7 & \cellcolor{tabsecond}97.4 & \cellcolor{tabfirst}97.5 && \cellcolor{tabfirst}9.4 & \cellcolor{tabsecond}14.3 & 35.1 & 49.1 \\
lounge && \cellcolor{tabfirst}34.1 & 30.2 & \cellcolor{tabsecond}34.0 & 33.9 && \cellcolor{tabfirst}35.4 & 34.1 & \cellcolor{tabsecond}35.3 & \cellcolor{tabsecond}35.3 && \cellcolor{tabfirst}35.6 & \cellcolor{tabsecond}34.8 & \cellcolor{tabfirst}35.6 & \cellcolor{tabfirst}35.6 && \cellcolor{tabfirst}0.4 & \cellcolor{tabfirst}0.4 & \cellcolor{tabsecond}1.3 & 1.8 \\
observatory && 58.4 & 63.8 & \cellcolor{tabfirst}65.4 & \cellcolor{tabsecond}64.4 && 83.7 & 86.3 & \cellcolor{tabfirst}87.0 & \cellcolor{tabsecond}86.5 && 89.9 & 91.7 & \cellcolor{tabfirst}92.1 & \cellcolor{tabsecond}91.8 && \cellcolor{tabsecond}5.8 & \cellcolor{tabfirst}3.3 & 12.2 & 24.4 \\
old\_computer && 23.3 & 49.0 & \cellcolor{tabsecond}53.8 & \cellcolor{tabfirst}78.7 && 41.5 & 59.6 & \cellcolor{tabsecond}61.4 & \cellcolor{tabfirst}90.2 && 48.4 & 61.9 & \cellcolor{tabsecond}63.0 & \cellcolor{tabfirst}92.7 && \cellcolor{tabsecond}5.9 & \cellcolor{tabfirst}2.2 & 8.4 & 19.6 \\
statue && 96.4 & \cellcolor{tabfirst}98.9 & \cellcolor{tabsecond}98.8 & 98.7 && \cellcolor{tabsecond}98.8 & \cellcolor{tabfirst}99.6 & \cellcolor{tabfirst}99.6 & \cellcolor{tabfirst}99.6 && 99.3 & \cellcolor{tabfirst}99.8 & \cellcolor{tabfirst}99.8 & \cellcolor{tabsecond}99.7 && \cellcolor{tabfirst}0.9 & \cellcolor{tabsecond}1.1 & 4.4 & 7.4 \\
terrace\_2 && 87.9 & 89.4 & \cellcolor{tabfirst}91.0 & \cellcolor{tabsecond}90.7 && 95.7 & 96.3 & \cellcolor{tabfirst}96.9 & \cellcolor{tabsecond}96.8 && 97.4 & 97.8 & \cellcolor{tabfirst}98.2 & \cellcolor{tabsecond}98.1 && \cellcolor{tabsecond}1.0 & \cellcolor{tabfirst}0.9 & 3.5 & 10.2 \\
\midrule
\textit{Average} && 60.4 & 73.5 & \cellcolor{tabfirst}79.3 & \cellcolor{tabsecond}79.2 && 68.1 & 82.7 & \cellcolor{tabfirst}87.0 & \cellcolor{tabsecond}86.5 && 70.1 & 85.0 & \cellcolor{tabfirst}88.8 & \cellcolor{tabsecond}88.1 && 26.5 & \cellcolor{tabfirst}7.9 & \cellcolor{tabsecond}16.7 & 27.5 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}



\begin{table}[t]
    \centering
    \caption{ETH3D Rig}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c a l c c c a l c c c a l c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{4}{c}{AUC @ $1^\circ$} && \multicolumn{4}{c}{AUC @ $3^\circ$} && \multicolumn{4}{c}{AUC @ $5^\circ$} 
        && \multicolumn{4}{c}{Time (s)}
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21}
        && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} &&  \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
delivery\_area && 0.0 & 30.0 & \cellcolor{tabfirst}76.1 & \cellcolor{tabsecond}66.6 && 0.1 & 71.0 & \cellcolor{tabfirst}91.2 & \cellcolor{tabsecond}87.5 && 0.3 & 81.6 & \cellcolor{tabfirst}94.6 & \cellcolor{tabsecond}92.2 && \cellcolor{tabfirst}235.7 & \cellcolor{tabsecond}250.0 & 505.1 & 1745.9 \\
electro && 0.2 & 13.4 & \cellcolor{tabfirst}47.4 & \cellcolor{tabsecond}38.4 && 1.8 & 48.2 & \cellcolor{tabfirst}72.7 & \cellcolor{tabsecond}65.2 && 2.9 & 63.3 & \cellcolor{tabfirst}81.5 & \cellcolor{tabsecond}75.2 && \cellcolor{tabfirst}99.9 & \cellcolor{tabsecond}181.2 & 362.9 & 3283.1 \\
forest && 0.0 & 68.3 & \cellcolor{tabsecond}74.2 & \cellcolor{tabfirst}74.7 && 0.0 & 87.7 & \cellcolor{tabsecond}90.0 & \cellcolor{tabfirst}90.3 && 0.1 & 92.1 & \cellcolor{tabsecond}93.5 & \cellcolor{tabfirst}93.7 && \cellcolor{tabfirst}306.6 & \cellcolor{tabsecond}532.1 & 1705.8 & 7571.6 \\
playground && 0.0 & \cellcolor{tabsecond}18.0 & \cellcolor{tabfirst}39.5 & 0.0 && 0.1 & \cellcolor{tabsecond}40.9 & \cellcolor{tabfirst}72.4 & 0.0 && 0.2 & \cellcolor{tabsecond}52.0 & \cellcolor{tabfirst}80.9 & 0.0 && \cellcolor{tabfirst}121.5 & 386.0 & 854.4 & \cellcolor{tabsecond}350.2 \\
terrains && 0.7 & 19.1 & \cellcolor{tabfirst}50.0 & \cellcolor{tabsecond}48.0 && 2.6 & 59.1 & \cellcolor{tabfirst}78.1 & \cellcolor{tabsecond}76.8 && 3.1 & 71.7 & \cellcolor{tabfirst}85.2 & \cellcolor{tabsecond}84.3 && \cellcolor{tabfirst}62.6 & \cellcolor{tabsecond}194.7 & 394.1 & 1333.9 \\
\midrule
\textit{Average} && 0.2 & 29.8 & \cellcolor{tabfirst}57.4 & \cellcolor{tabsecond}45.5 && 0.9 & 61.4 & \cellcolor{tabfirst}80.9 & \cellcolor{tabsecond}64.0 && 1.3 & \cellcolor{tabsecond}72.1 & \cellcolor{tabfirst}87.2 & 69.1 && \cellcolor{tabfirst}165.3 & \cellcolor{tabsecond}308.8 & 764.5 & 2857.0 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


\begin{table}[t]
    \centering
    \caption{IMC}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c a l c c c a l c c c a l c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{4}{c}{AUC @ $3^\circ$} && \multicolumn{4}{c}{AUC @ $5^\circ$} && \multicolumn{4}{c}{AUC @ $10^\circ$} 
        && \multicolumn{4}{c}{Time (s)}
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21}
        && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} &&  \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
bike && 0.0 & \cellcolor{tabsecond}37.9 & 34.9 & \cellcolor{tabfirst}77.9 && 0.0 & \cellcolor{tabsecond}47.5 & 38.9 & \cellcolor{tabfirst}86.7 && 0.0 & \cellcolor{tabsecond}67.7 & 42.9 & \cellcolor{tabfirst}93.4 && \cellcolor{tabfirst}0.0 & 2.0 & 1.5 & \cellcolor{tabsecond}1.1 \\
chairs && 0.0 & \cellcolor{tabsecond}16.4 & \cellcolor{tabfirst}82.6 & 0.8 && 0.0 & \cellcolor{tabsecond}20.3 & \cellcolor{tabfirst}89.6 & 0.8 && 0.0 & \cellcolor{tabsecond}26.1 & \cellcolor{tabfirst}94.8 & 0.8 && \cellcolor{tabfirst}0.0 & 2.8 & 1.6 & \cellcolor{tabsecond}0.6 \\
fountain && 22.1 & 90.6 & \cellcolor{tabsecond}91.2 & \cellcolor{tabfirst}91.3 && 24.2 & 94.3 & \cellcolor{tabsecond}94.7 & \cellcolor{tabfirst}94.8 && 25.7 & \cellcolor{tabsecond}97.2 & \cellcolor{tabfirst}97.4 & \cellcolor{tabfirst}97.4 && \cellcolor{tabfirst}0.8 & \cellcolor{tabsecond}2.2 & 3.8 & 5.9 \\
cyprus && 1.6 & \cellcolor{tabfirst}70.3 & \cellcolor{tabsecond}67.1 & 45.7 && 1.7 & \cellcolor{tabfirst}74.9 & \cellcolor{tabsecond}73.9 & 48.9 && 1.7 & \cellcolor{tabsecond}78.3 & \cellcolor{tabfirst}82.1 & 51.4 && \cellcolor{tabfirst}0.3 & 3.1 & \cellcolor{tabsecond}2.1 & 11.1 \\
dioscuri && 0.4 & 0.8 & \cellcolor{tabfirst}59.4 & \cellcolor{tabsecond}58.7 && 0.4 & 1.2 & \cellcolor{tabfirst}61.8 & \cellcolor{tabsecond}61.4 && 0.5 & 2.7 & \cellcolor{tabfirst}64.4 & \cellcolor{tabsecond}63.9 && \cellcolor{tabsecond}41.9 & \cellcolor{tabfirst}23.2 & 116.1 & 156.3 \\
wall && 57.1 & \cellcolor{tabsecond}91.6 & \cellcolor{tabfirst}94.6 & 88.6 && 73.9 & \cellcolor{tabsecond}95.0 & \cellcolor{tabfirst}96.8 & 93.2 && 87.0 & \cellcolor{tabsecond}97.5 & \cellcolor{tabfirst}98.4 & 96.6 && \cellcolor{tabfirst}23.8 & \cellcolor{tabsecond}35.4 & 66.0 & 63.5 \\
kyiv-puppet-theater && 0.7 & \cellcolor{tabsecond}4.0 & \cellcolor{tabfirst}12.1 & 0.3 && 0.7 & \cellcolor{tabsecond}4.7 & \cellcolor{tabfirst}16.1 & 0.3 && 0.9 & \cellcolor{tabsecond}6.4 & \cellcolor{tabfirst}19.8 & 0.3 && \cellcolor{tabfirst}0.3 & \cellcolor{tabsecond}2.0 & 2.7 & \cellcolor{tabfirst}0.3 \\
brandenburg\_gate && 21.4 & 1.8 & \cellcolor{tabsecond}70.0 & \cellcolor{tabfirst}70.1 && 35.0 & 4.6 & \cellcolor{tabsecond}76.4 & \cellcolor{tabfirst}77.2 && 53.6 & 12.5 & \cellcolor{tabsecond}82.5 & \cellcolor{tabfirst}83.9 && 1171.8 & \cellcolor{tabfirst}131.3 & \cellcolor{tabsecond}298.0 & 1472.1 \\
british\_museum && 18.5 & 18.1 & \cellcolor{tabsecond}61.0 & \cellcolor{tabfirst}61.6 && 32.0 & 29.6 & \cellcolor{tabsecond}71.5 & \cellcolor{tabfirst}72.7 && 51.3 & 46.9 & \cellcolor{tabsecond}82.2 & \cellcolor{tabfirst}83.9 && \cellcolor{tabsecond}78.1 & \cellcolor{tabfirst}44.5 & 115.3 & 318.0 \\
buckingham\_palace && 4.1 & 1.5 & \cellcolor{tabfirst}85.2 & \cellcolor{tabsecond}80.5 && 12.5 & 4.0 & \cellcolor{tabfirst}88.6 & \cellcolor{tabsecond}86.2 && 34.0 & 11.9 & \cellcolor{tabfirst}91.9 & \cellcolor{tabsecond}91.1 && \cellcolor{tabsecond}429.7 & \cellcolor{tabfirst}156.1 & 498.5 & 4948.2 \\
colosseum\_exterior && 37.3 & 3.0 & \cellcolor{tabfirst}80.8 & \cellcolor{tabsecond}80.7 && \cellcolor{tabsecond}52.8 & 6.3 & \cellcolor{tabfirst}86.1 & \cellcolor{tabfirst}86.1 && 69.2 & 13.5 & \cellcolor{tabsecond}90.7 & \cellcolor{tabfirst}90.8 && \cellcolor{tabsecond}542.8 & \cellcolor{tabfirst}331.3 & 804.6 & 3561.7 \\
grand\_place\_brussels && 18.3 & 8.9 & \cellcolor{tabfirst}70.0 & \cellcolor{tabsecond}68.7 && 32.4 & 15.1 & \cellcolor{tabsecond}76.5 & \cellcolor{tabfirst}76.6 && 50.5 & 33.5 & \cellcolor{tabsecond}82.5 & \cellcolor{tabfirst}84.2 && \cellcolor{tabsecond}124.2 & \cellcolor{tabfirst}71.6 & 241.0 & 520.3 \\
lincoln..\_statue && 1.0 & 7.7 & \cellcolor{tabfirst}68.2 & \cellcolor{tabsecond}67.2 && 4.4 & 17.0 & \cellcolor{tabfirst}72.3 & \cellcolor{tabsecond}71.5 && 23.8 & 33.1 & \cellcolor{tabfirst}75.8 & \cellcolor{tabsecond}75.3 && \cellcolor{tabsecond}99.9 & \cellcolor{tabfirst}44.3 & 110.0 & 362.3 \\
notre\_dame..\_facade && 32.5 & 1.2 & \cellcolor{tabsecond}66.3 & \cellcolor{tabfirst}69.1 && 43.0 & 4.5 & \cellcolor{tabsecond}69.9 & \cellcolor{tabfirst}72.5 && 55.2 & 14.6 & \cellcolor{tabsecond}73.3 & \cellcolor{tabfirst}75.5 && \cellcolor{tabsecond}2592.1 & \cellcolor{tabfirst}801.0 & 4066.8 & 52135.4 \\
pantheon\_exterior && 49.6 & 51.4 & \cellcolor{tabsecond}75.7 & \cellcolor{tabfirst}79.4 && 62.3 & 63.1 & \cellcolor{tabsecond}80.5 & \cellcolor{tabfirst}83.5 && 74.4 & 74.6 & \cellcolor{tabsecond}84.9 & \cellcolor{tabfirst}87.2 && \cellcolor{tabsecond}285.7 & \cellcolor{tabfirst}208.7 & 463.8 & 1454.6 \\
piazza\_san\_marco && 2.6 & 6.2 & \cellcolor{tabfirst}69.9 & \cellcolor{tabsecond}58.0 && 6.4 & 16.0 & \cellcolor{tabfirst}78.9 & \cellcolor{tabsecond}71.0 && 23.7 & 40.7 & \cellcolor{tabfirst}87.1 & \cellcolor{tabsecond}83.7 && \cellcolor{tabsecond}16.7 & \cellcolor{tabfirst}12.5 & 46.0 & 74.2 \\
sacre\_coeur && 37.1 & 15.5 & \cellcolor{tabsecond}78.3 & \cellcolor{tabfirst}78.5 && 50.8 & 24.4 & \cellcolor{tabsecond}80.8 & \cellcolor{tabfirst}80.9 && \cellcolor{tabsecond}64.8 & 40.6 & \cellcolor{tabfirst}82.8 & \cellcolor{tabfirst}82.8 && \cellcolor{tabsecond}196.1 & \cellcolor{tabfirst}105.1 & 300.4 & 682.2 \\
sagrada\_familia && 30.3 & 47.4 & \cellcolor{tabsecond}53.8 & \cellcolor{tabfirst}54.3 && 39.2 & 52.7 & \cellcolor{tabsecond}58.7 & \cellcolor{tabfirst}58.9 && 48.9 & \cellcolor{tabsecond}57.7 & \cellcolor{tabfirst}62.9 & \cellcolor{tabfirst}62.9 && \cellcolor{tabsecond}42.6 & \cellcolor{tabfirst}37.5 & 114.1 & 237.0 \\
st\_pauls\_cathedral && 1.9 & 10.3 & \cellcolor{tabfirst}74.2 & \cellcolor{tabsecond}72.7 && 6.5 & 24.6 & \cellcolor{tabfirst}80.3 & \cellcolor{tabsecond}78.9 && 25.8 & 44.8 & \cellcolor{tabfirst}85.8 & \cellcolor{tabsecond}85.0 && \cellcolor{tabsecond}61.9 & \cellcolor{tabfirst}35.9 & 94.2 & 241.4 \\
st\_peters\_square && 31.1 & 6.2 & \cellcolor{tabsecond}79.1 & \cellcolor{tabfirst}83.6 && 46.0 & 12.4 & \cellcolor{tabsecond}83.9 & \cellcolor{tabfirst}87.8 && 64.0 & 24.8 & \cellcolor{tabsecond}88.7 & \cellcolor{tabfirst}91.6 && \cellcolor{tabsecond}961.0 & \cellcolor{tabfirst}374.9 & 1055.2 & 6051.9 \\
taj\_mahal && 38.6 & 4.9 & \cellcolor{tabfirst}74.4 & \cellcolor{tabsecond}68.9 && 51.0 & 11.4 & \cellcolor{tabfirst}78.9 & \cellcolor{tabsecond}75.5 && 64.9 & 23.6 & \cellcolor{tabfirst}83.5 & \cellcolor{tabsecond}81.7 && \cellcolor{tabsecond}380.1 & \cellcolor{tabfirst}176.4 & 539.6 & 4528.9 \\
trevi\_fountain && 43.4 & 22.6 & \cellcolor{tabsecond}79.1 & \cellcolor{tabfirst}80.5 && 56.2 & 40.5 & \cellcolor{tabsecond}82.8 & \cellcolor{tabfirst}84.4 && 69.3 & 59.2 & \cellcolor{tabsecond}86.4 & \cellcolor{tabfirst}87.8 && \cellcolor{tabsecond}1202.9 & \cellcolor{tabfirst}689.5 & 1718.5 & 12294.4 \\
\midrule
\textit{Average} && 20.4 & 23.6 & \cellcolor{tabfirst}69.4 & \cellcolor{tabsecond}65.3 && 28.7 & 30.2 & \cellcolor{tabfirst}74.5 & \cellcolor{tabsecond}70.4 && 40.4 & 41.3 & \cellcolor{tabfirst}79.1 & \cellcolor{tabsecond}75.1 && \cellcolor{tabsecond}412.6 & \cellcolor{tabfirst}149.6 & 484.5 & 4051.0 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


\begin{table}[t]
    \centering
    \caption{ETH3D SLAM}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c a l c c c a l c c c a l c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{4}{c}{Recall @ 0.1m} && \multicolumn{4}{c}{AUC @ 0.1m} && \multicolumn{4}{c}{AUC @ 0.5m} 
        && \multicolumn{4}{c}{Time (s)}
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21}
        && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} &&  \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
cables && \cellcolor{tabsecond}76.8 & \cellcolor{tabfirst}88.0 & \cellcolor{tabfirst}88.0 & 68.0 && \cellcolor{tabsecond}59.1 & 53.6 & \cellcolor{tabfirst}75.3 & 56.5 && 77.4 & \cellcolor{tabsecond}81.1 & \cellcolor{tabfirst}85.4 & 70.4 && \cellcolor{tabfirst}103.1 & \cellcolor{tabsecond}170.9 & 179.2 & 2553.4 \\
camera && 2.2 & \cellcolor{tabsecond}33.0 & 32.5 & \cellcolor{tabfirst}34.8 && 2.0 & 15.7 & \cellcolor{tabsecond}22.4 & \cellcolor{tabfirst}24.7 && 2.2 & \cellcolor{tabfirst}35.4 & 30.8 & \cellcolor{tabsecond}33.2 && \cellcolor{tabfirst}1.5 & 24.6 & \cellcolor{tabsecond}7.3 & 196.2 \\
ceiling && 6.4 & \cellcolor{tabsecond}28.2 & \cellcolor{tabfirst}28.6 & \cellcolor{tabfirst}28.6 && 2.9 & 11.8 & \cellcolor{tabfirst}21.1 & \cellcolor{tabsecond}15.3 && 8.2 & \cellcolor{tabfirst}29.0 & \cellcolor{tabsecond}27.2 & 26.3 && \cellcolor{tabfirst}78.3 & 132.5 & \cellcolor{tabsecond}101.8 & 1057.7 \\
desk && 28.0 & \cellcolor{tabfirst}33.8 & \cellcolor{tabsecond}32.3 & 24.4 && 16.0 & 17.2 & \cellcolor{tabfirst}29.0 & \cellcolor{tabsecond}21.1 && 28.6 & \cellcolor{tabfirst}32.9 & \cellcolor{tabsecond}31.7 & 23.7 && 376.2 & \cellcolor{tabsecond}200.9 & \cellcolor{tabfirst}159.8 & 1115.1 \\
einstein && 32.9 & \cellcolor{tabsecond}41.3 & \cellcolor{tabfirst}49.4 & 33.6 && 22.7 & \cellcolor{tabsecond}29.2 & \cellcolor{tabfirst}37.2 & 25.4 && 34.2 & \cellcolor{tabsecond}42.4 & \cellcolor{tabfirst}48.0 & 36.7 && \cellcolor{tabsecond}150.3 & \cellcolor{tabfirst}61.2 & 152.1 & 1230.8 \\
kidnap && \cellcolor{tabsecond}73.1 & \cellcolor{tabfirst}73.3 & \cellcolor{tabfirst}73.3 & \cellcolor{tabfirst}73.3 && 63.4 & 59.8 & \cellcolor{tabfirst}70.0 & \cellcolor{tabsecond}68.5 && 71.2 & 70.6 & \cellcolor{tabfirst}72.6 & \cellcolor{tabsecond}72.3 && \cellcolor{tabfirst}114.4 & 668.8 & \cellcolor{tabsecond}136.6 & 731.2 \\
large && 35.4 & \cellcolor{tabsecond}47.6 & \cellcolor{tabfirst}49.0 & 44.5 && 18.1 & 20.2 & \cellcolor{tabfirst}45.1 & \cellcolor{tabsecond}20.7 && 33.7 & \cellcolor{tabsecond}43.4 & \cellcolor{tabfirst}48.2 & \cellcolor{tabsecond}43.4 && \cellcolor{tabsecond}91.9 & 113.0 & \cellcolor{tabfirst}73.7 & 983.8 \\
mannequin && 49.1 & 58.5 & \cellcolor{tabfirst}66.8 & \cellcolor{tabsecond}59.3 && 36.7 & 39.0 & \cellcolor{tabfirst}55.8 & \cellcolor{tabsecond}52.8 && 49.1 & \cellcolor{tabsecond}58.5 & \cellcolor{tabfirst}64.8 & 58.4 && \cellcolor{tabfirst}33.5 & 66.5 & \cellcolor{tabsecond}43.9 & 301.2 \\
motion && \cellcolor{tabsecond}18.8 & 14.1 & \cellcolor{tabfirst}44.7 & 17.7 && 11.0 & 7.7 & \cellcolor{tabfirst}23.1 & \cellcolor{tabsecond}12.9 && \cellcolor{tabsecond}23.3 & 13.7 & \cellcolor{tabfirst}56.1 & 19.7 && 859.7 & \cellcolor{tabfirst}84.8 & \cellcolor{tabsecond}654.2 & 9995.1 \\
planar && \cellcolor{tabsecond}30.6 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 12.5 & 94.4 & \cellcolor{tabfirst}98.7 & \cellcolor{tabsecond}98.3 && 38.0 & \cellcolor{tabsecond}98.9 & \cellcolor{tabfirst}99.7 & \cellcolor{tabfirst}99.7 && \cellcolor{tabsecond}313.8 & \cellcolor{tabfirst}154.8 & 572.4 & 2349.7 \\
plant && 77.0 & 87.0 & \cellcolor{tabsecond}92.0 & \cellcolor{tabfirst}92.8 && 62.9 & 71.4 & \cellcolor{tabsecond}81.4 & \cellcolor{tabfirst}82.3 && 77.1 & 89.4 & \cellcolor{tabsecond}92.1 & \cellcolor{tabfirst}92.5 && \cellcolor{tabfirst}21.7 & 48.8 & \cellcolor{tabsecond}26.9 & 202.7 \\
reflective && 12.6 & 16.2 & \cellcolor{tabsecond}22.2 & \cellcolor{tabfirst}26.2 && 6.7 & 4.8 & \cellcolor{tabsecond}8.6 & \cellcolor{tabfirst}9.2 && 16.5 & 20.0 & \cellcolor{tabsecond}29.1 & \cellcolor{tabfirst}33.5 && 721.3 & \cellcolor{tabfirst}104.7 & \cellcolor{tabsecond}448.1 & 6573.9 \\
repetitive && 26.3 & \cellcolor{tabsecond}28.7 & \cellcolor{tabfirst}32.7 & 28.5 && 23.9 & 14.1 & \cellcolor{tabsecond}26.7 & \cellcolor{tabfirst}27.2 && 25.8 & 26.8 & \cellcolor{tabfirst}31.5 & \cellcolor{tabsecond}28.3 && \cellcolor{tabfirst}63.2 & 106.4 & \cellcolor{tabsecond}86.7 & 561.1 \\
sfm && 83.2 & \cellcolor{tabsecond}90.4 & \cellcolor{tabfirst}97.0 & 55.9 && \cellcolor{tabsecond}57.9 & 46.0 & \cellcolor{tabfirst}78.3 & 35.7 && 80.0 & \cellcolor{tabsecond}86.3 & \cellcolor{tabfirst}95.0 & 55.8 && \cellcolor{tabfirst}91.7 & \cellcolor{tabsecond}158.7 & 209.5 & 469.6 \\
sofa && 11.2 & 18.6 & \cellcolor{tabsecond}23.9 & \cellcolor{tabfirst}32.2 && 5.5 & 10.7 & \cellcolor{tabsecond}21.8 & \cellcolor{tabfirst}28.6 && 10.3 & 18.3 & \cellcolor{tabsecond}23.5 & \cellcolor{tabfirst}31.6 && \cellcolor{tabfirst}9.1 & \cellcolor{tabsecond}9.9 & 10.1 & 157.3 \\
table && 79.1 & 83.9 & \cellcolor{tabsecond}94.3 & \cellcolor{tabfirst}99.9 && 68.2 & 57.8 & \cellcolor{tabsecond}88.5 & \cellcolor{tabfirst}95.6 && 76.9 & 81.9 & \cellcolor{tabsecond}93.2 & \cellcolor{tabfirst}99.1 && \cellcolor{tabsecond}182.0 & \cellcolor{tabfirst}61.2 & 233.1 & 2777.7 \\
vicon && 64.6 & 74.4 & \cellcolor{tabfirst}97.0 & \cellcolor{tabsecond}81.1 && 20.4 & \cellcolor{tabsecond}49.6 & \cellcolor{tabfirst}79.1 & 38.9 && 71.7 & \cellcolor{tabsecond}84.0 & \cellcolor{tabfirst}93.5 & 75.0 && \cellcolor{tabsecond}50.9 & 149.8 & \cellcolor{tabfirst}47.4 & 474.8 \\
\midrule
\textit{Average} && 48.2 & \cellcolor{tabsecond}60.1 & \cellcolor{tabfirst}66.3 & 57.9 && 34.9 & 40.6 & \cellcolor{tabfirst}56.0 & \cellcolor{tabsecond}47.6 && 48.6 & \cellcolor{tabsecond}60.0 & \cellcolor{tabfirst}65.3 & 57.9 && \cellcolor{tabsecond}120.8 & \cellcolor{tabfirst}97.7 & 130.6 & 1115.4 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


==> tex/tbl/refactored_more.tex <==

\begin{table}[t]
    \centering
    \caption{LaMAR}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c a l c c c a l c c c a l c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        % && \multicolumn{3}{c}{Thres 5m} && \multicolumn{3}{c}{AUC @ 5} && \multicolumn{3}{c}{AUC @ 10} 
        && \multicolumn{4}{c}{Recall @ 1m} && \multicolumn{4}{c}{AUC @ 1m} && \multicolumn{4}{c}{AUC @ 5m} 
        && \multicolumn{4}{c}{Time (s)}
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} &&  \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
CAB && - & 3.2 & 6.3 & \cellcolor{tabsecond}11.6 & \cellcolor{tabfirst}13.0 && - & 1.3 & 2.7 & \cellcolor{tabsecond} 4.7 & \cellcolor{tabfirst} 5.8 && - & 9.2 & 11.5 & \cellcolor{tabsecond}16.9 & \cellcolor{tabfirst}19.2 && - & \cellcolor{tabfirst}1453.5 & \cellcolor{tabsecond}3114.9 & 6162.24 & 194033.6 \\
HGE && - & 3.4 & 13.4 & \cellcolor{tabfirst}48.4 & \cellcolor{tabsecond}38.9 && - & 1.3 & 8.1 & \cellcolor{tabfirst}22.2 & \cellcolor{tabsecond}18.0 && - & 1.3 & 14.5 & \cellcolor{tabfirst}50.3 & \cellcolor{tabsecond}46.9 && - & \cellcolor{tabfirst}1829.7 & \cellcolor{tabsecond}2996.4 & 12587.2 & 249771.1 \\
LIN$^*$ && - & 8.6 & \cellcolor{tabfirst}87.3 & \cellcolor{tabsecond}44.2 && - & 3.3 & \cellcolor{tabfirst}46.7 & \cellcolor{tabsecond}17.7 &&  - & 24.1 & \cellcolor{tabfirst}85.6 & \cellcolor{tabsecond}52.3 &&  - & \cellcolor{tabfirst}2783.3 & \cellcolor{tabsecond}17182.9 & 620176.4 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}

\begin{table}[t]
    \centering
    \caption{Refactored -- Mip360}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{AUC @ $3^\circ$} && \multicolumn{5}{c}{AUC @ $5^\circ$} && \multicolumn{5}{c}{AUC @ $10^\circ$} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} \\  \midrule
bicycle && 89.2 & 70.7 & \cellcolor{tabsecond}95.3 & \cellcolor{tabfirst}95.8 & \cellcolor{tabfirst}95.8 && 92.7 & 81.0 & \cellcolor{tabsecond}97.2 & \cellcolor{tabfirst}97.5 & \cellcolor{tabfirst}97.5 && 95.3 & 89.4 & \cellcolor{tabsecond}98.6 & \cellcolor{tabfirst}98.7 & \cellcolor{tabfirst}98.7 && 123.1 & \cellcolor{tabfirst}34.5 & \cellcolor{tabsecond}55.3 & 60.6 & 120.6 \\
bonsai && 9.4 & 48.4 & 87.6 & \cellcolor{tabfirst}98.5 & \cellcolor{tabsecond}92.6 && 27.9 & 50.3 & 92.5 & \cellcolor{tabfirst}99.1 & \cellcolor{tabsecond}95.6 && 61.2 & 66.9 & 96.2 & \cellcolor{tabfirst}99.6 & \cellcolor{tabsecond}97.8 && \cellcolor{tabfirst}176.0 & \cellcolor{tabsecond}218.0 & 265.2 & 463.5 & 662.5 \\
counter && 96.9 & 99.0 & 97.9 & \cellcolor{tabfirst}99.3 & \cellcolor{tabsecond}99.2 && 98.1 & 99.4 & 98.8 & \cellcolor{tabfirst}99.6 & \cellcolor{tabsecond}99.5 && 99.1 & \cellcolor{tabsecond}99.7 & 99.4 & \cellcolor{tabfirst}99.8 & \cellcolor{tabfirst}99.8 && \cellcolor{tabfirst}46.6 & \cellcolor{tabsecond}79.5 & 130.8 & 206.7 & 270.5 \\
garden && 95.0 & 0.5 & \cellcolor{tabsecond}97.0 & \cellcolor{tabfirst}97.3 & \cellcolor{tabfirst}97.3 && 97.0 & 0.7 & \cellcolor{tabsecond}98.2 & \cellcolor{tabfirst}98.4 & \cellcolor{tabfirst}98.4 && 98.5 & 2.2 & \cellcolor{tabsecond}99.1 & \cellcolor{tabfirst}99.2 & \cellcolor{tabfirst}99.2 && \cellcolor{tabsecond}40.2 & \cellcolor{tabfirst}36.2 & 98.7 & 135.6 & 291.8 \\
kitchen && 88.5 & 92.0 & 92.3 & \cellcolor{tabsecond}94.8 & \cellcolor{tabfirst}94.9 && 93.1 & 95.2 & 95.4 & \cellcolor{tabsecond}96.9 & \cellcolor{tabfirst}97.0 && 96.5 & 97.6 & 97.7 & \cellcolor{tabsecond}98.4 & \cellcolor{tabfirst}98.5 && \cellcolor{tabfirst}127.0 & \cellcolor{tabsecond}146.8 & 303.5 & 435.0 & 619.1 \\
room && 39.6 & 32.6 & 88.1 & \cellcolor{tabfirst}97.8 & \cellcolor{tabsecond}96.2 && 42.2 & 33.8 & 92.3 & \cellcolor{tabfirst}98.7 & \cellcolor{tabsecond}97.7 && 44.9 & 35.7 & 95.8 & \cellcolor{tabfirst}99.3 & \cellcolor{tabsecond}98.9 && \cellcolor{tabsecond}96.3 & \cellcolor{tabfirst}80.2 & 168.5 & 226.9 & 371.6 \\
stump && 95.3 & 3.5 & \cellcolor{tabsecond}97.0 & \cellcolor{tabfirst}99.1 & \cellcolor{tabfirst}99.1 && 97.1 & 5.7 & \cellcolor{tabsecond}98.2 & \cellcolor{tabfirst}99.5 & \cellcolor{tabfirst}99.5 && 98.5 & 16.8 & \cellcolor{tabsecond}99.1 & \cellcolor{tabfirst}99.7 & \cellcolor{tabfirst}99.7 && 38.7 & \cellcolor{tabfirst}15.5 & \cellcolor{tabsecond}26.4 & 26.7 & 83.9 \\
\midrule
\textit{Average} && 73.4 & 49.5 & 93.6 & \cellcolor{tabfirst}97.5 & \cellcolor{tabsecond}96.5 && 78.3 & 52.3 & 96.1 & \cellcolor{tabfirst}98.5 & \cellcolor{tabsecond}97.9 && 84.9 & 58.3 & 98.0 & \cellcolor{tabfirst}99.3 & \cellcolor{tabsecond}98.9 && \cellcolor{tabsecond}92.6 & \cellcolor{tabfirst}87.2 & 149.8 & 222.2 & 345.7 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


\begin{table}[t]
    \centering
    \caption{New results -- ETH3D DSLR}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{AUC @ $1^\circ$} && \multicolumn{5}{c}{AUC @ $3^\circ$} && \multicolumn{5}{c}{AUC @ $5^\circ$} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} \\  \midrule
courtyard && 68.2 & \cellcolor{tabfirst}89.6 & 86.7 & \cellcolor{tabsecond}87.7 & 87.3 && 81.7 & \cellcolor{tabfirst}96.5 & 95.6 & \cellcolor{tabsecond}95.9 & 95.8 && 85.9 & \cellcolor{tabfirst}97.9 & 97.3 & \cellcolor{tabsecond}97.5 & \cellcolor{tabsecond}97.5 && \cellcolor{tabsecond}11.2 & \cellcolor{tabfirst}9.2 & 16.2 & 22.5 & 39.2 \\
delivery\_area && 91.4 & 89.5 & 92.2 & \cellcolor{tabfirst}92.8 & \cellcolor{tabsecond}92.3 && 97.1 & 96.5 & \cellcolor{tabsecond}97.4 & \cellcolor{tabfirst}97.6 & \cellcolor{tabsecond}97.4 && 98.3 & 97.9 & 98.4 & \cellcolor{tabfirst}98.6 & \cellcolor{tabsecond}98.5 && 235.7 & \cellcolor{tabfirst}3.3 & \cellcolor{tabsecond}8.0 & 12.3 & 26.4 \\
electro && 72.6 & 64.7 & \cellcolor{tabfirst}81.3 & \cellcolor{tabsecond}79.3 & 70.0 && 81.8 & 73.5 & \cellcolor{tabfirst}90.9 & \cellcolor{tabsecond}86.7 & 75.7 && 83.9 & 76.6 & \cellcolor{tabfirst}94.0 & \cellcolor{tabsecond}88.5 & 77.0 && 99.9 & \cellcolor{tabfirst}3.6 & \cellcolor{tabsecond}5.2 & 7.4 & 23.9 \\
facade && 89.4 & 90.0 & \cellcolor{tabsecond}90.6 & \cellcolor{tabfirst}91.1 & 90.3 && 96.4 & 96.6 & \cellcolor{tabsecond}96.8 & \cellcolor{tabfirst}97.0 & 96.7 && 97.8 & 98.0 & \cellcolor{tabsecond}98.1 & \cellcolor{tabfirst}98.2 & 98.0 && \cellcolor{tabsecond}35.1 & \cellcolor{tabfirst}33.0 & 57.7 & 80.2 & 113.5 \\
kicker && 82.0 & 79.2 & 86.0 & \cellcolor{tabsecond}86.3 & \cellcolor{tabfirst}86.6 && 89.6 & 86.0 & \cellcolor{tabfirst}95.2 & \cellcolor{tabsecond}94.3 & 91.3 && 91.2 & 88.5 & \cellcolor{tabfirst}97.1 & \cellcolor{tabsecond}96.5 & 92.2 && \cellcolor{tabfirst}1.7 & \cellcolor{tabsecond}2.2 & 3.7 & 6.7 & 16.2 \\
meadow && 10.5 & 26.1 & \cellcolor{tabfirst}76.4 & \cellcolor{tabsecond}74.7 & 61.6 && 13.8 & 36.7 & \cellcolor{tabfirst}90.7 & \cellcolor{tabsecond}90.4 & 77.8 && 14.7 & 40.6 & \cellcolor{tabfirst}94.4 & \cellcolor{tabsecond}94.2 & 81.5 && \cellcolor{tabfirst}0.3 & 1.0 & \cellcolor{tabsecond}0.7 & 2.1 & 5.1 \\
office && 19.3 & 40.3 & \cellcolor{tabsecond}59.3 & \cellcolor{tabfirst}59.9 & 45.2 && 24.1 & 53.5 & \cellcolor{tabsecond}81.5 & \cellcolor{tabfirst}82.2 & 56.5 && 25.6 & 59.1 & \cellcolor{tabsecond}88.3 & \cellcolor{tabfirst}88.9 & 59.9 && \cellcolor{tabfirst}0.4 & \cellcolor{tabsecond}0.6 & 0.8 & 1.1 & 19.1 \\
pipes && 29.4 & 76.6 & \cellcolor{tabsecond}88.9 & \cellcolor{tabfirst}89.8 & 86.3 && 36.3 & 91.6 & \cellcolor{tabsecond}96.3 & \cellcolor{tabfirst}96.6 & 95.4 && 41.1 & 95.0 & \cellcolor{tabsecond}97.8 & \cellcolor{tabfirst}98.0 & 97.3 && \cellcolor{tabfirst}0.3 & \cellcolor{tabsecond}0.4 & \cellcolor{tabsecond}0.4 & 0.8 & 3.4 \\
playground && 49.4 & 75.6 & \cellcolor{tabsecond}90.9 & \cellcolor{tabfirst}91.1 & 90.6 && 55.6 & 82.0 & \cellcolor{tabsecond}96.9 & \cellcolor{tabfirst}97.0 & 96.8 && 56.9 & 83.5 & \cellcolor{tabsecond}98.1 & \cellcolor{tabfirst}98.2 & \cellcolor{tabsecond}98.1 && 121.5 & \cellcolor{tabfirst}5.6 & \cellcolor{tabsecond}6.3 & 7.5 & 29.8 \\
relief && 89.8 & \cellcolor{tabsecond}93.4 & \cellcolor{tabsecond}93.4 & \cellcolor{tabfirst}93.7 & 93.3 && 96.6 & \cellcolor{tabsecond}97.8 & \cellcolor{tabsecond}97.8 & \cellcolor{tabfirst}97.9 & \cellcolor{tabsecond}97.8 && \cellcolor{tabsecond}97.9 & \cellcolor{tabfirst}98.7 & \cellcolor{tabfirst}98.7 & \cellcolor{tabfirst}98.7 & \cellcolor{tabfirst}98.7 && \cellcolor{tabfirst}3.7 & \cellcolor{tabsecond}5.7 & 10.9 & 15.3 & 34.1 \\
relief\_2 && 11.9 & 94.3 & 94.2 & \cellcolor{tabfirst}95.0 & \cellcolor{tabsecond}94.9 && 12.4 & 98.1 & 98.1 & \cellcolor{tabfirst}98.3 & \cellcolor{tabsecond}98.2 && 12.5 & \cellcolor{tabsecond}98.9 & 98.8 & \cellcolor{tabfirst}99.0 & \cellcolor{tabsecond}98.9 && \cellcolor{tabfirst}0.7 & \cellcolor{tabsecond}1.8 & 5.0 & 6.2 & 24.1 \\
terrace && 91.9 & 91.4 & 92.1 & \cellcolor{tabfirst}92.8 & \cellcolor{tabsecond}92.3 && 97.3 & 97.1 & \cellcolor{tabsecond}97.4 & \cellcolor{tabfirst}97.6 & \cellcolor{tabsecond}97.4 && 98.4 & 98.3 & 98.4 & \cellcolor{tabfirst}98.6 & \cellcolor{tabsecond}98.5 && \cellcolor{tabfirst}1.1 & \cellcolor{tabsecond}1.2 & 3.3 & 3.2 & 10.9 \\
terrains && 70.9 & 49.0 & \cellcolor{tabfirst}84.6 & \cellcolor{tabsecond}82.3 & 81.9 && 89.3 & 77.4 & \cellcolor{tabfirst}94.6 & \cellcolor{tabsecond}93.7 & 93.6 && 93.4 & 85.8 & \cellcolor{tabfirst}96.7 & \cellcolor{tabsecond}96.2 & 96.1 && 62.6 & \cellcolor{tabfirst}2.1 & \cellcolor{tabsecond}4.0 & 6.5 & 21.7 \\
botanical\_garden && 26.0 & \cellcolor{tabsecond}83.2 & \cellcolor{tabfirst}83.6 & 48.9 & 5.1 && 30.1 & \cellcolor{tabsecond}94.1 & \cellcolor{tabfirst}94.3 & 56.6 & 5.3 && 30.9 & \cellcolor{tabsecond}96.4 & \cellcolor{tabfirst}96.6 & 61.3 & 5.4 && \cellcolor{tabfirst}1.0 & \cellcolor{tabsecond}1.3 & 3.3 & 4.0 & 9.0 \\
boulders && 89.6 & 87.3 & 90.4 & \cellcolor{tabfirst}91.0 & \cellcolor{tabsecond}90.6 && 96.4 & 95.7 & 96.8 & \cellcolor{tabfirst}97.0 & \cellcolor{tabsecond}96.9 && 97.9 & 97.4 & \cellcolor{tabsecond}98.1 & \cellcolor{tabfirst}98.2 & \cellcolor{tabsecond}98.1 && \cellcolor{tabsecond}4.1 & \cellcolor{tabfirst}2.3 & 10.9 & 10.3 & 18.5 \\
bridge && 44.9 & 86.9 & 45.6 & \cellcolor{tabfirst}91.8 & \cellcolor{tabsecond}91.6 && 47.9 & \cellcolor{tabsecond}94.5 & 48.1 & \cellcolor{tabfirst}97.2 & \cellcolor{tabfirst}97.2 && 48.5 & \cellcolor{tabsecond}96.4 & 48.6 & \cellcolor{tabfirst}98.3 & \cellcolor{tabfirst}98.3 && \cellcolor{tabsecond}35.1 & \cellcolor{tabfirst}26.1 & 85.2 & 86.9 & 91.9 \\
door && 93.8 & 93.8 & \cellcolor{tabsecond}96.5 & 95.1 & \cellcolor{tabfirst}96.9 && 97.9 & 97.9 & \cellcolor{tabsecond}98.8 & 98.4 & \cellcolor{tabfirst}99.0 && 98.8 & 98.8 & \cellcolor{tabsecond}99.3 & 99.0 & \cellcolor{tabfirst}99.4 && \cellcolor{tabsecond}1.2 & \cellcolor{tabfirst}0.6 & 3.3 & 2.5 & 4.2 \\
exhibition\_hall && 11.0 & \cellcolor{tabsecond}32.4 & 19.8 & 25.5 & \cellcolor{tabfirst}85.4 && 15.2 & \cellcolor{tabsecond}38.6 & 23.0 & 29.7 & \cellcolor{tabfirst}94.3 && 16.3 & \cellcolor{tabsecond}40.2 & 23.7 & 30.7 & \cellcolor{tabfirst}96.5 && \cellcolor{tabfirst}20.6 & 72.3 & 107.8 & \cellcolor{tabsecond}69.5 & 72.0 \\
lecture\_room && 80.2 & 77.1 & \cellcolor{tabfirst}84.2 & \cellcolor{tabsecond}83.3 & 82.9 && 92.7 & 91.5 & \cellcolor{tabfirst}94.4 & \cellcolor{tabsecond}94.1 & \cellcolor{tabsecond}94.1 && 95.6 & 94.9 & \cellcolor{tabfirst}96.6 & \cellcolor{tabsecond}96.5 & 96.4 && \cellcolor{tabsecond}3.3 & \cellcolor{tabfirst}2.2 & 11.9 & 8.1 & 10.9 \\
living\_room && \cellcolor{tabsecond}88.0 & 85.1 & 87.7 & \cellcolor{tabsecond}88.0 & \cellcolor{tabfirst}88.3 && \cellcolor{tabfirst}95.8 & 94.6 & \cellcolor{tabsecond}95.7 & \cellcolor{tabfirst}95.8 & \cellcolor{tabfirst}95.8 && \cellcolor{tabsecond}97.4 & 96.7 & \cellcolor{tabsecond}97.4 & \cellcolor{tabsecond}97.4 & \cellcolor{tabfirst}97.5 && \cellcolor{tabfirst}9.4 & \cellcolor{tabsecond}14.3 & 30.3 & 35.1 & 49.1 \\
lounge && \cellcolor{tabfirst}34.1 & 30.2 & 33.1 & \cellcolor{tabsecond}34.0 & 33.9 && \cellcolor{tabfirst}35.4 & 34.1 & 35.0 & \cellcolor{tabsecond}35.3 & \cellcolor{tabsecond}35.3 && \cellcolor{tabfirst}35.6 & 34.8 & \cellcolor{tabsecond}35.4 & \cellcolor{tabfirst}35.6 & \cellcolor{tabfirst}35.6 && \cellcolor{tabfirst}0.4 & \cellcolor{tabfirst}0.4 & \cellcolor{tabsecond}0.6 & 1.3 & 1.8 \\
observatory && 58.4 & 63.8 & \cellcolor{tabsecond}64.7 & \cellcolor{tabfirst}65.4 & 64.4 && 83.7 & 86.3 & \cellcolor{tabsecond}86.7 & \cellcolor{tabfirst}87.0 & 86.5 && 89.9 & 91.7 & \cellcolor{tabsecond}91.9 & \cellcolor{tabfirst}92.1 & 91.8 && \cellcolor{tabsecond}5.8 & \cellcolor{tabfirst}3.3 & 25.8 & 12.2 & 24.4 \\
old\_computer && 23.3 & 49.0 & 50.7 & \cellcolor{tabsecond}53.8 & \cellcolor{tabfirst}78.7 && 41.5 & 59.6 & 58.4 & \cellcolor{tabsecond}61.4 & \cellcolor{tabfirst}90.2 && 48.4 & 61.9 & 60.1 & \cellcolor{tabsecond}63.0 & \cellcolor{tabfirst}92.7 && \cellcolor{tabsecond}5.9 & \cellcolor{tabfirst}2.2 & 11.4 & 8.4 & 19.6 \\
statue && 96.4 & \cellcolor{tabfirst}98.9 & \cellcolor{tabfirst}98.9 & \cellcolor{tabsecond}98.8 & 98.7 && \cellcolor{tabsecond}98.8 & \cellcolor{tabfirst}99.6 & \cellcolor{tabfirst}99.6 & \cellcolor{tabfirst}99.6 & \cellcolor{tabfirst}99.6 && 99.3 & \cellcolor{tabfirst}99.8 & \cellcolor{tabfirst}99.8 & \cellcolor{tabfirst}99.8 & \cellcolor{tabsecond}99.7 && \cellcolor{tabfirst}0.9 & \cellcolor{tabsecond}1.1 & 11.4 & 4.4 & 7.4 \\
terrace\_2 && 87.9 & 89.4 & \cellcolor{tabfirst}91.0 & \cellcolor{tabfirst}91.0 & \cellcolor{tabsecond}90.7 && 95.7 & 96.3 & \cellcolor{tabfirst}96.9 & \cellcolor{tabfirst}96.9 & \cellcolor{tabsecond}96.8 && 97.4 & 97.8 & \cellcolor{tabfirst}98.2 & \cellcolor{tabfirst}98.2 & \cellcolor{tabsecond}98.1 && \cellcolor{tabsecond}1.0 & \cellcolor{tabfirst}0.9 & 3.9 & 3.5 & 10.2 \\
\midrule
\textit{Average} && 60.4 & 73.5 & 78.5 & \cellcolor{tabfirst}79.3 & \cellcolor{tabsecond}79.2 && 68.1 & 82.7 & 86.3 & \cellcolor{tabfirst}87.0 & \cellcolor{tabsecond}86.5 && 70.1 & 85.0 & \cellcolor{tabsecond}88.1 & \cellcolor{tabfirst}88.8 & 88.1 && 26.5 & \cellcolor{tabfirst}7.9 & 17.1 & \cellcolor{tabsecond}16.7 & 27.5 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}



\begin{table}[t]
    \centering
    \caption{New results -- ETH3D Rig}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{AUC @ $1^\circ$} && \multicolumn{5}{c}{AUC @ $3^\circ$} && \multicolumn{5}{c}{AUC @ $5^\circ$} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} \\  \midrule

delivery\_area && 0.0 & 30.0 & \cellcolor{tabsecond}67.0 & \cellcolor{tabfirst}76.1 & 66.6 && 0.1 & 71.0 & \cellcolor{tabsecond}87.6 & \cellcolor{tabfirst}91.2 & 87.5 && 0.3 & 81.6 & \cellcolor{tabsecond}92.3 & \cellcolor{tabfirst}94.6 & 92.2 && \cellcolor{tabfirst}235.7 & \cellcolor{tabsecond}250.0 & 264.8 & 505.1 & 1745.9 \\
electro && 0.2 & 13.4 & \cellcolor{tabsecond}40.6 & \cellcolor{tabfirst}47.4 & 38.4 && 1.8 & 48.2 & \cellcolor{tabsecond}70.5 & \cellcolor{tabfirst}72.7 & 65.2 && 2.9 & 63.3 & \cellcolor{tabsecond}80.5 & \cellcolor{tabfirst}81.5 & 75.2 && \cellcolor{tabfirst}99.9 & \cellcolor{tabsecond}181.2 & 283.0 & 362.9 & 3283.1 \\
forest && 0.0 & 68.3 & 73.4 & \cellcolor{tabsecond}74.2 & \cellcolor{tabfirst}74.7 && 0.0 & 87.7 & 89.6 & \cellcolor{tabsecond}90.0 & \cellcolor{tabfirst}90.3 && 0.1 & 92.1 & 93.3 & \cellcolor{tabsecond}93.5 & \cellcolor{tabfirst}93.7 && \cellcolor{tabfirst}306.6 & \cellcolor{tabsecond}532.1 & 992.0 & 1705.8 & 7571.6 \\
playground && 0.0 & 18.0 & \cellcolor{tabfirst}45.4 & \cellcolor{tabsecond}39.5 & 0.0 && 0.1 & 40.9 & \cellcolor{tabfirst}76.6 & \cellcolor{tabsecond}72.4 & 0.0 && 0.2 & 52.0 & \cellcolor{tabfirst}84.5 & \cellcolor{tabsecond}80.9 & 0.0 && \cellcolor{tabfirst}121.5 & 386.0 & 511.2 & 854.4 & \cellcolor{tabsecond}350.2 \\
terrains && 0.7 & 19.1 & 42.4 & \cellcolor{tabfirst}50.0 & \cellcolor{tabsecond}48.0 && 2.6 & 59.1 & 74.5 & \cellcolor{tabfirst}78.1 & \cellcolor{tabsecond}76.8 && 3.1 & 71.7 & 82.8 & \cellcolor{tabfirst}85.2 & \cellcolor{tabsecond}84.3 && \cellcolor{tabfirst}62.6 & 194.7 & \cellcolor{tabsecond}176.1 & 394.1 & 1333.9 \\
\midrule
\textit{Average} && 0.2 & 29.8 & \cellcolor{tabsecond}53.8 & \cellcolor{tabfirst}57.4 & 45.5 && 0.9 & 61.4 & \cellcolor{tabsecond}79.8 & \cellcolor{tabfirst}80.9 & 64.0 && 1.3 & 72.1 & \cellcolor{tabsecond}86.7 & \cellcolor{tabfirst}87.2 & 69.1 && \cellcolor{tabfirst}165.3 & \cellcolor{tabsecond}308.8 & 445.4 & 764.5 & 2857.0 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


\begin{table}[t]
    \centering
    \caption{Refactored -- IMC}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{AUC @ $3^\circ$} && \multicolumn{5}{c}{AUC @ $5^\circ$} && \multicolumn{5}{c}{AUC @ $10^\circ$} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} \\  \midrule
bike && 0.0 & 37.9 & \cellcolor{tabsecond}65.8 & 34.9 & \cellcolor{tabfirst}77.9 && 0.0 & 47.5 & \cellcolor{tabsecond}74.3 & 38.9 & \cellcolor{tabfirst}86.7 && 0.0 & 67.7 & \cellcolor{tabsecond}80.7 & 42.9 & \cellcolor{tabfirst}93.4 && \cellcolor{tabfirst}0.0 & 2.0 & \cellcolor{tabsecond}0.9 & 1.5 & 1.1 \\
chairs && 0.0 & 16.4 & \cellcolor{tabsecond}22.0 & \cellcolor{tabfirst}82.6 & 0.8 && 0.0 & 20.3 & \cellcolor{tabsecond}27.4 & \cellcolor{tabfirst}89.6 & 0.8 && 0.0 & 26.1 & \cellcolor{tabsecond}34.4 & \cellcolor{tabfirst}94.8 & 0.8 && \cellcolor{tabfirst}0.0 & 2.8 & 1.6 & 1.6 & \cellcolor{tabsecond}0.6 \\
fountain && 22.1 & 90.6 & 89.3 & \cellcolor{tabsecond}91.2 & \cellcolor{tabfirst}91.3 && 24.2 & 94.3 & 93.6 & \cellcolor{tabsecond}94.7 & \cellcolor{tabfirst}94.8 && 25.7 & \cellcolor{tabsecond}97.2 & 96.8 & \cellcolor{tabfirst}97.4 & \cellcolor{tabfirst}97.4 && \cellcolor{tabfirst}0.8 & 2.2 & \cellcolor{tabsecond}1.8 & 3.8 & 5.9 \\
cyprus && 1.6 & \cellcolor{tabsecond}70.3 & \cellcolor{tabfirst}73.8 & 67.1 & 45.7 && 1.7 & \cellcolor{tabsecond}74.9 & \cellcolor{tabfirst}79.2 & 73.9 & 48.9 && 1.7 & 78.3 & \cellcolor{tabfirst}84.8 & \cellcolor{tabsecond}82.1 & 51.4 && \cellcolor{tabfirst}0.3 & 3.1 & \cellcolor{tabsecond}1.2 & 2.1 & 11.1 \\
dioscuri && 0.4 & 0.8 & 36.6 & \cellcolor{tabfirst}59.4 & \cellcolor{tabsecond}58.7 && 0.4 & 1.2 & 39.2 & \cellcolor{tabfirst}61.8 & \cellcolor{tabsecond}61.4 && 0.5 & 2.7 & 42.9 & \cellcolor{tabfirst}64.4 & \cellcolor{tabsecond}63.9 && \cellcolor{tabsecond}41.9 & \cellcolor{tabfirst}23.2 & 49.4 & 116.1 & 156.3 \\
wall && 57.1 & \cellcolor{tabsecond}91.6 & 22.3 & \cellcolor{tabfirst}94.6 & 88.6 && 73.9 & \cellcolor{tabsecond}95.0 & 35.0 & \cellcolor{tabfirst}96.8 & 93.2 && 87.0 & \cellcolor{tabsecond}97.5 & 59.1 & \cellcolor{tabfirst}98.4 & 96.6 && \cellcolor{tabfirst}23.8 & \cellcolor{tabsecond}35.4 & 196.5 & 66.0 & 63.5 \\
kyiv-puppet-theater && 0.7 & 4.0 & \cellcolor{tabsecond}4.1 & \cellcolor{tabfirst}12.1 & 0.3 && 0.7 & 4.7 & \cellcolor{tabsecond}5.2 & \cellcolor{tabfirst}16.1 & 0.3 && 0.9 & 6.4 & \cellcolor{tabsecond}6.6 & \cellcolor{tabfirst}19.8 & 0.3 && \cellcolor{tabfirst}0.3 & 2.0 & \cellcolor{tabsecond}0.8 & 2.7 & \cellcolor{tabfirst}0.3 \\
brandenburg\_gate && 21.4 & 1.8 & 51.6 & \cellcolor{tabsecond}70.0 & \cellcolor{tabfirst}70.1 && 35.0 & 4.6 & 62.0 & \cellcolor{tabsecond}76.4 & \cellcolor{tabfirst}77.2 && 53.6 & 12.5 & 73.4 & \cellcolor{tabsecond}82.5 & \cellcolor{tabfirst}83.9 && 1171.8 & \cellcolor{tabfirst}131.3 & \cellcolor{tabsecond}182.4 & 298.0 & 1472.1 \\
british\_museum && 18.5 & 18.1 & 43.9 & \cellcolor{tabsecond}61.0 & \cellcolor{tabfirst}61.6 && 32.0 & 29.6 & 57.2 & \cellcolor{tabsecond}71.5 & \cellcolor{tabfirst}72.7 && 51.3 & 46.9 & 73.3 & \cellcolor{tabsecond}82.2 & \cellcolor{tabfirst}83.9 && 78.1 & \cellcolor{tabfirst}44.5 & \cellcolor{tabsecond}49.6 & 115.3 & 318.0 \\
buckingham\_palace && 4.1 & 1.5 & 67.7 & \cellcolor{tabfirst}85.2 & \cellcolor{tabsecond}80.5 && 12.5 & 4.0 & 74.8 & \cellcolor{tabfirst}88.6 & \cellcolor{tabsecond}86.2 && 34.0 & 11.9 & 82.3 & \cellcolor{tabfirst}91.9 & \cellcolor{tabsecond}91.1 && 429.7 & \cellcolor{tabfirst}156.1 & \cellcolor{tabsecond}240.3 & 498.5 & 4948.2 \\
colosseum\_exterior && 37.3 & 3.0 & 41.7 & \cellcolor{tabfirst}80.8 & \cellcolor{tabsecond}80.7 && 52.8 & 6.3 & \cellcolor{tabsecond}61.5 & \cellcolor{tabfirst}86.1 & \cellcolor{tabfirst}86.1 && 69.2 & 13.5 & 77.9 & \cellcolor{tabsecond}90.7 & \cellcolor{tabfirst}90.8 && 542.8 & \cellcolor{tabfirst}331.3 & \cellcolor{tabsecond}429.9 & 804.6 & 3561.7 \\
grand\_place\_brussels && 18.3 & 8.9 & 62.7 & \cellcolor{tabfirst}70.0 & \cellcolor{tabsecond}68.7 && 32.4 & 15.1 & 72.2 & \cellcolor{tabsecond}76.5 & \cellcolor{tabfirst}76.6 && 50.5 & 33.5 & 81.3 & \cellcolor{tabsecond}82.5 & \cellcolor{tabfirst}84.2 && 124.2 & \cellcolor{tabfirst}71.6 & \cellcolor{tabsecond}94.7 & 241.0 & 520.3 \\
lincoln\_memorial\_statue && 1.0 & 7.7 & 63.2 & \cellcolor{tabfirst}68.2 & \cellcolor{tabsecond}67.2 && 4.4 & 17.0 & 68.4 & \cellcolor{tabfirst}72.3 & \cellcolor{tabsecond}71.5 && 23.8 & 33.1 & 73.4 & \cellcolor{tabfirst}75.8 & \cellcolor{tabsecond}75.3 && 99.9 & \cellcolor{tabfirst}44.3 & \cellcolor{tabsecond}50.9 & 110.0 & 362.3 \\
notre\_dame\_front\_facade && 32.5 & 1.2 & 59.7 & \cellcolor{tabsecond}66.3 & \cellcolor{tabfirst}69.1 && 43.0 & 4.5 & 65.2 & \cellcolor{tabsecond}69.9 & \cellcolor{tabfirst}72.5 && 55.2 & 14.6 & 70.6 & \cellcolor{tabsecond}73.3 & \cellcolor{tabfirst}75.5 && 2592.1 & \cellcolor{tabfirst}801.0 & \cellcolor{tabsecond}1723.6 & 4066.8 & 52135.4 \\
pantheon\_exterior && 49.6 & 51.4 & 66.2 & \cellcolor{tabsecond}75.7 & \cellcolor{tabfirst}79.4 && 62.3 & 63.1 & 74.2 & \cellcolor{tabsecond}80.5 & \cellcolor{tabfirst}83.5 && 74.4 & 74.6 & 81.9 & \cellcolor{tabsecond}84.9 & \cellcolor{tabfirst}87.2 && 285.7 & \cellcolor{tabsecond}208.7 & \cellcolor{tabfirst}174.7 & 463.8 & 1454.6 \\
piazza\_san\_marco && 2.6 & 6.2 & \cellcolor{tabsecond}68.7 & \cellcolor{tabfirst}69.9 & 58.0 && 6.4 & 16.0 & \cellcolor{tabfirst}78.9 & \cellcolor{tabfirst}78.9 & \cellcolor{tabsecond}71.0 && 23.7 & 40.7 & \cellcolor{tabfirst}88.2 & \cellcolor{tabsecond}87.1 & 83.7 && \cellcolor{tabsecond}16.7 & \cellcolor{tabfirst}12.5 & 22.7 & 46.0 & 74.2 \\
sacre\_coeur && 37.1 & 15.5 & 73.7 & \cellcolor{tabsecond}78.3 & \cellcolor{tabfirst}78.5 && 50.8 & 24.4 & 77.7 & \cellcolor{tabsecond}80.8 & \cellcolor{tabfirst}80.9 && 64.8 & 40.6 & \cellcolor{tabsecond}81.1 & \cellcolor{tabfirst}82.8 & \cellcolor{tabfirst}82.8 && 196.1 & \cellcolor{tabfirst}105.1 & \cellcolor{tabsecond}138.8 & 300.4 & 682.2 \\
sagrada\_familia && 30.3 & 47.4 & 53.1 & \cellcolor{tabsecond}53.8 & \cellcolor{tabfirst}54.3 && 39.2 & 52.7 & 57.4 & \cellcolor{tabsecond}58.7 & \cellcolor{tabfirst}58.9 && 48.9 & 57.7 & \cellcolor{tabsecond}61.7 & \cellcolor{tabfirst}62.9 & \cellcolor{tabfirst}62.9 && \cellcolor{tabsecond}42.6 & \cellcolor{tabfirst}37.5 & 53.5 & 114.1 & 237.0 \\
st\_pauls\_cathedral && 1.9 & 10.3 & 64.7 & \cellcolor{tabfirst}74.2 & \cellcolor{tabsecond}72.7 && 6.5 & 24.6 & 73.5 & \cellcolor{tabfirst}80.3 & \cellcolor{tabsecond}78.9 && 25.8 & 44.8 & 81.8 & \cellcolor{tabfirst}85.8 & \cellcolor{tabsecond}85.0 && 61.9 & \cellcolor{tabfirst}35.9 & \cellcolor{tabsecond}52.0 & 94.2 & 241.4 \\
st\_peters\_square && 31.1 & 6.2 & 66.4 & \cellcolor{tabsecond}79.1 & \cellcolor{tabfirst}83.6 && 46.0 & 12.4 & 74.7 & \cellcolor{tabsecond}83.9 & \cellcolor{tabfirst}87.8 && 64.0 & 24.8 & 83.0 & \cellcolor{tabsecond}88.7 & \cellcolor{tabfirst}91.6 && 961.0 & \cellcolor{tabfirst}374.9 & \cellcolor{tabsecond}505.6 & 1055.2 & 6051.9 \\
taj\_mahal && 38.6 & 4.9 & 68.8 & \cellcolor{tabfirst}74.4 & \cellcolor{tabsecond}68.9 && 51.0 & 11.4 & 74.2 & \cellcolor{tabfirst}78.9 & \cellcolor{tabsecond}75.5 && 64.9 & 23.6 & 80.0 & \cellcolor{tabfirst}83.5 & \cellcolor{tabsecond}81.7 && 380.1 & \cellcolor{tabfirst}176.4 & \cellcolor{tabsecond}326.5 & 539.6 & 4528.9 \\
trevi\_fountain && 43.4 & 22.6 & 74.6 & \cellcolor{tabsecond}79.1 & \cellcolor{tabfirst}80.5 && 56.2 & 40.5 & 79.7 & \cellcolor{tabsecond}82.8 & \cellcolor{tabfirst}84.4 && 69.3 & 59.2 & 84.6 & \cellcolor{tabsecond}86.4 & \cellcolor{tabfirst}87.8 && 1202.9 & \cellcolor{tabsecond}689.5 & \cellcolor{tabfirst}569.5 & 1718.5 & 12294.4 \\
\midrule
\textit{Average} && 20.4 & 23.6 & 56.4 & \cellcolor{tabfirst}69.4 & \cellcolor{tabsecond}65.3 && 28.7 & 30.2 & 63.9 & \cellcolor{tabfirst}74.5 & \cellcolor{tabsecond}70.4 && 40.4 & 41.3 & 71.8 & \cellcolor{tabfirst}79.1 & \cellcolor{tabsecond}75.1 && 412.6 & \cellcolor{tabfirst}149.6 & \cellcolor{tabsecond}221.2 & 484.5 & 4051.0 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}


\begin{table}[t]
    \centering
    \caption{New results -- SLAM}
    \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c c a l c c c c a l c c c c a l c c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{5}{c}{Recall @ 0.1m} && \multicolumn{5}{c}{AUC @ 0.1m} && \multicolumn{5}{c}{AUC @ 0.5m} 
        && \multicolumn{5}{c}{Time (s)}
        \\
        \cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-19} \cmidrule{21-25}
        && \tiny{OpenMVG} & \tiny{Theia} & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{Theia}  & \tiny{~Paper~} & \tiny{Current} & \tiny{COLMAP} \\  \midrule
cables && \cellcolor{tabsecond}76.8 & \cellcolor{tabfirst}88.0 & \cellcolor{tabfirst}88.0 & \cellcolor{tabfirst}88.0 & \cellcolor{tabfirst}88.0 && 59.1 & 53.6 & \cellcolor{tabfirst}77.0 & 66.1 & \cellcolor{tabsecond}75.3 && 77.4 & 81.1 & \cellcolor{tabfirst}85.8 & 83.6 & \cellcolor{tabsecond}85.4 && \cellcolor{tabsecond}103.1 & 170.9 & \cellcolor{tabfirst}68.5 & 179.2 & 2553.4 \\
camera && 2.2 & \cellcolor{tabsecond}33.0 & \cellcolor{tabfirst}47.1 & 32.3 & 32.5 && 2.0 & 15.7 & \cellcolor{tabfirst}32.5 & \cellcolor{tabsecond}22.4 & \cellcolor{tabsecond}22.4 && 2.2 & \cellcolor{tabsecond}35.4 & \cellcolor{tabfirst}44.9 & 30.7 & 30.8 && \cellcolor{tabfirst}1.5 & 24.6 & 11.5 & \cellcolor{tabsecond}7.3 & 196.2 \\
ceiling && 6.4 & 28.2 & \cellcolor{tabfirst}33.8 & 28.5 & \cellcolor{tabsecond}28.6 && 2.9 & 11.8 & 15.3 & \cellcolor{tabsecond}19.3 & \cellcolor{tabfirst}21.1 && 8.2 & \cellcolor{tabsecond}29.0 & \cellcolor{tabfirst}30.8 & 26.8 & 27.2 && \cellcolor{tabsecond}78.3 & 132.5 & \cellcolor{tabfirst}62.3 & 101.8 & 1057.7 \\
desk && 28.0 & \cellcolor{tabsecond}33.8 & \cellcolor{tabfirst}34.2 & 32.3 & 32.3 && 16.0 & 17.2 & 27.1 & \cellcolor{tabsecond}28.3 & \cellcolor{tabfirst}29.0 && 28.6 & \cellcolor{tabsecond}32.9 & \cellcolor{tabfirst}35.2 & 31.5 & 31.7 && 376.2 & 200.9 & \cellcolor{tabfirst}92.3 & \cellcolor{tabsecond}159.8 & 1115.1 \\
einstein && 32.9 & 41.3 & 43.2 & \cellcolor{tabsecond}47.1 & \cellcolor{tabfirst}49.4 && 22.7 & 29.2 & \cellcolor{tabsecond}33.6 & 31.0 & \cellcolor{tabfirst}37.2 && 34.2 & 42.4 & 42.8 & \cellcolor{tabsecond}46.6 & \cellcolor{tabfirst}48.0 && 150.3 & \cellcolor{tabfirst}61.2 & \cellcolor{tabsecond}61.5 & 152.1 & 1230.8 \\
kidnap && \cellcolor{tabsecond}73.1 & \cellcolor{tabfirst}73.3 & \cellcolor{tabfirst}73.3 & \cellcolor{tabfirst}73.3 & \cellcolor{tabfirst}73.3 && 63.4 & 59.8 & \cellcolor{tabsecond}69.5 & 69.1 & \cellcolor{tabfirst}70.0 && 71.2 & 70.6 & \cellcolor{tabsecond}72.5 & \cellcolor{tabsecond}72.5 & \cellcolor{tabfirst}72.6 && \cellcolor{tabsecond}114.4 & 668.8 & \cellcolor{tabfirst}64.0 & 136.6 & 731.2 \\
large && 35.4 & \cellcolor{tabsecond}47.6 & 37.3 & \cellcolor{tabfirst}49.0 & \cellcolor{tabfirst}49.0 && 18.1 & 20.2 & 31.7 & \cellcolor{tabsecond}37.0 & \cellcolor{tabfirst}45.1 && 33.7 & 43.4 & 36.8 & \cellcolor{tabsecond}46.6 & \cellcolor{tabfirst}48.2 && 91.9 & 113.0 & \cellcolor{tabfirst}42.1 & \cellcolor{tabsecond}73.7 & 983.8 \\
mannequin && 49.1 & 58.5 & \cellcolor{tabfirst}67.9 & 66.1 & \cellcolor{tabsecond}66.8 && 36.7 & 39.0 & 48.5 & \cellcolor{tabsecond}52.2 & \cellcolor{tabfirst}55.8 && 49.1 & 58.5 & \cellcolor{tabfirst}67.0 & 64.0 & \cellcolor{tabsecond}64.8 && \cellcolor{tabsecond}33.5 & 66.5 & \cellcolor{tabfirst}26.1 & 43.9 & 301.2 \\
motion && 18.8 & 14.1 & 23.1 & \cellcolor{tabsecond}42.0 & \cellcolor{tabfirst}44.7 && 11.0 & 7.7 & 10.3 & \cellcolor{tabsecond}19.6 & \cellcolor{tabfirst}23.1 && 23.3 & 13.7 & 28.2 & \cellcolor{tabsecond}55.2 & \cellcolor{tabfirst}56.1 && 859.7 & \cellcolor{tabfirst}84.8 & \cellcolor{tabsecond}291.4 & 654.2 & 9995.1 \\
planar && \cellcolor{tabsecond}30.6 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 12.5 & 94.4 & 97.6 & \cellcolor{tabsecond}98.2 & \cellcolor{tabfirst}98.7 && 38.0 & 98.9 & 99.5 & \cellcolor{tabsecond}99.6 & \cellcolor{tabfirst}99.7 && 313.8 & \cellcolor{tabfirst}154.8 & \cellcolor{tabsecond}228.5 & 572.4 & 2349.7 \\
plant && 77.0 & 87.0 & 90.4 & \cellcolor{tabsecond}90.9 & \cellcolor{tabfirst}92.0 && 62.9 & 71.4 & 75.1 & \cellcolor{tabsecond}78.1 & \cellcolor{tabfirst}81.4 && 77.1 & 89.4 & \cellcolor{tabsecond}92.0 & 90.7 & \cellcolor{tabfirst}92.1 && \cellcolor{tabsecond}21.7 & 48.8 & \cellcolor{tabfirst}19.9 & 26.9 & 202.7 \\
reflective && 12.6 & 16.2 & 18.8 & \cellcolor{tabsecond}21.1 & \cellcolor{tabfirst}22.2 && 6.7 & 4.8 & \cellcolor{tabsecond}7.0 & 6.8 & \cellcolor{tabfirst}8.6 && 16.5 & 20.0 & 24.9 & \cellcolor{tabsecond}28.8 & \cellcolor{tabfirst}29.1 && 721.3 & \cellcolor{tabfirst}104.7 & \cellcolor{tabsecond}171.6 & 448.1 & 6573.9 \\
repetitive && 26.3 & 28.7 & \cellcolor{tabfirst}33.3 & 32.4 & \cellcolor{tabsecond}32.7 && 23.9 & 14.1 & \cellcolor{tabfirst}27.3 & 23.2 & \cellcolor{tabsecond}26.7 && 25.8 & 26.8 & \cellcolor{tabfirst}32.1 & 30.7 & \cellcolor{tabsecond}31.5 && \cellcolor{tabsecond}63.2 & 106.4 & \cellcolor{tabfirst}53.0 & 86.7 & 561.1 \\
sfm && 83.2 & 90.4 & 90.1 & \cellcolor{tabsecond}96.5 & \cellcolor{tabfirst}97.0 && 57.9 & 46.0 & 62.2 & \cellcolor{tabsecond}76.1 & \cellcolor{tabfirst}78.3 && 80.0 & 86.3 & 89.5 & \cellcolor{tabsecond}94.3 & \cellcolor{tabfirst}95.0 && \cellcolor{tabfirst}91.7 & \cellcolor{tabsecond}158.7 & 207.7 & 209.5 & 469.6 \\
sofa && 11.2 & 18.6 & \cellcolor{tabfirst}24.2 & 23.8 & \cellcolor{tabsecond}23.9 && 5.5 & 10.7 & 14.0 & \cellcolor{tabsecond}18.8 & \cellcolor{tabfirst}21.8 && 10.3 & 18.3 & \cellcolor{tabsecond}23.0 & 22.9 & \cellcolor{tabfirst}23.5 && \cellcolor{tabsecond}9.1 & 9.9 & \cellcolor{tabfirst}8.2 & 10.1 & 157.3 \\
table && 79.1 & 83.9 & \cellcolor{tabfirst}99.9 & \cellcolor{tabsecond}94.3 & \cellcolor{tabsecond}94.3 && 68.2 & 57.8 & 74.8 & \cellcolor{tabsecond}83.7 & \cellcolor{tabfirst}88.5 && 76.9 & 81.9 & \cellcolor{tabfirst}94.9 & 92.2 & \cellcolor{tabsecond}93.2 && 182.0 & \cellcolor{tabfirst}61.2 & \cellcolor{tabsecond}89.9 & 233.1 & 2777.7 \\
vicon && 64.6 & 74.4 & \cellcolor{tabsecond}94.8 & 94.4 & \cellcolor{tabfirst}97.0 && 20.4 & 49.6 & 56.5 & \cellcolor{tabsecond}66.8 & \cellcolor{tabfirst}79.1 && 71.7 & 84.0 & \cellcolor{tabsecond}91.0 & 90.9 & \cellcolor{tabfirst}93.5 && 50.9 & 149.8 & \cellcolor{tabfirst}33.2 & \cellcolor{tabsecond}47.4 & 474.8 \\
\midrule
\textit{Average} && 48.2 & 60.1 & \cellcolor{tabsecond}65.5 & \cellcolor{tabsecond}65.5 & \cellcolor{tabfirst}66.3 && 34.9 & 40.6 & 49.7 & \cellcolor{tabsecond}52.1 & \cellcolor{tabfirst}56.0 && 48.6 & 60.0 & \cellcolor{tabsecond}64.8 & 64.4 & \cellcolor{tabfirst}65.3 && 120.8 & \cellcolor{tabsecond}97.7 & \cellcolor{tabfirst}70.2 & 130.6 & 1115.4 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:mip360_instant_ngp}
    % \vspace{-20px}
\end{table}

